Towards Fair and Explainable AI using a Human-Centered AI Approach

The rise of machine learning (ML) is accompanied by several high-profile cases that have stressed the need for fairness, accountability, explainability and trust in ML systems. The existing literature has largely focused on fully automated ML approaches that try to optimize for some performance metric. However, human-centric measures like fairness, trust, explainability, etc. are subjective in nature, context-dependent, and might not correlate with conventional performance metrics. To deal with these challenges, we explore a human-centered AI approach that empowers people by providing more transparency and human control. In this dissertation, we present 5 research projects that aim to enhance explainability and fairness in classification systems and word embeddings. The first project explores the utility/downsides of introducing local model explanations as interfaces for machine teachers (crowd workers). Our study found that adding explanations supports trust calibration for the resulting ML model and enables rich forms of teaching feedback. The second project presents D-BIAS, a causality-based human-in-the-loop visual tool for identifying and mitigating social biases in tabular datasets. Apart from fairness, we found that our tool also enhances trust and accountability. The third project presents WordBias, a visual interactive tool that helps audit pre-trained static word embeddings for biases against groups, such as females, or subgroups, such as Black Muslim females. The fourth project presents DramatVis Personae, a visual analytics tool that helps identify social biases in creative writing. Finally, the last project presents an empirical study aimed at understanding the cumulative impact of multiple fairness-enhancing interventions at different stages of the ML pipeline on fairness, utility and different population groups. We conclude by discussing some of the future directions.

==> chapters/archive/chapter04/chap04.tex <==
\let\textcircled=\pgftextcircled
\chapter{Implementation}
\label{chap:imple}

\begin{figure}[tb]
 \centering 
 \includegraphics[width=1.0\columnwidth]{fig04/SyntheticData}
  \setlength{\belowcaptionskip}{-8pt}
\setlength{\abovecaptionskip}{-4pt}

 \caption{The flow chart for the construction of the synthetic hiring dataset.}
 \label{fig:synthetic}
\end{figure}


\section{Implementation}
We will present how the D-BIAS tool can be used to mitigate the effects of bias. We will first explain the different parts of the tool and then illustrate its use by ways of a synthetic dataset.

\subsection {Visual Tool}
The visual tool can be divided into three parts (1) Influence Detection Suite, (2) Fairness Adjustment Suite and (3) Fairness Report Suite.

\subsubsection{Influence Detection Suite}
The influence detection suite contains parts of the visual tool that identify how the different attributes influence each other. This influence structure plays a vital role in identifying and mitigating the effect of bias. The suite is composed of four parts.

The \textbf{Control Panel} (see \autoref{fig:teaser}(a)) is used to change the different parameters related to the data as well as the Influence Network. The \textbf{Influence Network} (see \autoref{fig:teaser}(b)) shows the causal model as well as the correlation model. Edges are used to show how influence flows through the network. A green colored edge shows a positive influence and a red colored edge shows a negative influence. The green plus sign or the red minus sign (if presents) attached to an edge shows if the relation is benefiting the model quality. This is measured by the difference of a regression's Bayesian Information Criterion (BIC) punishment with and without the relation. Note that a lower BIC punishment means a better regression model. The change of the overall model's quality, which is the sum of the BIC of all regressions, are displayed as a bar on the right. The user can make changes to the model using the control panel as well as the Relation Suggestions. 

The \textbf{Relation Suggestion} panel (see \autoref{fig:teaser}(c)) recommends different relations to the user. The relations are ranked using the method discussed in \autoref{sec:suggestions}. We use different shades of grey to represent add, reverse and delete options. The \textbf{Influence Parameters} panel (see \autoref{fig:teaser}(d)) shows the confidence scores as well as the regression analysis of the causal model regarding each node and its predictors. The user can click on any node in the causal graph to see the parameters.

\subsubsection{Fairness Adjustment Suite}
The \textbf{Fairness Adjustment Suite} (see \autoref{fig:teaser}(e)) allows the user to adjust the influence of the different attributes.  The slider corresponding to an attribute can be used to adjust the influence associated with that attribute. The user can also select the protected variable in the dataset by selecting the combo box in front of the attribute.

\subsubsection{Fairness Report Suite}
The Fairness Report suite shows the visualization and evaluation of the bias mitigation process. The \textbf{Group Fairness Plot} (see \autoref{fig:teaser}(f)) visualizes the data using a dimension reduction technique. The points in the plot are colored using the group variable selected by the user. Various evaluation metrics relating to the fairness, utility and distortion of the data are shown in the \textbf{Performance Panel} (see \autoref{fig:teaser}(g)).

\subsection{Synthetic Dataset}
We use a synthetic dataset instead of a real dataset because the source of the bias can be clearly explained using a relatively small number of attribute variables. Real world examples will be presented in \autoref{sec:usage_scenario}.  

The synthetic dataset relates to a hiring firm. The dataset has ten attributes; the attributes are generated using the  chart shown in \autoref{fig:synthetic}. Each attribute is constructed using a weighted sum of its parent nodes and random noise. $Intelligence$ is treated as a latent variable and therefore is not included in the actual dataset. 


\begin{figure*}[tb]
 \centering 
 \includegraphics[width=1.85\columnwidth]{fig04/Workflow1}
 \setlength{\belowcaptionskip}{-8pt}
\setlength{\abovecaptionskip}{0pt}
 \caption{The workflow of the synthetic hiring dataset. (a) The default Influence Network. (b) The Relations Suggestions panel. (c) Updated Influence Network. (d) Influence Parameters. (e) The Group Fairness Plot, shows the original dataset and the debiased dataset. Using the $Sex$ attribute to color the points. (f) The Fairness Adjustment Panel panel, showing the weights calculated using the "Remove Collinearity" strategy. (g) The Group Fairness Plot, shows the original dataset and the debiased dataset. Using the $College\_Rank$ attribute to color the points.}
 \label{fig:workflow}
\end{figure*}

\begin{figure}[tb]

 \centering 
 \includegraphics[width=1.0\columnwidth]{fig04/syn_eval}
\setlength{\belowcaptionskip}{-8pt}
\setlength{\abovecaptionskip}{-4pt}
\caption{Detailed evaluation of the synthetic hiring dataset. The image compares the debiased data with the original data using different evaluation metrics.}
 \label{fig:syn_eval}
\end{figure}

\subsection{Illustration}
We will now illustrate how the visual tool can be used for both debiasing strategies (Factor-based Debiasing and Representation Balancing). We will utilize a  hypothetical example of a hiring manager, Jane, who wants to investigate the dataset of previous job applicants in her company. 

\subsubsection{Factor-based Debiasing} 
Jane knows that her company's hiring policy emphasizes grade point average, work experience, and the college rank of the applicant and does not discriminate on the basis of race or sex of the applicant. However, after reading how bias can creep into seemingly unbiased decision making processes she decides to use D-BIAS to analyze her dataset. She identifies $Race$ and $Sex$ as the two protected variables in the dataset. She would like to ensure that there is no discrimination based on these attributes. In the event that there is some bias in the hiring process of the company she would like to mitigate the effect of the bias.% so that the hiring process does not discriminate on the basis of race or sex. 



Jane uploads the synthetic dataset into the system using the control panel. She selects $Job$ as the label variable. In the Nominal Attribute panel she selects $Race$. As discussed in \autoref{sec:causal_inference} nominal variables are treated differently from numeric and ordinal data. We ask the user to manually select the nominal attributes in the data because it is difficult to differentiate between nominal and ordinal attributes automatically. Jane chooses the causal model to discover the relations between the attributes of the data. 

The causal model (see \autoref{fig:workflow}(a)) shows the causal relations of the data. The causal relations are discovered using the method described in \autoref{sec:causal}, but the output attribute \textit{Job} is ignored as we will use it to measure the performance of our methods later. We can see that the causal model has extracted the relations that were coded into the artificial dataset (see \autoref{fig:synthetic}). All the causal links have been captured. However, the method has been unable to determine the direction of the edge between $Age$ and $Experience$. The model also detects an undirected edge between $SAT\_Score$ and $Highschool\_Grade$, since the same latent variable ($Intelligence$) was used to create them. Jane now inspects the causal graph to see whether the edges are plausible using her knowledge of how things work in the hiring business.
%The causal model makes certain assumptions about the dataset which may not be true. Jane can use their own judgment and knowledge of how things work in the real world to alter the structure of the causal model.
%The visual tool assists the user in creating a proper causal model. The control panel allows the user to add, remove or reverse the direction of an edge. Semantic analysis of the attributes is also used to give the user suggestions on possible edges in the graph. 



Jane examines the causal graph and finds it interesting that $Sex$ has a causal edge leading to $College\_Rank$. To gain a more overall understanding of the factors influencing  $College\_Rank$ let us pause for a moment and open $College\_Rank$ in the Causal Models Parameters panel. The Causal Models Parameters panel shows the regression analysis of the causal model regarding each node and its predictors (see \autoref{fig:workflow}(b)). Here, we see that the regression model of $College\_Rank$ shows a zero p-value from the F-statistics, meaning the model fits the data very well. What's more, by looking at the coefficients of the independent variables, we observe that both $Sex$ and $SAT\_Score$ have a strong and similar influence on $College\_Rank$. This is consistent with how we constructed the dataset. 
 
The causal link from $Sex \to College\_Rank$ suggests to Jane that there might be bias based on $Sex$ in her company's hiring process. Since $College\_Rank$ is an important variable for hiring, its causal relation to $Sex$ apparently produces an unintended bias in the hiring decisions. 
%Even though Jane and her hiring team do not discriminate on the basis of $Sex$, 
It seems that there is a bias in the admissions process of the colleges which is indirectly affecting the hiring process. Conversely. $Race$, the second protected variable is unrelated to the other variables and therefore it will not affect the hiring process.

Jane examines the other links in the causal graph. She uses her  knowledge to direct the edge between $"Age"$  and $"Highschool\_Grade"$  from the former to the latter using the control panel. The Relations Suggestions panel (see \autoref{fig:workflow}(c)) gives Jane some suggestions on possible edges in the causal model. The suggestions are generated by combining semantic analysis with the causal model. Since there is a semantic similarity between the attributes $SAT\_Score$ , $Highschool\_Grade$ and $Grade\_Point\_Average$ there are suggestions to make the edges from and to these attributes similar, such as from $SAT\_Score \to Highschool\_Grade$, $Highschool\_Grade \to College\_Rank$ etc. Jane looks at the suggestions and decides to add the edge $SAT\_Score \to Highschool\_Grade $ into the graph.  The Model Score Variation shows that the model's BIC decreases, which means the model has improved. Jane examines the other edges and is satisfied with the structure of the causal graph. The final causal model can be seen in \autoref{fig:workflow}(d). 

  

She then selects $Sex$ as the protected variable in the slider panel and selects the Factor-based Debiasing strategy. The debiased results are shown in the Group Fairness Plot panel and the Performance panel. \autoref{fig:workflow}(e) shows the visualization of the bias removal. 
The original data and debiased data are visualized using t-SNE \cite{maaten2008visualizing}. 
The points in the scatter plot are colored using the protected variable. We observe that in the original dataset the two clusters are completely separated indicating strong bias. However, after removing the effect of bias from the dataset the separation due to $Sex$ has vanished from the visualization! 

This positive change is also reflected in the difference between the two datasets in the Detailed Performance Panel (see \autoref{fig:syn_eval}). The Detailed Performance Panel shows the results of the individual machine learning algorithms that are used to determine the Accuracy and Data Discrimination scores. 
%In addition to the visual representation of bias we also use supervised machine learning methods to evaluate the degree to which the data has been debiased. The results of the above mentioned metrics are shown in \autoref{fig:syn_eval}.
The Accuracy  and Individual Fairness metric show that the measures remain more or less the same. 
%However, most machine learning methods are able to identify a decease in discrimination in the unbiased \colorbox{yellow}{dataset} \marginpar{\small Explain why decision tree has a different result.}.
Further, the results are achieved with a relatively small amount of data distortion.

\subsubsection{Representation Balancing}
Jane also wants to see how bias due to over representation effects the data.
%Jane opens the correlation model to see the correlation between the attributes (see \autoref{fig:workflow}(f)).  The correlation model uses Pearson's correlation to determine the layout of the different attributes. Attributes that are close together have a higher correlation. The causal edges between the attributes can also be seen in the correlation model. Jane observes that the attributes related to intelligence ($SAT\_Score, Highschool\_Grade, Grade\_Point\_Average$) have strong collinearity. The may suggest that this aspect is being over represented in the the data.
Jane decides to use the Representation Balancing strategy to reduce the effect of collinearity. She updates the weights of the attributes by clicking the Assess Weights function in the Fairness Adjustment panel. The weights of the individual attributes are updated (see \autoref{fig:workflow}(f)) based on the method described in \autoref{sec:coll}. The weights of $Highschool\_Grade,\ College\_Rank,\ Grade\_Point\_Average$ and $SAT\_Score$ show significant reduction. Since these are all referring to the same aspect of the data their value is now under-emphasized which removes the over representation bias. The results of the emphasis reduction are seen in the Group Fairness Plot  (\autoref{fig:workflow}(g)). The scatter plots are colored using the $College\_Rank$ attribute. In the visualization of the original data we can see that points that are close together have a similar color. This shows that $College\_Rank$ 
is a strong contributor to the structure of the dataset ($Highschool\_Grade,\ Grade\_Point\_Average$ and $SAT\_Score$ also show similar visualizations). Visualization of the debiased data shows that the influence of this aspect of the data has been reduced. However, this represents a process bias that Jane wants to keep in the hiring data. Therefore, she decides to ignore these results.


==> chapters/archive/chapter05/chap05.tex <==
\let\textcircled=\pgftextcircled
\chapter{Usage Scenario}
\label{chap:usage}

We will now present two usage scenarios of our visual tool that use real world data. In these scenarios the objective of the user is to identify sources of bias in the data and mitigate the effect of that bias. 

\begin{figure*}[tb]
 \centering 
 \includegraphics[scale=0.5]{fig05/adult-income}
  \setlength{\belowcaptionskip}{0pt}
\setlength{\abovecaptionskip}{0pt}
 \caption{The workflow of the Adult income dataset. (a-b) The default causal map. (b) The updates causal map. (c) The Group Fairness Plot using the  $Sex$ attribute to color the points. (d) Performance Panels. (e) Fairness Adjustment Panel using the Representation Balancing strategy. (f) The Group Fairness Plot using $Age$ attribute to color the points. (g) Performance Panel. (h) The updates Fairness Adjustment Panel. (i) Performance Panel for the updated weights.}
 \label{fig:adultMDS}
\end{figure*}

\subsection{German Credit Dataset}
The German Credit dataset  \cite{germanUCI} is a popular dataset which has been used in multiple studies dealing with bias \cite{zemel2013learning, kamiran2009classifying}. It consists of 1,000 rows and 20 columns with a mix of categorical and numerical attributes. Each row represents different features corresponding to a person, such as account balance, credit amount, sex, marital status, etc. These input attributes can be used to classify a person as having low or high credit risk. We will use $Age$ as the protected variable, which is a binary variable in the dataset. In the following use case we first try to analyze causal relationships between different attributes. Thereafter, we will assess and  mitigate bias for different age groups with respect to their credibility risk.

\begin{figure}[tb]
 \centering 
 \includegraphics[width=0.6\columnwidth]{fig05/adult-income2}
  \setlength{\belowcaptionskip}{-12pt}
\setlength{\abovecaptionskip}{0pt}
 \caption{Performance Panel for the Factor-based debiasing strategy. The images shows the performance metrics for different weights affecting the sex variable.}
 \label{fig:adult_eval}
\end{figure}

We select the attribute $Creditability$ (this attribute represents the credibility risk of a person) as the label variable. The attributes $Payment\_Status\_of\_Previous\_Credit, \ Occupattion, \ Type\_of\_Apartment$ and $Sex\_and\_Marital\_Status$ are selected as nominal attributes. The causal graph generated by the data can be seen in \autoref{fig:teaser}(b).  The graph shows that $Age$ has edges to the attributes $Duration\_in\_Current\_Address$, $Length\_of\_Current\_Employment$,   $Telephone$,  $Type\_of\_ Apartment$, $Sex\_and\_Marital\_Status$  and  $No\_of\_Dependents$. We learn that older people are more likely to have telephones, and that the marital status of a person is also linked with age. It is easy to see how all of the attributes would be effected by $Age$. 

Since there are many nodes and edges in the causal graph it is possible that the user may miss some potential edges.
The Relation Suggestions panel shows potential relations, and there are quite a few suggestions that seem plausible. However, adding too many edges may introduce personal bias into the system and the new relations may not be supported by the data. Therefore, it is not advisable to add too many relations in the causal model. We add the edge $Age \to Duration\_of\_Credit$ because other attributes related to the duration are also connected to $Age$ (see \autoref{fig:teaser}). 

We can see that the $Age$ attribute is influencing many other attributes that would effect whether a person is considered a credit risk or not. To reduce the bias  we select  $Age$ as a protected variable in the Debias Weight panel, and select the Representation Balance strategy. The results of the debiasing can be seen in  \autoref{fig:teaser}(f, g). In the original dataset, we can see the distribution of the two clusters is uneven, whereas the distribution in the unbiased dataset is relatively even.
These observations are also confirmed by the clustering metrics and the data distribution. We can see that the individual fairness and accuracy of the unbiased dataset is also very similar to the original dataset. However, the reduction of bias did cause some distortion in the data. 



\subsection{Adult Income dataset}
Our second use case will try to reduce bias in the adult income dataset, which can be used to predict if a person's income will be greater or less than \$50k based on attributes like age, sex, education, marital status, etc. Each data point in the dataset represents a person described by 14 attributes recorded from the US 1994 census. The dataset is also widely used in other studies dealing with algorithmic bias \cite{inprocess,sureshKDD,nipsIBM}. In this use case, we will try to mitigate the influence of gender on income with the strategies discussed in Section \ref{debiaisngTech}

%In our study, we first analyzed causal influences between different attributes. Thereafter, we tried to mitigate the influence of gender on income using debiasing strategies discussed in \ref{debiaisngTech}. 

%Before feeding dataset into our system, we did a bit of preprocessing. We dropped two nominal columns namely, country and occupation from the dataset since they have more than 15 levels making it difficult to quantize them.

After feeding the dataset into our visual tool, \textit{income} is selected as the label attribute and \textit{sex} as the protected variable. \textit{Race}, \textit{relationship}, \textit{marital status} and \textit{work class} are the nominal variables in the dataset. Thereafter, we built the influence network shown in \autoref{fig:adultMDS}(a)), which describes the underlying data dependency and how the bias is propagated. 
%To counter this inherent bias, our system enables the end user to make changes to the causal network based on domain knowledge or real world experience. 
Here, we observe that there is a link from $sex$ to $age$, $relationship$, $race$ and $hours\_per\_week$. Based on real world experience, we know that race or age of a person is not influenced by his/her sex, hence we delete the two edges from the causal network. These changes will propagate throughout the network and will impact the debiasing process. Furthermore, we observe that there are a few dotted edges which represent weak links. We eliminate these edges simply by selecting the Remove Weak Relations functionality in the control panel. Similarly, we can tune coefficients of the threshold parameter to retain only those edges implying strong influences. \autoref{fig:adultMDS}(b) shows the resulting causal graph devoid of weak links and infused with domain knowledge. Thereafter, we ran the factor based debiaisng (see \autoref{sec:remove_protected}) using $sex$ as the protected variable.    

\begin{comment}
\begin{figure}[tb]
 \centering 
 \includegraphics[width=1.0\columnwidth]{fig05/adult_metrics}
 \caption{Different evaluation metrics for debiased Adult income dataset}
 \label{fig:adultMet}
\end{figure}
\end{comment}
\autoref{fig:adultMDS}(c)) shows the MDS layout for the original and debiased datasets, colored by the sex attribute. We can observe that the distribution of points with respect to sex is more uniformly spread in the debiased data than in the original data. \autoref{fig:adultMDS}(d) shows that the accuracy for the debiased dataset is virtually the same as for the original dataset while there is a significant drop in group bias and cluster bias. This means that we have preserved the utility of the original dataset in terms of accuracy while significantly reducing bias. 

Different use cases might require us to remove the influence of a protected variable by different extents. Our system provides the flexibility to assign weights to protected variables and decrease their influence accordingly. $Weight=1$ means maximum debiasing and $Weight=0$ means no debiasing. \autoref{fig:adult_eval} represent debiasing with $sex$ as the protected attribute to three different extents. We can observe that group and cluster bias increase as we move from  weight=1 (left) to weight=0.5 (right). But we also observe that debiasing comes at the cost of data distortion. The higher the weight, the higher the distortion. This experiment shows the advantage of an interactive visual interface likes ours. It enables the end user to make an informed decision for the optimal weight based on his or her specific use case and objectives.            
%We also observed that infusing domain knowledge into the network by changing the causal network actually helped the group fairness score. In this case, removing a couple of edges enhanced group fairness of resulting dataset.    


Next, we tried to counter over-representation using the representation balancing technique \autoref{sec:coll}. The initial steps to construct the causal network (as shown in \autoref{fig:adultMDS}(b)) are the same as with the factor based debiaisng. Thereafter, we access the weights as shown in \autoref{fig:adultMDS}(e). We observe that $age$ and other attributes pointing to it like $martial status$ and $sex$ are being assigned lower weights. This suggests that the $age$ attribute is overrepresented in the original dataset. After debiasing, we observe that the distribution of points with respect to age are more uniformly spread in the debiased dataset (see \autoref{fig:adultMDS}(f)). Performance metrics shown in \autoref{fig:adultMDS}(g) also confirm that group bias and cluster bias with respect to age has dropped while preserving accuracy. 

\subsubsection{Managing Procedural Fairness and Priorities}
The representation balancing technique can be also used to introduce institutional preferences into a decision pipeline. This is accomplished by introducing procedural bias \cite{processFairness} via tuning the weights. For example, an organization might decide to pay higher salary to more educated employees. But at the same time it wants to avoid to be accused of biasing towards other personal traits and attributes, such as age, race, sex, etc. which could expose them to workforce discontent or even legal action. The company would use our system and assign a higher weight to education such that education has a higher influence on income, as shown in \autoref{fig:adultMDS}(h) where we increase the weight for education from 0.7 (\autoref{fig:adultMDS}(e)) to 0.9. Thereafter, we compare the performance metrics before (\autoref{fig:adultMDS}(g)) and after (\autoref{fig:adultMDS}(i)) the change. We observe that there is only a small change in cluster bias and data distortion but accuracy and individual fairness are pretty much the same. Different organizations may tune the weights to levels that meet their own objectives while keeping the bias at a level they are comfortable with.


==> chapters/archive/chapter07/chap07.tex <==
\let\textcircled=\pgftextcircled
\chapter{Conclusion}
\label{chap:conclusion}

In this paper, we have described a visual analytics approach that allows users to remove bias from data and manage the amount of bias still remaining. Our framework uses advanced statistical techniques like causality and semantic analysis to assist the user in the bias removal and management process. Detecting bias in a dataset, and enforcing fairness in automated decision making systems that make use of these data is a difficult task. It requires an understanding of how the different attributes of the data are related to each other. Our tool brings the human into the bias detection process and allows the user to make adjustments towards that end in an informed manner. 

We use the visual representations of the causal and correlation models to communicate to the user how the different attributes of the data are related to each other. The user can adjust the amount of bias they wish to remove from the data. Visualizations of the data before and after bias removal give a pictorial representation of the bias removal. However, involving the user into the bias removal process has the downside of introducing undesired process bias into the system as well as reduce the accuracy of the automated decision making systems that use the data.
In order to safeguard the user from process bias we have provided multiple metrics regarding fairness, distortion and utility of the data and show visuals of these in our interface.

We have presented two different use cases to demonstrate how our visual tool can be used in practice. We believe our tool makes it easy for the user to understand and influence the bias removal process. For the future we plan to apply our tool to a variety of real-life settings and data. This will help us to fine tune the components and recognize the span of possible application areas.

==> frontmatter/declaration.tex <==
%
% File: declaration.tex
% Author: V?ctor Bre?a-Medina
% Description: Contains the declaration page
%
% UoB guidelines:
%
% Author's declaration
%
% I declare that the work in this dissertation was carried out in accordance
% with the requirements of the University's Regulations and Code of Practice
% for Research Degree Programmes and that it has not been submitted for any
% other academic award. Except where indicated by specific reference in the
% text, the work is the candidate's own work. Work done in collaboration with,
% or with the assistance of, others, is indicated as such. Any views expressed
% in the dissertation are those of the author.
%
% SIGNED: .............................................................
% DATE:..........................
%
\chapter*{Author's declaration}
\begin{SingleSpace}
\begin{quote}
\initial{I} declare that the work in this dissertation was carried out in accordance with the requirements of  the University's Regulations and Code of Practice for Research Degree Programmes and that it  has not been submitted for any other academic award. Except where indicated by specific  reference in the text, the work is the candidate's own work. Work done in collaboration with, or with the assistance of, others, is indicated as such. Any views expressed in the dissertation are those of the author.

\vspace{1.5cm}
\noindent
\hspace{-0.75cm}\textsc{SIGNED: .................................................... DATE: ..........................................}
\end{quote}
\end{SingleSpace}
\clearpage

==> frontmatter/dedication.tex <==
%
% file: dedication.tex
% author: V?ctor Bre?a-Medina
% description: Contains the text for thesis dedication
%

\chapter*{Dedication and acknowledgements}
\begin{SingleSpace}
\initial{H}ere goes the dedication.
\end{SingleSpace}
\clearpage

==> references_old.tex <==
@article{wang2020double,
  title={Double-Hard Debias: Tailoring Word Embeddings for Gender Bias Mitigation},
  author={Wang, Tianlu and Lin, Xi Victoria and Rajani, Nazneen Fatema and McCann, Bryan and Ordonez, Vicente and Xiong, Caiming},
  journal={arXiv preprint arXiv:2005.00965},
  year={2020}
}

@article{zhao2018gender,
  title={Gender bias in coreference resolution: Evaluation and debiasing methods},
  author={Zhao, Jieyu and Wang, Tianlu and Yatskar, Mark and Ordonez, Vicente and Chang, Kai-Wei},
  journal={arXiv preprint arXiv:1804.06876},
  year={2018}
}

@article{kumar2020nurse,
  title={Nurse is closer to woman than surgeon? mitigating gender-biased proximities in word embeddings},
  author={Kumar, Vaibhav and Bhotia, Tenzin Singhay and Kumar, Vaibhav and Chakraborty, Tanmoy},
  journal={Transactions of the Association for Computational Linguistics},
  volume={8},
  pages={486--503},
  year={2020},
  publisher={MIT Press}
}

@article{group_words,
  title={Robustness and Reliability of Gender Bias Assessment in WordEmbeddings: The Role of Base Pairs},
  author={Zhang, Haiyang and Sneyd, Alison and Stevenson, Mark},
  journal={arXiv preprint arXiv:2010.02847},
  year={2020}
}

@article{vargas2020exploring,
  title={Exploring the linear subspace hypothesis in gender bias mitigation},
  author={Vargas, Francisco and Cotterell, Ryan},
  journal={arXiv preprint arXiv:2009.09435},
  year={2020}
}

@article{kim2020intersectional,
  title={Intersectional Bias in Hate Speech and Abusive Language Datasets},
  author={Kim, Jae Yeon and Ortiz, Carlos and Nam, Sarah and Santiago, Sarah and Datta, Vivek},
  journal={arXiv preprint arXiv:2005.05921},
  year={2020}
}

@article{200sentiment,
  title={Examining gender and race bias in two hundred sentiment analysis systems},
  author={Kiritchenko, Svetlana and Mohammad, Saif M},
  journal={arXiv preprint arXiv:1805.04508},
  year={2018}
}

@article{surveyEval,
  title={A Survey of Word Embeddings Evaluation Methods},
  author={Bakarov, Amir},
  journal={arXiv preprint arXiv:1801.09536},
  year={2018}
}

@article{elmo,
  title={Deep contextualized word representations},
  author={Peters, Matthew E and Neumann, Mark and Iyyer, Mohit and Gardner, Matt and Clark, Christopher and Lee, Kenton and Zettlemoyer, Luke},
  journal={arXiv preprint arXiv:1802.05365},
  year={2018}
}

@article{bert,
  title={Bert: Pre-training of deep bidirectional transformers for language understanding},
  author={Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  journal={arXiv preprint arXiv:1810.04805},
  year={2018}
}

@inproceedings{genderShades,
  title={Gender shades: Intersectional accuracy disparities in commercial gender classification},
  author={Buolamwini, Joy and Gebru, Timnit},
  booktitle={Conference on Fairness, Accountability and Transparency},
  pages={77--91},
  year={2018}
}

@inproceedings{bolukbasi2016man,
  title={Man is to computer programmer as woman is to homemaker? debiasing word embeddings},
  author={Bolukbasi, Tolga and Chang, Kai-Wei and Zou, James Y and Saligrama, Venkatesh and Kalai, Adam T},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4349--4357},
  year={2016}
}

@inproceedings{ekstrand2018exploring,
  title={Exploring author gender in book rating and recommendation},
  author={Ekstrand, Michael D and Tian, Mucun and Kazi, Mohammed R Imran and Mehrpouyan, Hoda and Kluver, Daniel},
  booktitle={Proceedings of the 12th ACM Conference on Recommender Systems},
  pages={242--250},
  year={2018},
  organization={ACM}
}

@article{angwin2016machine,
  title={Machine bias},
  author={Angwin, Julia and Larson, Jeff and Mattu, Surya and Kirchner, Lauren},
  journal={ProPublica, May},
  volume={23},
  year={2016}
}

@article{100years,
  title={Word embeddings quantify 100 years of gender and ethnic stereotypes},
  author={Garg, Nikhil and Schiebinger, Londa and Jurafsky, Dan and Zou, James},
  journal={Proceedings of the National Academy of Sciences},
  volume={115},
  number={16},
  pages={E3635--E3644},
  year={2018},
  publisher={National Acad Sciences}
}

@article{narayan2017semantics,
  title={Semantics derived automatically from language corpora contain human-like biases},
  author={Caliskan, Aylin and Bryson, Joanna J and Narayanan, Arvind},
  journal={Science},
  volume={356},
  number={6334},
  pages={183--186},
  year={2017},
  publisher={American Association for the Advancement of Science}
}

@article{trust,
  title={Overcoming algorithm aversion: People will use imperfect algorithms if they can (even slightly) modify them},
  author={Dietvorst, Berkeley J and Simmons, Joseph P and Massey, Cade},
  journal={Management Science},
  volume={64},
  number={3},
  pages={1155--1170},
  year={2016},
  publisher={INFORMS}
}

@article{smilkov2016embedding,
  title={Embedding projector: Interactive visualization and interpretation of embeddings},
  author={Smilkov, Daniel and Thorat, Nikhil and Nicholson, Charles and Reif, Emily and Vi{\'e}gas, Fernanda B and Wattenberg, Martin},
  journal={arXiv preprint arXiv:1611.05469},
  year={2016}
}

@article{fairvis,
  title={FairVis: Visual analytics for discovering intersectional bias in machine learning},
  author={Cabrera, {\'A}ngel Alexander and Epperson, Will and Hohman, Fred and Kahng, Minsuk and Morgenstern, Jamie and Chau, Duen Horng},
  journal={arXiv preprint arXiv:1904.05419},
  year={2019}
}

@inproceedings{intersectional,
  title={Assessing social and intersectional biases in contextualized word representations},
  author={Tan, Yi Chern and Celis, L Elisa},
  booktitle={Advances in Neural Information Processing Systems},
  pages={13209--13220},
  year={2019}
}

@article{what_if,
  title={The what-if tool: Interactive probing of machine learning models},
  author={Wexler, James and Pushkarna, Mahima and Bolukbasi, Tolga and Wattenberg, Martin and Vi{\'e}gas, Fernanda and Wilson, Jimbo},
  journal={IEEE transactions on visualization and computer graphics},
  volume={26},
  number={1},
  pages={56--65},
  year={2019},
  publisher={IEEE}
}

@article{fairsight,
  title={Fairsight: Visual analytics for fairness in decision making},
  author={Ahn, Yongsu and Lin, Yu-Ru},
  journal={IEEE transactions on visualization and computer graphics},
  volume={26},
  number={1},
  pages={1086--1095},
  year={2019},
  publisher={IEEE}
}

@article{disability,
  title={Unintended machine learning biases as social barriers for persons with disabilitiess},
  author={Hutchinson, Ben and Prabhakaran, Vinodkumar and Denton, Emily and Webster, Kellie and Zhong, Yu and Denuyl, Stephen},
  journal={ACM SIGACCESS Accessibility and Computing},
  number={125},
  pages={1--1},
  year={2020},
  publisher={ACM New York, NY, USA}
}

@inproceedings{wang2019gender,
  title={Gender bias in contextualized word embeddings},
  author={Wang, Tianlu and Zhao, Jieyu and Yatskar, Mark and Cotterell, Ryan and Ordonez, Vicente and Chang, Kai-Wei},
  booktitle={North American Chapter of the Association for Computational Linguistics (NAACL)},
  year={2019}
}

@inproceedings{glove,
  title={Glove: Global vectors for word representation},
  author={Pennington, Jeffrey and Socher, Richard and Manning, Christopher D},
  booktitle={Proceedings of the 2014 conference on empirical methods in natural language processing (EMNLP)},
  pages={1532--1543},
  year={2014}
}

@inproceedings{mikolov2013distributed,
  title={Distributed representations of words and phrases and their compositionality},
  author={Mikolov, Tomas and Sutskever, Ilya and Chen, Kai and Corrado, Greg S and Dean, Jeff},
  booktitle={Advances in neural information processing systems},
  pages={3111--3119},
  year={2013}
}

@inproceedings{fr_es,
  title={Examining Gender Bias in Languages with Grammatical Gender},
  author={Zhou, Pei and Shi, Weijia and Zhao, Jieyu and Huang, Kuan-Hao and Chen, Muhao and Cotterell, Ryan and Chang, Kai-Wei},
  booktitle={Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP)},
  pages={5279--5287},
  year={2019}
}

@inproceedings{hindi,
  title={Debiasing Gender biased Hindi Words with Word-embedding},
  author={Pujari, Arun K and Mittal, Ansh and Padhi, Anshuman and Jain, Anshul and Jadon, Mukesh and Kumar, Vikas},
  booktitle={Proceedings of the 2019 2nd International Conference on Algorithms, Computing and Artificial Intelligence},
  pages={450--456},
  year={2019}
}

@inproceedings{german,
  title={Bias in word embeddings},
  author={Papakyriakopoulos, Orestis and Hegelich, Simon and Serrano, Juan Carlos Medina and Marco, Fabienne},
  booktitle={Proceedings of the 2020 Conference on Fairness, Accountability, and Transparency},
  pages={446--457},
  year={2020}
}

@book{intersectionality_book,
  title={Intersectionality},
  author={Collins, Patricia Hill and Bilge, Sirma},
  year={2020},
  publisher={John Wiley \& Sons}
}

@article{rozado2020wide,
  title={Wide range screening of algorithmic bias in word embedding models using large sentiment lexicons reveals underreported bias types},
  author={Rozado, David},
  journal={PloS one},
  volume={15},
  number={4},
  pages={e0231189},
  year={2020},
  publisher={Public Library of Science San Francisco, CA USA}
}

@article{parasol,
  title={Parasol: an open source, interactive parallel coordinates library for multi-objective decision making},
  author={Raseman, William J and Jacobson, Joshuah and Kasprzyk, Joseph R},
  journal={Environmental modelling \& software},
  volume={116},
  pages={153--163},
  year={2019},
  publisher={Elsevier}
}

@article{dataContextMap,
  title={The data context map: Fusing data and attributes into a unified display},
  author={Cheng, Shenghui and Mueller, Klaus},
  journal={IEEE transactions on visualization and computer graphics},
  volume={22},
  number={1},
  pages={121--130},
  year={2015},
  publisher={IEEE}
}

@inproceedings{bios,
  title={Bias in bios: A case study of semantic representation bias in a high-stakes setting},
  author={De-Arteaga, Maria and Romanov, Alexey and Wallach, Hanna and Chayes, Jennifer and Borgs, Christian and Chouldechova, Alexandra and Geyik, Sahin and Kenthapadi, Krishnaram and Kalai, Adam Tauman},
  booktitle={Proceedings of the Conference on Fairness, Accountability, and Transparency},
  pages={120--128},
  year={2019}
}

@misc{percentile_score,
    author = "{Wikipedia contributors}",
    title = "Percentile rank --- {Wikipedia}{,} The Free Encyclopedia",
    year = "2020",
    url = "https://en.wikipedia.org/w/index.php?title=Percentile_rank&oldid=954713866",
    note = "[Online; accessed 3-October-2020]"
}


@inproceedings{graham2003using,
  title={Using curves to enhance parallel coordinate visualisations},
  author={Graham, Martin and Kennedy, Jessie},
  booktitle={Proceedings on Seventh International Conference on Information Visualization, 2003. IV 2003.},
  pages={10--16},
  year={2003},
  organization={IEEE}
}

@article{iat,
  title={Measuring individual differences in implicit cognition: the implicit association test.},
  author={Greenwald, Anthony G and McGhee, Debbie E and Schwartz, Jordan LK},
  journal={Journal of personality and social psychology},
  volume={74},
  number={6},
  pages={1464},
  year={1998},
  publisher={American Psychological Association}
}

@article{prates2019assessing,
  title={Assessing gender bias in machine translation: a case study with google translate},
  author={Prates, Marcelo OR and Avelar, Pedro H and Lamb, Lu{\'\i}s C},
  journal={Neural Computing and Applications},
  pages={1--19},
  year={2019},
  publisher={Springer}
}

@inproceedings{stanovsky2019evaluating,
  title={Evaluating Gender Bias in Machine Translation},
  author={Stanovsky, Gabriel and Smith, Noah A and Zettlemoyer, Luke},
  booktitle={Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics},
  pages={1679--1684},
  year={2019}
}

@inproceedings{silva,
  title={Silva: Interactively Assessing Machine Learning Fairness Using Causality},
  author={Yan, Jing Nathan and Gu, Ziwei and Lin, Hubert and Rzeszotarski, Jeffrey M},
  booktitle={Proceedings of the 2020 CHI Conference on Human Factors in Computing Systems},
  pages={1--13},
  year={2020}
}

@article{kozlowski2019geometry,
  title={The geometry of culture: Analyzing the meanings of class through word embeddings},
  author={Kozlowski, Austin C and Taddy, Matt and Evans, James A},
  journal={American Sociological Review},
  volume={84},
  number={5},
  pages={905--949},
  year={2019},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{guo2020detecting,
  title={Detecting Emergent Intersectional Biases: Contextualized Word Embeddings Contain a Distribution of Human-like Biases},
  author={Guo, Wei and Caliskan, Aylin},
  journal={arXiv preprint arXiv:2006.03955},
  year={2020}
}

@article{manzini2019black,
  title={Black is to criminal as caucasian is to police: Detecting and removing multiclass bias in word embeddings},
  author={Manzini, Thomas and Lim, Yao Chong and Tsvetkov, Yulia and Black, Alan W},
  journal={arXiv preprint arXiv:1904.04047},
  year={2019}
}

@INPROCEEDINGS{edge_bundling,  author={G. {Palmas} and M. {Bachynskyi} and A. {Oulasvirta} and H. P. {Seidel} and T. {Weinkauf}},  booktitle={2014 IEEE Pacific Visualization Symposium},   title={An Edge-Bundling Layout for Interactive Parallel Coordinates},   year={2014},  volume={},  number={},  pages={57-64},}

@inproceedings{foulds2020intersectional,
  title={An intersectional definition of fairness},
  author={Foulds, James R and Islam, Rashidul and Keya, Kamrun Naher and Pan, Shimei},
  booktitle={2020 IEEE 36th International Conference on Data Engineering (ICDE)},
  pages={1918--1921},
  year={2020},
  organization={IEEE}
}

@article{ghavami2013intersectional,
  title={An intersectional analysis of gender and ethnic stereotypes: Testing three hypotheses},
  author={Ghavami, Negin and Peplau, Letitia Anne},
  journal={Psychology of Women Quarterly},
  volume={37},
  number={1},
  pages={113--127},
  year={2013},
  publisher={Sage Publications Sage CA: Los Angeles, CA}
}

@inproceedings{dev2019attenuating,
  title={Attenuating Bias in Word vectors},
  author={Dev, Sunipa and Phillips, Jeff},
  booktitle={The 22nd International Conference on Artificial Intelligence and Statistics},
  pages={879--887},
  year={2019}
}

@article{miller2019explanation,
  title={Explanation in artificial intelligence: Insights from the social sciences},
  author={Miller, Tim},
  journal={Artificial Intelligence},
  volume={267},
  pages={1--38},
  year={2019},
  publisher={Elsevier}
}

@misc{progressive_rendering,
    author = "{Kai Chang}",
    title= {Progressive Rendering},
    year = {Accessed October 2020},
    note= {Progressive Rendering},
    URL= {http://bl.ocks.org/syntagmatic/raw/3341641/}
}

@inproceedings{inselberg1990parallel,
  title={Parallel coordinates: a tool for visualizing multi-dimensional geometry},
  author={Inselberg, Alfred and Dimsdale, Bernard},
  booktitle={Proc. IEEE Visualization},
  pages={361--378},
  year={1990}
}

@article{arabic,
  title={AraWEAT: Multidimensional Analysis of Biases in Arabic Word Embeddings},
  author={Lauscher, Anne and Takieddin, Rafik and Ponzetto, Simone Paolo and Glava{\v{s}}, Goran},
  journal={arXiv preprint arXiv:2011.01575},
  year={2020}
}

@article{dutch,
  title={Evaluating Bias In Dutch Word Embeddings},
  author={Mulsa, Rodrigo Alejandro Ch{\'a}vez and Spanakis, Gerasimos},
  journal={arXiv preprint arXiv:2011.00244},
  year={2020}
}

@inproceedings{font2019equalizing,
  title={Equalizing Gender Bias in Neural Machine Translation with Word Embeddings Techniques},
  author={Font, Joel Escud{\'e} and Costa-juss{\`a}, Marta R},
  booktitle={Proceedings of the First Workshop on Gender Bias in Natural Language Processing},
  pages={147--154},
  year={2019}
}

@inproceedings{swinger2019biases,
  title={What are the biases in my word embedding?},
  author={Swinger, Nathaniel and De-Arteaga, Maria and Heffernan IV, Neil Thomas and Leiserson, Mark DM and Kalai, Adam Tauman},
  booktitle={Proceedings of the 2019 AAAI/ACM Conference on AI, Ethics, and Society},
  pages={305--311},
  year={2019}
}

@article{crenshaw1989demarginalizing,
  title={Demarginalizing the intersection of race and sex: A black feminist critique of antidiscrimination doctrine, feminist theory and antiracist politics},
  author={Crenshaw, Kimberl{\'e}},
  journal={u. Chi. Legal f.},
  pages={139},
  year={1989},
  publisher={HeinOnline}
}

@article{crenshaw1990mapping,
  title={Mapping the margins: Intersectionality, identity politics, and violence against women of color},
  author={Crenshaw, Kimberle},
  journal={Stan. L. Rev.},
  volume={43},
  pages={1241},
  year={1990},
  publisher={HeinOnline}
}

@book{fleming2018less,
  title={How to be less stupid about race: On racism, white supremacy, and the racial divide},
  author={Fleming, Crystal Marie},
  year={2018},
  publisher={Beacon Press}
}

@book{crenshaw2017intersectionality,
  title={On intersectionality: Essential writings},
  author={Crenshaw, Kimberl{\'e} W},
  year={2017},
  publisher={The New Press}
}

@inproceedings{antoniak2021bad,
  title={Bad Seeds: Evaluating Lexical Methods for Bias Measurement},
  author={Antoniak, Maria and Mimno, David},
  booktitle={Proceedings of ACL},
  year={2021}
}

@article{mehrabi2021survey,
  title={A survey on bias and fairness in machine learning},
  author={Mehrabi, Ninareh and Morstatter, Fred and Saxena, Nripsuta and Lerman, Kristina and Galstyan, Aram},
  journal={ACM Computing Surveys (CSUR)},
  volume={54},
  number={6},
  pages={1--35},
  year={2021},
  publisher={ACM New York, NY, USA}
 } 

@incollection{keim2008visual,
  title={Visual analytics: Definition, process, and challenges},
  author={Keim, Daniel and Andrienko, Gennady and Fekete, Jean-Daniel and G{\"o}rg, Carsten and Kohlhammer, J{\"o}rn and Melan{\c{c}}on, Guy},
  booktitle={Information visualization},
  pages={154--175},
  year={2008},
  publisher={Springer}
}

@article{bellamy2019ai,
  title={AI Fairness 360: An extensible toolkit for detecting and mitigating algorithmic bias},
  author={Bellamy, Rachel KE and Dey, Kuntal and Hind, Michael and Hoffman, Samuel C and Houde, Stephanie and Kannan, Kalapriya and Lohia, Pranay and Martino, Jacquelyn and Mehta, Sameep and Mojsilovi{\'c}, Aleksandra and others},
  journal={IBM Journal of Research and Development},
  volume={63},
  number={4/5},
  pages={4--1},
  year={2019},
  publisher={IBM}
}

@article{kusner2017counterfactual,
  title={Counterfactual fairness},
  author={Kusner, Matt J and Loftus, Joshua R and Russell, Chris and Silva, Ricardo},
  journal={arXiv preprint arXiv:1703.06856},
  year={2017}
}

@inproceedings{ghai2021wordbias,
  title={WordBias: An Interactive Visual Tool for Discovering Intersectional Biases Encoded in Word Embeddings},
  author={Ghai, Bhavya and Hoque, Md Naimul and Mueller, Klaus},
  booktitle={Extended Abstracts of the 2021 CHI Conference on Human Factors in Computing Systems},
  pages={1--7},
  year={2021}
}

@article{bao2021s,
  title={It's COMPASlicated: The Messy Relationship between RAI Datasets and Algorithmic Fairness Benchmarks},
  author={Bao, Michelle and Zhou, Angela and Zottola, Samantha and Brubach, Brian and Desmarais, Sarah and Horowitz, Aaron and Lum, Kristian and Venkatasubramanian, Suresh},
  journal={arXiv preprint arXiv:2106.05498},
  year={2021}
}

@misc{ghai2020measuring,
      title={Measuring Social Biases of Crowd Workers using Counterfactual Queries}, 
      author={Bhavya Ghai and Q. Vera Liao and Yunfeng Zhang and Klaus Mueller},
      year={2020},
      eprint={2004.02028},
      archivePrefix={arXiv},
      primaryClass={cs.HC}
}

@inproceedings{holstein2019improving,
  title={Improving fairness in machine learning systems: What do industry practitioners need?},
  author={Holstein, Kenneth and Wortman Vaughan, Jennifer and Daum{\'e} III, Hal and Dudik, Miro and Wallach, Hanna},
  booktitle={Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems},
  pages={1--16},
  year={2019}
}

@inproceedings{ekstrand,
  title={Exploring author gender in book rating and recommendation},
  author={Ekstrand, Michael D and Tian, Mucun and Kazi, Mohammed R Imran and Mehrpouyan, Hoda and Kluver, Daniel},
  booktitle={Proceedings of the 12th ACM Conference on Recommender Systems},
  pages={242--250},
  year={2018},
  organization={ACM}
}

@article{sweeney2013discrimination,
  title={Discrimination in online ad delivery},
  author={Sweeney, Latanya},
  journal={Queue},
  volume={11},
  number={3},
  pages={10},
  year={2013},
  publisher={ACM}
}

@unpublished{accent,
title= {The Accent Gap},
author = {Drew Harwell},
year = {2018},
note= {The Washington Post},
URL= {https://www.washingtonpost.com/graphics/2018/business/alexa-does-not-understand-your-accent/?noredirect=on&utm_term=.8ca67c7f13b9},
}

@inproceedings{boluk,
  title={Man is to computer programmer as woman is to homemaker? debiasing word embeddings},
  author={Bolukbasi, Tolga and Chang, Kai-Wei and Zou, James Y and Saligrama, Venkatesh and Kalai, Adam T},
  booktitle={Advances in neural information processing systems},
  pages={4349--4357},
  year={2016}
}

@inproceedings{genderShades,
  title={Gender shades: Intersectional accuracy disparities in commercial gender classification},
  author={Buolamwini, Joy and Gebru, Timnit},
  booktitle={Conference on Fairness, Accountability and Transparency},
  pages={77--91},
  year={2018}
}

@article{100word,
  title={Word embeddings quantify 100 years of gender and ethnic stereotypes},
  author={Garg, Nikhil and Schiebinger, Londa and Jurafsky, Dan and Zou, James},
  journal={Proceedings of the National Academy of Sciences},
  volume={115},
  number={16},
  pages={E3635--E3644},
  year={2018},
  publisher={National Acad Sciences}
}

@article{bios,
  title={Bias in Bios: A Case Study of Semantic Representation Bias in a High-Stakes Setting},
  author={De-Arteaga, Maria and Romanov, Alexey and Wallach, Hanna and Chayes, Jennifer and Borgs, Christian and Chouldechova, Alexandra and Geyik, Sahin and Kenthapadi, Krishnaram and Kalai, Adam Tauman},
  journal={arXiv preprint arXiv:1901.09451},
  year={2019}
}

@inproceedings{convnets,
  title={Convnets and imagenet beyond accuracy: Understanding mistakes and uncovering biases},
  author={Stock, Pierre and Cisse, Moustapha},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={498--512},
  year={2018}
}

@article{vision,
  title={Understanding Unequal Gender Classification Accuracy from Face Images},
  author={Muthukumar, Vidya and Pedapati, Tejaswini and Ratha, Nalini and Sattigeri, Prasanna and Wu, Chai-Wah and Kingsbury, Brian and Kumar, Abhishek and Thomas, Samuel and Mojsilovic, Aleksandra and Varshney, Kush R},
  journal={arXiv preprint arXiv:1812.00099},
  year={2018}
}

@inproceedings{ceo,
  title={Unequal representation and gender stereotypes in image search results for occupations},
  author={Kay, Matthew and Matuszek, Cynthia and Munson, Sean A},
  booktitle={Proceedings of the 33rd Annual ACM Conference on Human Factors in Computing Systems},
  pages={3819--3828},
  year={2015},
  organization={ACM}
}

@article{kamiran2012data,
  title={Data preprocessing techniques for classification without discrimination},
  author={Kamiran, Faisal and Calders, Toon},
  journal={Knowledge and Information Systems},
  volume={33},
  number={1},
  pages={1--33},
  year={2012},
  publisher={Springer}
}

@inproceedings{feldman2015certifying,
  title={Certifying and removing disparate impact},
  author={Feldman, Michael and Friedler, Sorelle A and Moeller, John and Scheidegger, Carlos and Venkatasubramanian, Suresh},
  booktitle={proceedings of the 21th ACM SIGKDD international conference on knowledge discovery and data mining},
  pages={259--268},
  year={2015}
}

@inproceedings{kamishima2012fairness,
  title={Fairness-aware classifier with prejudice remover regularizer},
  author={Kamishima, Toshihiro and Akaho, Shotaro and Asoh, Hideki and Sakuma, Jun},
  booktitle={Joint European Conference on Machine Learning and Knowledge Discovery in Databases},
  pages={35--50},
  year={2012},
  organization={Springer}
}

@inproceedings{agarwal2018reductions,
  title={A reductions approach to fair classification},
  author={Agarwal, Alekh and Beygelzimer, Alina and Dud{\'\i}k, Miroslav and Langford, John and Wallach, Hanna},
  booktitle={International Conference on Machine Learning},
  pages={60--69},
  year={2018},
  organization={PMLR}
}

@inproceedings{agarwal2019fair,
  title={Fair regression: Quantitative definitions and reduction-based algorithms},
  author={Agarwal, Alekh and Dud{\'\i}k, Miroslav and Wu, Zhiwei Steven},
  booktitle={International Conference on Machine Learning},
  pages={120--129},
  year={2019},
  organization={PMLR}
}

@article{pleiss2017fairness,
  title={On fairness and calibration},
  author={Pleiss, Geoff and Raghavan, Manish and Wu, Felix and Kleinberg, Jon and Weinberger, Kilian Q},
  journal={arXiv preprint arXiv:1709.02012},
  year={2017}
}

@article{hardt2016equality,
  title={Equality of opportunity in supervised learning},
  author={Hardt, Moritz and Price, Eric and Srebro, Nati},
  journal={Advances in neural information processing systems},
  volume={29},
  pages={3315--3323},
  year={2016}
}

@inproceedings{kamiran2012decision,
  title={Decision theory for discrimination-aware classification},
  author={Kamiran, Faisal and Karim, Asim and Zhang, Xiangliang},
  booktitle={2012 IEEE 12th International Conference on Data Mining},
  pages={924--929},
  year={2012},
  organization={IEEE}
}

@inproceedings{calmon2017optimized,
  title={Optimized pre-processing for discrimination prevention},
  author={Calmon, Flavio P and Wei, Dennis and Vinzamuri, Bhanukiran and Ramamurthy, Karthikeyan Natesan and Varshney, Kush R},
  booktitle={Proceedings of the 31st International Conference on Neural Information Processing Systems},
  pages={3995--4004},
  year={2017}
}

@inproceedings{dwork2018group,
  title={Group fairness under composition},
  author={Dwork, Cynthia and Ilvento, Christina},
  booktitle={Conference on Fairness, Accountability, and Transparency (FAT* 2018)}
}

@article{aif360,
  title={AI Fairness 360: An extensible toolkit for detecting, understanding, and mitigating unwanted algorithmic bias},
  author={Bellamy, Rachel KE and Dey, Kuntal and Hind, Michael and Hoffman, Samuel C and Houde, Stephanie and Kannan, Kalapriya and Lohia, Pranay and Martino, Jacquelyn and Mehta, Sameep and Mojsilovic, Aleksandra and others},
  journal={arXiv},
  year={2018}
}

@article{bechavod2017penalizing,
  title={Penalizing unfairness in binary classification},
  author={Bechavod, Yahav and Ligett, Katrina},
  journal={arXiv preprint arXiv:1707.00044},
  year={2017}
}


@unpublished{kate,
title= {The Trouble with Bias},
author = {Kate Crawford},
year = {2017},
note= {Neural Information Processing Systems 2017 Keynote talk}
}


@unpublished{arvindTalk,
title= {21 Fairness Definitions and Their Politics},
author = {Arvind Narayanan},
year = {2018},
note= {Conference on Fairness, Accountability, and Transparency, NYC}
}

@inproceedings{dwork2012fairness,
  title={Fairness through awareness},
  author={Dwork, Cynthia and Hardt, Moritz and Pitassi, Toniann and Reingold, Omer and Zemel, Richard},
  booktitle={Proceedings of the 3rd innovations in theoretical computer science conference},
  pages={214--226},
  year={2012},
  organization={ACM}
}

@article{mehrabi2020statistical,
  title={Statistical Equity: A Fairness Classification Objective},
  author={Mehrabi, Ninareh and Huang, Yuzhong and Morstatter, Fred},
  journal={arXiv preprint arXiv:2005.07293},
  year={2020}
}

@article{friedler2021possibility,
  title={The (im) possibility of fairness: Different value systems require different mechanisms for fair decision making},
  author={Friedler, Sorelle A and Scheidegger, Carlos and Venkatasubramanian, Suresh},
  journal={Communications of the ACM},
  volume={64},
  number={4},
  pages={136--143},
  year={2021},
  publisher={ACM New York, NY, USA}
}

@article{ding2021retiring,
  title={Retiring Adult: New Datasets for Fair Machine Learning},
  author={Ding, Frances and Hardt, Moritz and Miller, John and Schmidt, Ludwig},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  year={2021}
}

@inproceedings{menon2018cost,
  title={The cost of fairness in binary classification},
  author={Menon, Aditya Krishna and Williamson, Robert C},
  booktitle={Conference on Fairness, Accountability and Transparency},
  pages={107--118},
  year={2018},
  organization={PMLR}
}

@article{wu2021fair,
  title={Fair AutoML},
  author={Wu, Qingyun and Wang, Chi},
  journal={arXiv preprint arXiv:2111.06495},
  year={2021}
}

@inproceedings{kearns2018preventing,
  title={Preventing fairness gerrymandering: Auditing and learning for subgroup fairness},
  author={Kearns, Michael and Neel, Seth and Roth, Aaron and Wu, Zhiwei Steven},
  booktitle={International Conference on Machine Learning},
  pages={2564--2572},
  year={2018},
  organization={PMLR}
}

@article{biswas2021fair,
  title={Fair Preprocessing: Towards Understanding Compositional Fairness of Data Transformers in Machine Learning Pipeline},
  author={Biswas, Sumon and Rajan, Hridesh},
  journal={arXiv preprint arXiv:2106.06054},
  year={2021}
}

@inproceedings{wang2021practical,
  title={Practical Compositional Fairness: Understanding Fairness in Multi-Component Recommender Systems},
  author={Wang, Xuezhi and Thain, Nithum and Sinha, Anu and Prost, Flavien and Chi, Ed H and Chen, Jilin and Beutel, Alex},
  booktitle={Proceedings of the 14th ACM International Conference on Web Search and Data Mining},
  pages={436--444},
  year={2021}
}

@article{bower2017fair,
  title={Fair pipelines},
  author={Bower, Amanda and Kitchen, Sarah N and Niss, Laura and Strauss, Martin J and Vargas, Alexander and Venkatasubramanian, Suresh},
  journal={arXiv preprint arXiv:1707.00391},
  year={2017}
}

@article{martin2021engineering,
  title={Engineering fair machine learning pipelines},
  author={Martin Hirzel, Kiran Kate and Ram, Parikshit},
  journal={target},
  volume={73},
  number={2.2},
  pages={1--028},
  year={2021}
}

@inproceedings{lee2021landscape,
  title={The landscape and gaps in open source fairness toolkits},
  author={Lee, Michelle Seng Ah and Singh, Jat},
  booktitle={Proceedings of the 2021 CHI Conference on Human Factors in Computing Systems},
  pages={1--13},
  year={2021}
}

@article{emelianov2019price,
  title={The price of local fairness in multistage selection},
  author={Emelianov, Vitalii and Arvanitakis, George and Gast, Nicolas and Gummadi, Krishna and Loiseau, Patrick},
  journal={arXiv preprint arXiv:1906.06613},
  year={2019}
}

@article{dwork2020individual,
  title={Individual fairness in pipelines},
  author={Dwork, Cynthia and Ilvento, Christina and Jagadeesan, Meena},
  journal={arXiv preprint arXiv:2004.05167},
  year={2020}
}

@article{berk2017convex,
  title={A convex framework for fair regression},
  author={Berk, Richard and Heidari, Hoda and Jabbari, Shahin and Joseph, Matthew and Kearns, Michael and Morgenstern, Jamie and Neel, Seth and Roth, Aaron},
  journal={arXiv preprint arXiv:1706.02409},
  year={2017}
}

@article{kleinberg2016inherent,
  title={Inherent trade-offs in the fair determination of risk scores},
  author={Kleinberg, Jon and Mullainathan, Sendhil and Raghavan, Manish},
  journal={arXiv preprint arXiv:1609.05807},
  year={2016}
}

@unpublished{arvindTalk,
title= {21 Fairness Definitions and Their Politics},
author = {Arvind Narayanan},
year = {2018},
note= {Conference on Fairness, Accountability, and Transparency, NYC},
URL= {https://www.youtube.com/watch?v=jIXIuYdnyyk},
}

@article{kamiran2012,
  title={Data preprocessing techniques for classification without discrimination},
  author={Kamiran, Faisal and Calders, Toon},
  journal={Knowledge and Information Systems},
  volume={33},
  number={1},
  pages={1--33},
  year={2012},
  publisher={Springer}
}

@inproceedings{kamishima2011,
  title={Fairness-aware learning through regularization approach},
  author={Kamishima, Toshihiro and Akaho, Shotaro and Sakuma, Jun},
  booktitle={Data Mining Workshops (ICDMW), 2011 IEEE 11th International Conference on},
  pages={643--650},
  year={2011},
  organization={IEEE}
}

@article{inprocess,
  title={Learning fair classifiers: A regularization-inspired approach},
  author={Bechavod, Yahav and Ligett, Katrina},
  journal={arXiv preprint arXiv:1707.00044},
  year={2017}
}

@article{zafar2017fairness,
  title={Fairness constraints: Mechanisms for fair classification},
  author={Zafar, Muhammad Bilal and Valera, Isabel and Gomez Rodriguez, Manuel and Gummadi, Krishna P},
  journal={arXiv preprint arXiv:1507.05259},
  year={2017}
}

@article{sweeney2013discrimination,
  title={Discrimination in online ad delivery},
  author={Sweeney, Latanya},
  journal={Queue},
  volume={11},
  number={3},
  pages={10},
  year={2013},
  publisher={ACM}
}

@inproceedings{postProcessing,
  title={Equality of opportunity in supervised learning},
  author={Hardt, Moritz and Price, Eric and Srebro, Nati and others},
  booktitle={Advances in neural information processing systems},
  pages={3315--3323},
  year={2016}
}

@article{processFairness,
  title={Beyond Distributive Fairness in Algorithmic Decision Making: Feature Selection for Procedurally Fair Learning},
  author={Grgic-Hlaca, Nina and Zafar, Muhammad Bilal and Gummadi, Krishna P and Weller, Adrian},
  year={2018}
}

@article{nipsIBM,
  title={Optimized Data Pre-Processing for Discrimination Prevention},
  author={Calmon, Flavio P and Wei, Dennis and Ramamurthy, Karthikeyan Natesan and Varshney, Kush R},
  journal={arXiv preprint arXiv:1704.03354},
  year={2017}
}

@inproceedings{sureshKDD,
  title={Certifying and removing disparate impact},
  author={Feldman, Michael and Friedler, Sorelle A and Moeller, John and Scheidegger, Carlos and Venkatasubramanian, Suresh},
  booktitle={Proceedings of the 21th ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
  pages={259--268},
  year={2015},
  organization={ACM}
}

@article{hajian2013dataModification,
  title={A methodology for direct and indirect discrimination prevention in data mining},
  author={Hajian, Sara and Domingo-Ferrer, Josep},
  journal={IEEE transactions on knowledge and data engineering},
  volume={25},
  number={7},
  pages={1445--1459},
  year={2013},
  publisher={IEEE}
}

@inproceedings{zemel2013learning,
  title={Learning fair representations},
  author={Zemel, Rich and Wu, Yu and Swersky, Kevin and Pitassi, Toni and Dwork, Cynthia},
  booktitle={International Conference on Machine Learning},
  pages={325--333},
  year={2013}
}

@inproceedings{kamiran2009classifying,
  title={Classifying without discriminating},
  author={Kamiran, Faisal and Calders, Toon},
  booktitle={Computer, Control and Communication, 2009. IC4 2009. 2nd International Conference on},
  pages={1--6},
  year={2009},
  organization={IEEE}
}

@misc{germanUCI,
author = {"D. Newman, S. Hettich, C. Blake, and C. Merz"},
year = "1998",
title = {UCI Machine Learning Repository},
url = "https://archive.ics.uci.edu/ml/datasets/statlog+(german+credit+data)",
institution = "University of California, Irvine, School of Information and Computer Sciences" }

@inproceedings{erk2009representing,
  title={Representing words as regions in vector space},
  author={Erk, Katrin},
  booktitle={Proceedings of the Thirteenth Conference on Computational Natural Language Learning},
  pages={57--65},
  year={2009},
  organization={Association for Computational Linguistics}
}
@article{maaten2008visualizing,
  title={Visualizing data using t-SNE},
  author={Maaten, Laurens van der and Hinton, Geoffrey},
  journal={Journal of machine learning research},
  volume={9},
  number={Nov},
  pages={2579--2605},
  year={2008}
}
@inproceedings{hinton1986learning,
  title={Learning distributed representations of concepts},
  author={Hinton, Geoffrey E},
  booktitle={Proceedings of the eighth annual conference of the cognitive science society},
  volume={1},
  pages={12},
  year={1986},
  organization={Amherst, MA}
}
@inproceedings{martins2017mvn,
  title={MVN-Reduce: Dimensionality Reduction for the Visual Analysis of Multivariate Networks},
  author={Martins, Rafael Messias and Kruiger, JF and Minghim, Rosane and Telea, Alexandru C and Kerren, Andreas},
  booktitle={19th EG/VGTC Conference on Visualization (EuroVis' 17), 12-16 June 2017, Barcelona, Spain},
  year={2017},
  organization={Eurographics-European Association for Computer Graphics}
}
@article{bengio2008adaptive,
  title={Adaptive importance sampling to accelerate training of a neural probabilistic language model},
  author={Bengio, Yoshua and Sen{\'e}cal, Jean-S{\'e}bastien},
  journal={IEEE Transactions on Neural Networks},
  volume={19},
  number={4},
  pages={713--722},
  year={2008},
  publisher={IEEE}
}
@inproceedings{morin2005hierarchical,
  title={Hierarchical Probabilistic Neural Network Language Model.},
  author={Morin, Frederic and Bengio, Yoshua},
  booktitle={Aistats},
  volume={5},
  pages={246--252},
  year={2005},
  organization={Citeseer}
}
@inproceedings{mikolov2013linguistic,
  title={Linguistic Regularities in Continuous Space Word Representations.},
  author={Mikolov, Tomas and Yih, Wen-tau and Zweig, Geoffrey},
  booktitle={Hlt-naacl},
  volume={13},
  pages={746--751},
  year={2013}
}
@inproceedings{tsuboi2014neural,
  title={Neural Networks Leverage Corpus-wide Information for Part-of-speech Tagging.},
  author={Tsuboi, Yuta},
  booktitle={EMNLP},
  pages={938--950},
  year={2014}
}
@article{hinton1985learning,
  title={Learning internal representations by back-propagating errors},
  author={Hinton, GE and Rumelhart, DE and Williams, RJ},
  journal={Parallel Distributed Processing: Explorations in the Microstructure of Cognition},
  volume={1},
  year={1985}
}
@inproceedings{raina2009large,
  title={Large-scale deep unsupervised learning using graphics processors},
  author={Raina, Rajat and Madhavan, Anand and Ng, Andrew Y},
  booktitle={Proceedings of the 26th annual international conference on machine learning},
  pages={873--880},
  year={2009},
  organization={ACM}
}
@book{jolliffe2002principal,
  title={Principal component analysis},
  author={Jolliffe, Ian},
  year={2002},
  publisher={Wiley Online Library}
}
@article{mikolov2013efficient,
  title={Efficient estimation of word representations in vector space},
  author={Mikolov, Tomas and Chen, Kai and Corrado, Greg and Dean, Jeffrey},
  journal={arXiv preprint arXiv:1301.3781},
  year={2013}
}
@inproceedings{mikolov2013distributed,
  title={Distributed representations of words and phrases and their compositionality},
  author={Mikolov, Tomas and Sutskever, Ilya and Chen, Kai and Corrado, Greg S and Dean, Jeff},
  booktitle={Advances in neural information processing systems},
  pages={3111--3119},
  year={2013}
}
@book{manning2008introduction,
  title={Introduction to information retrieval},
  author={Manning, Christopher D and Raghavan, Prabhakar and Sch{\"u}tze, Hinrich and others},
  volume={1},
  number={1},
  year={2008},
  publisher={Cambridge university press Cambridge}
}
@inproceedings{mccarthy2004finding,
  title={Finding predominant word senses in untagged text},
  author={McCarthy, Diana and Koeling, Rob and Weeds, Julie and Carroll, John},
  booktitle={Proceedings of the 42nd Annual Meeting on Association for Computational Linguistics},
  pages={279},
  year={2004},
  organization={Association for Computational Linguistics}
}


@inproceedings{le2014distributed,
  title={Distributed representations of sentences and documents},
  author={Le, Quoc and Mikolov, Tomas},
  booktitle={International Conference on Machine Learning},
  pages={1188--1196},
  year={2014}
}
@inproceedings{socher2013recursive,
  title={Recursive deep models for semantic compositionality over a sentiment treebank},
  author={Socher, Richard and Perelygin, Alex and Wu, Jean and Chuang, Jason and Manning, Christopher D and Ng, Andrew and Potts, Christopher},
  booktitle={Proceedings of the 2013 conference on empirical methods in natural language processing},
  pages={1631--1642},
  year={2013}
}
@inproceedings{kenter2015short,
  title={Short text similarity with word embeddings},
  author={Kenter, Tom and De Rijke, Maarten},
  booktitle={Proceedings of the 24th ACM international on conference on information and knowledge management},
  pages={1411--1420},
  year={2015},
  organization={ACM}
}
@article{robertson2009probabilistic,
  title={The probabilistic relevance framework: BM25 and beyond},
  author={Robertson, Stephen and Zaragoza, Hugo and others},
  journal={Foundations and Trends{\textregistered} in Information Retrieval},
  volume={3},
  number={4},
  pages={333--389},
  year={2009},
  publisher={Now Publishers, Inc.}
}
@article{kruskal1964multidimensional,
  title={Multidimensional scaling by optimizing goodness of fit to a nonmetric hypothesis},
  author={Kruskal, Joseph B},
  journal={Psychometrika},
  volume={29},
  number={1},
  pages={1--27},
  year={1964},
  publisher={Springer}
}
@article{rousseeuw1987silhouettes,
  title={Silhouettes: a graphical aid to the interpretation and validation of cluster analysis},
  author={Rousseeuw, Peter J},
  journal={Journal of computational and applied mathematics},
  volume={20},
  pages={53--65},
  year={1987},
  publisher={Elsevier}
}
@article{calinski1974dendrite,
  title={A dendrite method for cluster analysis},
  author={Cali{\'n}ski, Tadeusz and Harabasz, Jerzy},
  journal={Communications in Statistics-theory and Methods},
  volume={3},
  number={1},
  pages={1--27},
  year={1974},
  publisher={Taylor \& Francis}
}

@article{Zhang2015VisualMap,
    title = {{Visual Correlation Analysis of Numerical and Categorical Data on the Correlation Map}},
    year = {2015},
    journal = {IEEE Transactions on Visualization and Computer Graphics},
    author = {Zhang, Zhiyuan and Mcdonnell, Kevin T and Zadok, Erez and Mueller, Klaus},
    number = {2},
    pages = {289--303},
    volume = {21}
}

@inproceedings{Inselberg1990,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Inselberg, Alfred and Dimsdale, Bernard},
booktitle = {1st conference on Visualization '90},
doi = {10.1109/VISUAL.1990.146402},
eprint = {arXiv:1011.1669v3},
isbn = {0-8186-2083-8},
issn = {1098-6596},
pages = {361--378},
pmid = {25246403},
title = {{Parallel Coordinates: a tool for visualizing muti-dimensional geometry}},
url = {http://dl.acm.org/citation.cfm?id=949588},
year = {1990}
}
@book{Pearl2000,
author = {Pearl, Judea},
isbn = {978-0521895606},
publisher = {Cambridge University Press},
title = {{Causality: Models, Reasoning, and Inference}},
year = {2000}
}
@article{Pearl2009,
archivePrefix = {arXiv},
arxivId = {arXiv:1112.1788v3},
author = {Pearl, Judea},
doi = {10.1214/09-SS057},
eprint = {arXiv:1112.1788v3},
isbn = {1935-7516},
issn = {1935-7516},
journal = {Statistics Surveys},
number = {0},
pages = {96--146},
pmid = {25246403},
title = {{Causal inference in statistics: An overview}},
volume = {3},
year = {2009}
}

@book{Spirtes2000,
address = {Cambridge, MA},
author = {Spirtes, Peter and Glymour, Clark and Scheines, Richard},
isbn = {978-0262194402},
keywords = {FCI,PC,SGS},
mendeley-groups = {Causal Inference Algorithms},
mendeley-tags = {FCI,PC,SGS},
publisher = {MIT Press},
title = {{Causation, Prediction, and Search}},
year = {2000}
}

@article{Pearl2001,
author = {Pearl, Judea and Russell, Stuart},
pages = {1--7},
title = {{Bayesian networks}},
year = {2001}
}

@article{Pearl2010AnInference,
    title = {{An Introduction to Causal Inference}},
    year = {2010},
    journal = {The International Journal of Biostatistics},
    author = {Pearl, Judea},
    number = {2},
    pages = {1--62},
    volume = {6},
    isbn = {0049124196},
    doi = {10.2202/1557-4679.1203},
    issn = {1557-4679},
    pmid = {20305706},
    arxivId = {0803973233},
    keywords = {Algorithms, Causality, Confounding Factors (Epidemiology), Humans, Models, Research Design, Statistical}
}
    
@article{Bongers2016StructuralReductions,
    title = {{Structural Causal Models: Cycles, Marginalizations, Exogenous Reparametrizations and Reductions}},
    year = {2016},
    journal = {arXiv},
    author = {Bongers, Stephan and Peters, Jonas and Sch{\"{o}}lkopf, Bernhard and Mooij, Joris M},
    month = {11},
    url = {http://arxiv.org/abs/1611.06221},
    arxivId = {1611.06221},
    keywords = {()}
}

@article{Pearl1995,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Pearl, Judea and Verma, Thomas S.},
doi = {10.1016/S0049-237X(06)80074-1},
eprint = {arXiv:1011.1669v3},
isbn = {1558601651},
issn = {0049237X},
journal = {Studies in Logic and the Foundations of Mathematics},
keywords = {IC},
mendeley-groups = {Causal Inference Algorithms},
mendeley-tags = {IC},
pages = {789--811},
pmid = {25246403},
title = {{A theory of inferred causation}},
volume = {134},
year = {1995}
}
@article{Colombo2014Order-independentLearning,
    title = {{Order-independent constraint-based causal structure learning}},
    year = {2014},
    journal = {Journal of Machine Learning Research},
    author = {Colombo, Diego and Maathuis, Marloes H},
    number = {1},
    pages = {3741--3782},
    volume = {15},
    doi = {papers3://publication/uuid/CC1A353F-4C95-4058-93CC-05855FD6E5E3},
    issn = {15337928},
    arxivId = {1211.3295},
    keywords = {ccd-algorithm, consistency, dependence, directed acyclic graph, fci-algorithm, high-dimensional data, order-, pc-algorithm}
}
@article{pellet2008using,
  title={Using Markov blankets for causal structure learning},
  author={Pellet, Jean-Philippe and Elisseeff, Andr{\'e}},
  journal={Journal of Machine Learning Research},
  volume={9},
  number={Jul},
  pages={1295--1342},
  year={2008}
}


@inproceedings{Dang2015ReactionFlow:Pathways,
    title = {{ReactionFlow: an interactive visualization tool for causality analysis in biological pathways}},
    year = {2015},
    booktitle = {Proceedings of the 5th Symposium on Biological Data Visualization: Part 2},
    author = {Dang, Tuan and Murray, Paul and Aurisano, Jillian and Forbes, Angus},
    number = {Suppl 6},
    volume = {9},
    url = {http://bmcproc.biomedcentral.com/articles/10.1186/1753-6561-9-S6-S6},
    doi = {10.1186/1753-6561-9-S6-S6},
    issn = {1753-6561}
}

@article{Elmqvist2004AnimatedGeometry,
    title = {{Animated visualization of causal relations through growing 2D geometry}},
    year = {2004},
    journal = {Information Visualization},
    author = {Elmqvist, Niklas and Tsigas, Philippas},
    number = {3},
    pages = {154--172},
    volume = {3},
    url = {http://dl.acm.org/citation.cfm?id=1039751.1039754},
    isbn = {1473-8716},
    doi = {10.1057/palgrave.ivs.9500074},
    issn = {1473-8716},
    keywords = {causal relations, interactive animation}
}

@article{Wang2016,
    author = {Wang, Jun and Mueller, Klaus},
    doi = {10.1109/TVCG.2015.2467931},
    isbn = {1077-2626},
    issn = {10772626},
    journal = {IEEE Transactions on Visualization and Computer Graphics},
    keywords = {Correlation,Inference algorithms,Layout,Linear regression,Optimization,Visualization},
    number = {1},
    pages = {230--239},
    pmid = {26529703},
    title = {{The Visual Causality Analyst: An Interactive Interface for Causal Reasoning}},
    volume = {22},
    year = {2016}
}

@inproceedings{Wang2017,
address = {Phoenix, AZ},
author = {Wang, Jun and Mueller, Klaus},
booktitle = {IEEE Conference Visual Analytics Science and Technology (VAST)},
title = {{Visual Causality Analysis Made Practical}},
year = {2017}
}

@article{Kadaba2007,
author = {Kadaba, Nivedita R. and Irani, Pourang P. and Leboe, Jason},
doi = {10.1109/TVCG.2007.70528},
file = {:D$\backslash$:/WorkSpace/Mendeley/Visualizing causal semantics using animations - IEEE Transactions on Visualization and Computer Graphics - 2007.pdf:pdf},
isbn = {1077-2626},
issn = {10772626},
journal = {IEEE Transactions on Visualization and Computer Graphics},
keywords = {Animated graphs,Causality,Graph semantics,Perception,Semantics,Visualization,Visualizing cause and effect},
number = {6},
pages = {1254--1261},
pmid = {17968072},
title = {{Visualizing causal semantics using animations}},
volume = {13},
year = {2007}
}

@article{Burnham2004,
abstract = {AICc justification},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Burnham, K. P. and Anderson, R.P.},
doi = {10.1177/0049124104268644},
eprint = {arXiv:1011.1669v3},
isbn = {00491241 (ISSN)},
issn = {0049-1241},
journal = {Sociological Methods {\&} Research},
number = {2},
pages = {261--304},
pmid = {21699709},
title = {{Multimodel Inference: Understanding AIC and BIC in Model Selection}},
volume = {33},
year = {2004}
}

@article{Siirtola1997,
doi = {10.1057/palgrave.ivs.9500086},
isbn = {1473-8716},
issn = {14738724},
journal = {Information Visualization},
keywords = {Multi-dimensional data visualization,barycenter heuristic,cluster analysis,the reorderable matrix,user interface},
number = {1},
pages = {32--48},
title = {{Constructing and reconstructing the reorderable matrix}},
volume = {4},
year = {1997}
}

@article{dressel2018accuracy,
  title={The accuracy, fairness, and limits of predicting recidivism},
  author={Dressel, Julia and Farid, Hany},
  journal={Science Advances},
  volume={4},
  number={1},
  pages={eaao5580},
  year={2018},
  publisher={American Association for the Advancement of Science}
}

@article{angwin2016machine,
  title={Machine bias},
  author={Angwin, Julia and Larson, Jeff and Mattu, Surya and Kirchner, Lauren},
  journal={ProPublica, May},
  volume={23},
  year={2016}
}

@book{hellman2008discrimination,
  title={When is discrimination wrong?},
  author={Hellman, Deborah},
  year={2008},
  publisher={Harvard University Press}
}

@article{marshall2018automating,
  title={Automating Inequality. How High-Tech Tools Profile, Police and Punish the Poor},
  author={Marshall, Robert},
  journal={Alternate Routes: A Journal of Critical Social Research},
  year={2018}
}

@inproceedings{kusner2017counterfactual,
  title={Counterfactual fairness},
  author={Kusner, Matt J and Loftus, Joshua and Russell, Chris and Silva, Ricardo},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4069--4079},
  year={2017}
}

@article{calinski1974dendrite,
  title={A dendrite method for cluster analysis},
  author={Cali{\'n}ski, Tadeusz and Harabasz, Jerzy},
  journal={Communications in Statistics-theory and Methods},
  volume={3},
  number={1},
  pages={1--27},
  year={1974},
  publisher={Taylor \& Francis}
}

@book{rousseeuw1990finding,
  title={Finding groups in data},
  author={Rousseeuw, Peter J and Kaufman, L},
  year={1990},
  publisher={Wiley Online Library Hoboken}
}

@article{kullback1951information,
  title={On information and sufficiency},
  author={Kullback, Solomon and Leibler, Richard A},
  journal={The annals of mathematical statistics},
  volume={22},
  number={1},
  pages={79--86},
  year={1951},
  publisher={JSTOR}
}

@article{deb2002fast,
  title={A fast and elitist multiobjective genetic algorithm: NSGA-II},
  author={Deb, Kalyanmoy and Pratap, Amrit and Agarwal, Sameer and Meyarivan, TAMT},
  journal={IEEE transactions on evolutionary computation},
  volume={6},
  number={2},
  pages={182--197},
  year={2002},
  publisher={IEEE}
}

@inproceedings{jain2013improved,
  title={An improved adaptive approach for elitist nondominated sorting genetic algorithm for many-objective optimization},
  author={Jain, Himanshu and Deb, Kalyanmoy},
  booktitle={International Conference on Evolutionary Multi-Criterion Optimization},
  pages={307--321},
  year={2013},
  organization={Springer}
}


@inproceedings{qu2013psogd,
  title={PSOGD: A new method for graph drawing},
  author={Qu, Jianhua and Song, Yi and Bressan, St{\'e}phane},
  booktitle={Data Engineering Workshops (ICDEW), 2013 IEEE 29th International Conference on},
  pages={229--235},
  year={2013},
  organization={IEEE}
}
	
@inproceedings{aggarwal2001surprising,
  title={On the surprising behavior of distance metrics in high dimensional space},
  author={Aggarwal, Charu C and Hinneburg, Alexander and Keim, Daniel A},
  booktitle={International Conference on Database Theory},
  pages={420--434},
  year={2001},
  organization={Springer}
}

@book{kruskal1978multidimensional,
  title={Multidimensional scaling},
  author={Kruskal, Joseph B and Wish, Myron},
  volume={11},
  year={1978},
  publisher={Sage}
}

@misc{lee2014pyswarm,
  title={pyswarm: Particle swarm optimization (PSO) with constraint support},
  author={Lee, Abraham},
  howpublished={\url{https://pythonhosted.org/pyswarm/}},
  year={2014}
}

@misc{batagelj2006pajek,
  title={Pajek datasets},
  author={Batagelj, Vladimir and Mrvar, Andrej},
  howpublished={\url{http://vlado.fmf.uni-lj.si/pub/networks/data/sport/football.htm}},
  year={2006}
}

@article{angwin2016machine,
  title={Machine bias},
  author={Angwin, Julia and Larson, Jeff and Mattu, Surya and Kirchner, Lauren},
  journal={ProPublica, May},
  volume={23},
  year={2016}
}

@article{youtube,
  title={YouTube Extremism and the Long Tail},
  author={CONOR FRIEDERSDOR},
  journal={The Atlantic},
  howpublished={\url{https://www.theatlantic.com/politics/archive/2018/03/youtube-extremism-and-the-long-tail/555350/}},
  year={2018}
}

@article{translate,
  title={Google Translate},
  journal={Wikipedia},
  howpublished={\url{https://en.wikipedia.org/wiki/Google_Translate}},
  year={2018}
}

@article{translate2,
  title={Google Translate’s gender bias pairs “he” with “hardworking” and “she” with lazy, and other examples},
  journal={Quartz},
  author={Nikhil Sonnad},
  howpublished={\url{https://qz.com/1141122/google-translates-gender-bias-pairs-he-with-hardworking-and-she-with-lazy-and-other-examples/}},
  year={2017}
}

@inproceedings{kay2015unequal,
  title={Unequal representation and gender stereotypes in image search results for occupations},
  author={Kay, Matthew and Matuszek, Cynthia and Munson, Sean A},
  booktitle={Proceedings of the 33rd Annual ACM Conference on Human Factors in Computing Systems},
  pages={3819--3828},
  year={2015},
  organization={ACM}
}

@article{amazonPrime,
  title={Amazon same-day delivery less likely in black areas, report says},
  journal={USA Today},
  author={Elizabeth Weise},
  howpublished={\url{https://www.usatoday.com/story/tech/news/2016/04/22/amazon-same-day-delivery-less-likely-black-areas-report-says/83345684/}},
  year={2016}
}

@article{amazonPrime,
  title={Amazon same-day delivery less likely in black areas, report says},
  author={Elizabeth Weise},
  journal={USA Today},
  howpublished={\url{https://www.usatoday.com/story/tech/news/2016/04/22/amazon-same-day-delivery-less-likely-black-areas-report-says/83345684/}},
  year={2016}
}


@article{facebookNews,
  title={How Facebook Biases Your News Feed},
  author={Nelson Granados},
  journal={Forbes},
  howpublished={\url{https://www.forbes.com/sites/nelsongranados/2016/06/30/how-facebook-biases-your-news-feed/#1c0734b81d51}},
  year={2016}
}

@article{accentBias,
  title={The Accent Bias},
  author={Johnson},
  journal={The Washington Post},
  howpublished={\url{https://www.washingtonpost.com/graphics/2018/business/alexa-does-not-understand-your-accent/?noredirect=on&utm_term=.d19fdbb6f168}},
  year={2018}
}

@article{kateNIPS,
  title={The Trouble with Bias},
  author={Kate Crawford},
  journal={NIPS 2017 Keynote},
  howpublished={\url{https://www.youtube.com/watch?v=fMym_BKWQzk}},
  year={2017}
}

@article{amazonBloomberg,
  title={Amazon Doesn’t Consider the Race of Its Customers. Should It?},
  author={David Ingold, Spencer Soper},
  journal={Bloomberg},
  howpublished={\url{https://www.bloomberg.com/graphics/2016-amazon-same-day/}},
  year={2016}
}

@article{lawmakers,
  title={LAWMAKERS CAN'T IGNORE FACIAL RECOGNITION'S BIAS ANYMORE},
  author={BRIAN BARRETT},
  journal={Wired},
  howpublished={\url{https://www.wired.com/story/amazon-facial-recognition-congress-bias-law-enforcement/}},
  year={2018}
}

@article{AIWinter,
  title={AI Winter},
  journal={Wikipedia},
  howpublished={\url{https://en.wikipedia.org/wiki/AI_winter}},
  year={2018}
}

@article{HumanAI,
  title={How to Make A.I. That’s Good for People},
  author={Fei Fei Li},
  journal={New York Times},
  howpublished={\url{https://www.nytimes.com/2018/03/07/opinion/artificial-intelligence-human.html}},
  year={2018}
}

@article{sweeney2013discrimination,
  title={Discrimination in online ad delivery},
  author={Sweeney, Latanya},
  journal={Queue},
  volume={11},
  number={3},
  pages={10},
  year={2013},
  publisher={ACM}
}

@inproceedings{buolamwini2018gender,
  title={Gender shades: Intersectional accuracy disparities in commercial gender classification},
  author={Buolamwini, Joy and Gebru, Timnit},
  booktitle={Conference on Fairness, Accountability and Transparency},
  pages={77--91},
  year={2018}
}

@article{friedler2016possibility,
  title={On the (im) possibility of fairness},
  author={Friedler, Sorelle A and Scheidegger, Carlos and Venkatasubramanian, Suresh},
  journal={arXiv preprint arXiv:1609.07236},
  year={2016}
}
@article{kleinberg2016inherent,
  title={Inherent trade-offs in the fair determination of risk scores},
  author={Kleinberg, Jon and Mullainathan, Sendhil and Raghavan, Manish},
  journal={arXiv preprint arXiv:1609.05807},
  year={2016}
}

@inproceedings{dwork2012fairness,
  title={Fairness through awareness},
  author={Dwork, Cynthia and Hardt, Moritz and Pitassi, Toniann and Reingold, Omer and Zemel, Richard},
  booktitle={Proceedings of the 3rd innovations in theoretical computer science conference},
  pages={214--226},
  year={2012},
  organization={ACM}
}

@article{zhao2017men,
  title={Men also like shopping: Reducing gender bias amplification using corpus-level constraints},
  author={Zhao, Jieyu and Wang, Tianlu and Yatskar, Mark and Ordonez, Vicente and Chang, Kai-Wei},
  journal={arXiv preprint arXiv:1707.09457},
  year={2017}
}
@article{greenwald1998measuring,
  title={Measuring individual differences in implicit cognition: the implicit association test.},
  author={Greenwald, Anthony G and McGhee, Debbie E and Schwartz, Jordan LK},
  journal={Journal of personality and social psychology},
  volume={74},
  number={6},
  pages={1464},
  year={1998},
  publisher={American Psychological Association}
}

@inproceedings{bolukbasi2016man,
  title={Man is to computer programmer as woman is to homemaker? debiasing word embeddings},
  author={Bolukbasi, Tolga and Chang, Kai-Wei and Zou, James Y and Saligrama, Venkatesh and Kalai, Adam T},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4349--4357},
  year={2016}
}

@article{loftus2018causal,
  title={Causal Reasoning for Algorithmic Fairness},
  author={Loftus, Joshua R and Russell, Chris and Kusner, Matt J and Silva, Ricardo},
  journal={arXiv preprint arXiv:1805.05859},
  year={2018}
}

@article{miconi2017impossibility,
  title={The impossibility of “fairness”: a generalized impossibility result for decisions},
  author={Miconi, Thomas},
  journal={arXiv preprint arXiv:1707.01195},
  year={2017}
}

@article{ghai2020explainable,
  title={Explainable Active Learning (XAL): An Empirical Study of How Local Explanations Impact Annotator Experience},
  author={Ghai, Bhavya and Liao, Q Vera and Zhang, Yunfeng and Bellamy, Rachel and Mueller, Klaus},
  journal={arXiv preprint arXiv:2001.09219},
  year={2020}
}


@article{fairvis,
  title={FairVis: Visual analytics for discovering intersectional bias in machine learning},
  author={Cabrera, {\'A}ngel Alexander and Epperson, Will and Hohman, Fred and Kahng, Minsuk and Morgenstern, Jamie and Chau, Duen Horng},
  journal={arXiv},
  year={2019}
}

@article{fairsight,
  title={Fairsight: Visual analytics for fairness in decision making},
  author={Ahn, Yongsu and Lin, Yu-Ru},
  journal={IEEE transactions on visualization and computer graphics},
  volume={26},
  number={1},
  pages={1086--1095},
  year={2019},
  publisher={IEEE}
}

@inproceedings{drozdal2020trust,
  title={Trust in AutoML: exploring information needs for establishing trust in automated machine learning systems},
  author={Drozdal, Jaimie and Weisz, Justin and Wang, Dakuo and Dass, Gaurav and Yao, Bingsheng and Zhao, Changruo and Muller, Michael and Ju, Lin and Su, Hui},
  booktitle={International Conference on Intelligent User Interfaces},
  year={2020}
}

@article{trust2,
  title={Initial trust formation in new organizational relationships},
  author={McKnight, D Harrison and Cummings, Larry L and Chervany, Norman L},
  journal={Academy of Management Review},
  volume={23},
  number={3},
  pages={473--490},
  year={1998},
  publisher={Academy of Management Briarcliff Manor, NY 10510}
}

@article{trust1,
  title={Developing and validating trust measures for e-commerce: An integrative typology},
  author={McKnight, D Harrison and Choudhury, Vivek and Kacmar, Charles},
  journal={Information Systems Research},
  year={2002},
  publisher={INFORMS}
}

@inproceedings{madsen2000measuring,
  title={Measuring human-computer trust},
  author={Madsen, Maria and Gregor, Shirley},
  booktitle={11th australasian conference on information systems},
  year={2000}
}

@inproceedings{cai2019effects,
  title={The effects of example-based explanations in a machine learning interface},
  author={Cai, Carrie J and Jongejan, Jonas and Holbrook, Jess},
  booktitle={Proceedings of the 24th International Conference on Intelligent User Interfaces},
  year={2019}
}

@article{XAL,
  title={Explainable active learning (xal) toward AI explanations as interfaces for machine teachers},
  author={Ghai, Bhavya and Liao, Q Vera and Zhang, Yunfeng and Bellamy, Rachel and Mueller, Klaus},
  journal={Proc. of the ACM on Human-Computer Interaction},
  number={CSCW3},
  year={2021}
}


@article{sus,
  title={SUS-A quick and dirty usability scale},
  author={Brooke, John and others},
  journal={Usability evaluation in industry},
  volume={189},
  number={194},
  pages={4--7},
  year={1996},
  publisher={London--}
}

@incollection{nasa_tlx,
  title={Development of NASA-TLX (Task Load Index): Results of empirical and theoretical research},
  author={Hart, Sandra G and Staveland, Lowell E},
  booktitle={Advances in Psychology},
  volume={52},
  pages={139--183},
  year={1988}
}

@article{fci,
  title={An algorithm for causal inference in the presence of latent variables and selection bias},
  author={Spirtes, Peter and Meek, Christopher and Richardson, Thomas},
  journal={Computation, causation, and discovery},
  volume={21},
  pages={1--252},
  year={1999}
}

@article{challenges,
  title={Challenges and opportunities with causal Discovery Algorithms: Application to Alzheimer’s pathophysiology},
  author={Shen, Xinpeng and Ma, Sisi and Vemuri, Prashanthi and Simon, Gyorgy},
  journal={Scientific Reports},
  year={2020},
  publisher={Nature Publishing Group}
}

@article{aif360,
  title={AI Fairness 360: An extensible toolkit for detecting, understanding, and mitigating unwanted algorithmic bias},
  author={Bellamy, Rachel KE and Dey, Kuntal and Hind, Michael and others},
  journal={arXiv},
  year={2018}
}

@article{aif360_all_authors,
  title={AI Fairness 360: An extensible toolkit for detecting, understanding, and mitigating unwanted algorithmic bias},
  author={Bellamy, Rachel KE and Dey, Kuntal and Hind, Michael and Hoffman, Samuel C and Houde, Stephanie and Kannan, Kalapriya and Lohia, Pranay and Martino, Jacquelyn and Mehta, Sameep and Mojsilovic, Aleksandra and others},
  journal={arXiv},
  year={2018}
}

@article{bechavod2017penalizing,
  title={Penalizing unfairness in binary classification},
  author={Bechavod, Yahav and Ligett, Katrina},
  journal={arXiv preprint arXiv:1707.00044},
  year={2017}
}

@inproceedings{dwork2012fairness,
  title={Fairness through awareness},
  author={Dwork, Cynthia and Hardt, Moritz and Pitassi, Toniann and Reingold, Omer and Zemel, Richard},
  booktitle={Proceedings of the 3rd innovations in theoretical computer science conference},
  pages={214--226},
  year={2012},
  organization={ACM}
}

@inproceedings{dwork2018group,
  title={Group fairness under composition},
  author={Dwork, Cynthia and Ilvento, Christina},
  booktitle={Conference on Fairness, Accountability, and Transparency (FAT* 2018)}
}

@article{lohia2018bias,
  title={Bias mitigation post-processing for individual and group fairness},
  author={Lohia, Pranay K and Ramamurthy, Karthikeyan Natesan and Bhide, Manish and Saha, Diptikalyan and Varshney, Kush R and Puri, Ruchir},
  journal={arXiv preprint arXiv:1812.06135},
  year={2018}
}

@article{saxena2018fairness,
  title={How Do Fairness Definitions Fare? Examining Public Attitudes Towards Algorithmic Definitions of Fairness},
  author={Saxena, Nripsuta and Huang, Karen and DeFilippis, Evan and Radanovic, Goran and Parkes, David and Liu, Yang},
  journal={arXiv},
  year={2018}
}

@article{hohman2018visual,
  title={Visual analytics in deep learning: An interrogative survey for the next frontiers},
  author={Hohman, Fred Matthew and Kahng, Minsuk and Pienta, Robert and Chau, Duen Horng},
  journal={IEEE transactions on visualization and computer graphics},
  year={2018},
  publisher={IEEE}
}

@article{dietvorst2016overcoming,
  title={Overcoming algorithm aversion: People will use imperfect algorithms if they can (even slightly) modify them},
  author={Dietvorst, Berkeley J and Simmons, Joseph P and Massey, Cade},
  journal={Management Science},
  year={2016},
  publisher={INFORMS}
}

@article{gajane2017formalizing,
  title={On formalizing fairness in prediction with machine learning},
  author={Gajane, Pratik and Pechenizkiy, Mykola},
  journal={arXiv preprint arXiv:1710.03184},
  year={2017}
}

@article{kleinberg2016inherent,
  title={Inherent trade-offs in the fair determination of risk scores},
  author={Kleinberg, Jon and Mullainathan, Sendhil and Raghavan, Manish},
  journal={arXiv},
  year={2016}
}

@inproceedings{obermeyer2019dissecting,
  title={Dissecting Racial Bias in an Algorithm that Guides Health Decisions for 70 Million People},
  author={Obermeyer, Ziad and Mullainathan, Sendhil},
  booktitle={Proceedings of the Conference on Fairness, Accountability, and Transparency},
  pages={89--89},
  year={2019},
  organization={ACM}
}

@article{brennan2009evaluating,
  title={Evaluating the predictive validity of the COMPAS risk and needs assessment system},
  author={Brennan, Tim and Dieterich, William and Ehret, Beate},
  journal={Criminal Justice and Behavior},
  volume={36},
  number={1},
  pages={21--40},
  year={2009},
  publisher={Sage Publications Sage CA: Los Angeles, CA}
}

@misc{mahoney2007method,
  title={Method and system for loan origination and underwriting},
  author={Mahoney, John F and Mohen, James M},
  year={2007},
  month=oct # "~23",
  publisher={Google Patents},
  note={US Patent 7,287,008}
}

@inproceedings{holstein2019improving,
  title={Improving fairness in machine learning systems: What do industry practitioners need?},
  author={Holstein, Kenneth and Wortman Vaughan, Jennifer and Daum{\'e} III, Hal and Dudik, Miro and Wallach, Hanna},
  booktitle={Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems}
}

@inproceedings{ceo,
  title={Unequal representation and gender stereotypes in image search results for occupations},
  author={Kay, Matthew and Matuszek, Cynthia and Munson, Sean A},
  booktitle={Proceedings of the 33rd Annual ACM Conference on Human Factors in Computing Systems},
  pages={3819--3828},
  year={2015},
  organization={ACM}
}

@unpublished{amazon,
title= {Amazon scraps secret AI recruiting tool that showed bias against women},
author = {Jeffrey Dastin},
year = {2018},
note= {Reuters},
URL= {https://www.reuters.com/article/us-amazon-com-jobs-automation-insight/amazon-scraps-secret-ai-recruiting-tool-that-showed-bias-against-women-idUSKCN1MK08G},
}


@unpublished{BlackGorilla,
title= {Google engineer apologizes after Photos app tags two black people as gorillas},
author = {Loren Grush},
year = {2015},
note= {The Verge},
URL= {https://www.theverge.com/2015/7/1/8880363/google-apologizes-photos-app-tags-two-black-people-gorillas},
}

@unpublished{amazonHiringSexist,
title= {Amazon scraps secret AI recruiting tool that showed bias against women},
author = {Jeffrey Dastin},
year = {2018},
note= {Reuters},
URL= {https://www.reuters.com/article/us-amazon-com-jobs-automation-insight/amazon-scraps-secret-ai-recruiting-tool-that-showed-bias-against-women-idUSKCN1MK08G},
}


@inproceedings{genderShades,
  title={Gender shades: Intersectional accuracy disparities in commercial gender classification},
  author={Buolamwini, Joy and Gebru, Timnit},
  booktitle={Conference on Fairness, Accountability and Transparency},
  pages={77--91},
  year={2018}
}

@article{100word,
  title={Word embeddings quantify 100 years of gender and ethnic stereotypes},
  author={Garg, Nikhil and Schiebinger, Londa and Jurafsky, Dan and Zou, James},
  journal={Proceedings of the National Academy of Sciences},
  volume={115},
  number={16},
  pages={E3635--E3644},
  year={2018},
  publisher={National Acad Sciences}
}

@unpublished{kate,
title= {The Trouble with Bias},
author = {Kate Crawford},
year = {2017},
note= {Neural Information Processing Systems 2017 Keynote talk}
}

@unpublished{realaidanger,
title= {Forget Killer Robots—Bias Is the Real AI Danger},
author = {Will Knight},
year = {2018},
note= {MIT Technology Review},
URL= {https://www.technologyreview.com/s/608986/forget-killer-robotsbias-is-the-real-ai-danger/},
}

@unpublished{accent,
title= {The Accent Gap},
author = {Drew Harwell},
year = {2018},
note= {The Washington Post},
URL= {https://www.washingtonpost.com/graphics/2018/business/alexa-does-not-understand-your-accent/?noredirect=on&utm_term=.8ca67c7f13b9},
}

@inproceedings{convnets,
  title={Convnets and imagenet beyond accuracy: Understanding mistakes and uncovering biases},
  author={Stock, Pierre and Cisse, Moustapha},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={498--512},
  year={2018}
}

@article{vision,
  title={Understanding Unequal Gender Classification Accuracy from Face Images},
  author={Muthukumar, Vidya and Pedapati, Tejaswini and Ratha, Nalini and Sattigeri, Prasanna and Wu, Chai-Wah and Kingsbury, Brian and Kumar, Abhishek and Thomas, Samuel and Mojsilovic, Aleksandra and Varshney, Kush R},
  journal={arXiv preprint arXiv:1812.00099},
  year={2018}
}

@inproceedings{ekstrand,
  title={Exploring author gender in book rating and recommendation},
  author={Ekstrand, Michael D and Tian, Mucun and Kazi, Mohammed R Imran and Mehrpouyan, Hoda and Kluver, Daniel},
  booktitle={Proceedings of the 12th ACM Conference on Recommender Systems},
  pages={242--250},
  year={2018},
  organization={ACM}
}

@inproceedings{boluk,
  title={Man is to computer programmer as woman is to homemaker? debiasing word embeddings},
  author={Bolukbasi, Tolga and Chang, Kai-Wei and Zou, James Y and Saligrama, Venkatesh and Kalai, Adam T},
  booktitle={Advances in neural information processing systems},
  pages={4349--4357},
  year={2016}
}

@article{bios,
  title={Bias in Bios: A Case Study of Semantic Representation Bias in a High-Stakes Setting},
  author={De-Arteaga, Maria and Romanov, Alexey and Wallach, Hanna and Chayes, Jennifer and Borgs, Christian and Chouldechova, Alexandra and Geyik, Sahin and Kenthapadi, Krishnaram and Kalai, Adam Tauman},
  journal={arXiv preprint arXiv:1901.09451},
  year={2019}
}

@unpublished{arvindTalk,
title= {21 Fairness Definitions and Their Politics},
author = {Arvind Narayanan},
year = {2018},
note= {Conference on Fairness, Accountability, and Transparency, NYC}
}

@article{kamiran2012,
  title={Data preprocessing techniques for classification without discrimination},
  author={Kamiran, Faisal and Calders, Toon},
  journal={Knowledge and Information Systems},
  volume={33},
  number={1},
  pages={1--33},
  year={2012},
  publisher={Springer}
}

@inproceedings{kamishima2011,
  title={Fairness-aware learning through regularization approach},
  author={Kamishima, Toshihiro and Akaho, Shotaro and Sakuma, Jun},
  booktitle={Data Mining Workshops (ICDMW), 2011 IEEE 11th International Conference on},
  organization={IEEE}
}

@article{inprocess,
  title={Learning fair classifiers: A regularization-inspired approach},
  author={Bechavod, Yahav and Ligett, Katrina},
  journal={arXiv:1707.00044},
  year={2017}
}

@inproceedings{zafar2017fairness,
  title={Fairness constraints: Mechanisms for fair classification},
  author={Zafar, Muhammad Bilal and Valera, Isabel and Rogriguez, Manuel Gomez and Gummadi, Krishna P},
  booktitle={Artificial Intelligence and Statistics},
  year={2017}
}

@article{sweeney2013discrimination,
  title={Discrimination in online ad delivery},
  author={Sweeney, Latanya},
  journal={Queue},
  volume={11},
  number={3},
  pages={10},
  year={2013},
  publisher={ACM}
}

@inproceedings{postProcessing,
  title={Equality of opportunity in supervised learning},
  author={Hardt, Moritz and Price, Eric and Srebro, Nati and others},
  booktitle={Advances in neural information processing systems},
  pages={3315--3323},
  year={2016}
}

@article{processFairness,
  title={Beyond Distributive Fairness in Algorithmic Decision Making: Feature Selection for Procedurally Fair Learning},
  author={Grgic-Hlaca, Nina and Zafar, Muhammad Bilal and Gummadi, Krishna P and Weller, Adrian},
  year={2018}
}

@article{nipsIBM,
  title={Optimized Data Pre-Processing for Discrimination Prevention},
  author={Calmon, Flavio P and Wei, Dennis and Ramamurthy, Karthikeyan Natesan and Varshney, Kush R},
  journal={arXiv preprint arXiv:1704.03354},
  year={2017}
}

@inproceedings{sureshKDD,
  title={Certifying and removing disparate impact},
  author={Feldman, Michael and Friedler, Sorelle A and Moeller, John and Scheidegger, Carlos and Venkatasubramanian, Suresh},
  booktitle={Proceedings of the 21th ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
  year={2015}
}

@article{hajian2013dataModification,
  title={A methodology for direct and indirect discrimination prevention in data mining},
  author={Hajian, Sara and Domingo-Ferrer, Josep},
  journal={IEEE transactions on knowledge and data engineering},
  year={2013},
  publisher={IEEE}
}

@inproceedings{zemel2013learning,
  title={Learning fair representations},
  author={Zemel, Rich and Wu, Yu and Swersky, Kevin and Pitassi, Toni and Dwork, Cynthia},
  booktitle={International Conference on Machine Learning},
  pages={325--333},
  year={2013}
}

@inproceedings{kamiran2009classifying,
  title={Classifying without discriminating},
  author={Kamiran, Faisal and Calders, Toon},
  booktitle={Computer, Control and Communication, 2009. IC4 2009. 2nd International Conference on},
  pages={1--6},
  year={2009},
  organization={IEEE}
}

@misc{germanUCI,
author = {"D. Newman, S. Hettich, C. Blake, and C. Merz"},
year = "1998",
title = {UCI Machine Learning Repository},
url = "https://archive.ics.uci.edu/ml/datasets/statlog+(german+credit+data)",
institution = "University of California, Irvine, School of Information and Computer Sciences" }

@inproceedings{erk2009representing,
  title={Representing words as regions in vector space},
  author={Erk, Katrin},
  booktitle={Proceedings of the Thirteenth Conference on Computational Natural Language Learning},
  pages={57--65},
  year={2009},
  organization={Association for Computational Linguistics}
}
@article{maaten2008visualizing,
  title={Visualizing data using t-SNE},
  author={Maaten, Laurens van der and Hinton, Geoffrey},
  journal={Journal of machine learning research},
  volume={9},
  number={Nov},
  pages={2579--2605},
  year={2008}
}
@inproceedings{hinton1986learning,
  title={Learning distributed representations of concepts},
  author={Hinton, Geoffrey E},
  booktitle={Proceedings of the eighth annual conference of the cognitive science society},
  volume={1},
  pages={12},
  year={1986},
  organization={Amherst, MA}
}

@inproceedings{martins2017mvn,
  title={MVN-Reduce: Dimensionality Reduction for the Visual Analysis of Multivariate Networks},
  author={Martins, Rafael Messias and Kruiger, JF and Minghim, Rosane and Telea, Alexandru C and Kerren, Andreas},
  booktitle={19th EG/VGTC Conference on Visualization (EuroVis' 17), 12-16 June 2017, Barcelona, Spain},
  year={2017},
  organization={Eurographics-European Association for Computer Graphics}
}
@article{bengio2008adaptive,
  title={Adaptive importance sampling to accelerate training of a neural probabilistic language model},
  author={Bengio, Yoshua and Sen{\'e}cal, Jean-S{\'e}bastien},
  journal={IEEE Transactions on Neural Networks},
  volume={19},
  number={4},
  pages={713--722},
  year={2008},
  publisher={IEEE}
}
@inproceedings{morin2005hierarchical,
  title={Hierarchical Probabilistic Neural Network Language Model.},
  author={Morin, Frederic and Bengio, Yoshua},
  booktitle={Aistats},
  volume={5},
  pages={246--252},
  year={2005},
  organization={Citeseer}
}
@inproceedings{mikolov2013linguistic,
  title={Linguistic Regularities in Continuous Space Word Representations.},
  author={Mikolov, Tomas and Yih, Wen-tau and Zweig, Geoffrey},
  booktitle={Hlt-naacl},
  volume={13},
  pages={746--751},
  year={2013}
}
@inproceedings{tsuboi2014neural,
  title={Neural Networks Leverage Corpus-wide Information for Part-of-speech Tagging.},
  author={Tsuboi, Yuta},
  booktitle={EMNLP},
  pages={938--950},
  year={2014}
}
@article{hinton1985learning,
  title={Learning internal representations by back-propagating errors},
  author={Hinton, GE and Rumelhart, DE and Williams, RJ},
  journal={Parallel Distributed Processing: Explorations in the Microstructure of Cognition},
  volume={1},
  year={1985}
}
@inproceedings{raina2009large,
  title={Large-scale deep unsupervised learning using graphics processors},
  author={Raina, Rajat and Madhavan, Anand and Ng, Andrew Y},
  booktitle={Proceedings of the 26th annual international conference on machine learning},
  pages={873--880},
  year={2009},
  organization={ACM}
}
@book{jolliffe2002principal,
  title={Principal component analysis},
  author={Jolliffe, Ian},
  year={2002},
  publisher={Wiley Online Library}
}
@article{mikolov2013efficient,
  title={Efficient estimation of word representations in vector space},
  author={Mikolov, Tomas and Chen, Kai and Corrado, Greg and Dean, Jeffrey},
  journal={arXiv preprint arXiv:1301.3781},
  year={2013}
}
@inproceedings{mikolov2013distributed,
  title={Distributed representations of words and phrases and their compositionality},
  author={Mikolov, Tomas and Sutskever, Ilya and Chen, Kai and Corrado, Greg S and Dean, Jeff},
  booktitle={Advances in neural information processing systems},
  pages={3111--3119},
  year={2013}
}
@book{manning2008introduction,
  title={Introduction to information retrieval},
  author={Manning, Christopher D and Raghavan, Prabhakar and Sch{\"u}tze, Hinrich and others},
  volume={1},
  number={1},
  year={2008},
  publisher={Cambridge university press Cambridge}
}
@inproceedings{mccarthy2004finding,
  title={Finding predominant word senses in untagged text},
  author={McCarthy, Diana and Koeling, Rob and Weeds, Julie and Carroll, John},
  booktitle={Proceedings of the 42nd Annual Meeting on Association for Computational Linguistics},
  pages={279},
  year={2004},
  organization={Association for Computational Linguistics}
}


@inproceedings{le2014distributed,
  title={Distributed representations of sentences and documents},
  author={Le, Quoc and Mikolov, Tomas},
  booktitle={International Conference on Machine Learning},
  pages={1188--1196},
  year={2014}
}
@inproceedings{socher2013recursive,
  title={Recursive deep models for semantic compositionality over a sentiment treebank},
  author={Socher, Richard and Perelygin, Alex and Wu, Jean and Chuang, Jason and Manning, Christopher D and Ng, Andrew and Potts, Christopher},
  booktitle={Proceedings of the 2013 conference on empirical methods in natural language processing},
  pages={1631--1642},
  year={2013}
}
@inproceedings{kenter2015short,
  title={Short text similarity with word embeddings},
  author={Kenter, Tom and De Rijke, Maarten},
  booktitle={Proceedings of the 24th ACM international on conference on information and knowledge management},
  pages={1411--1420},
  year={2015},
  organization={ACM}
}
@article{robertson2009probabilistic,
  title={The probabilistic relevance framework: BM25 and beyond},
  author={Robertson, Stephen and Zaragoza, Hugo and others},
  journal={Foundations and Trends{\textregistered} in Information Retrieval},
  volume={3},
  number={4},
  pages={333--389},
  year={2009},
  publisher={Now Publishers, Inc.}
}
@article{kruskal1964multidimensional,
  title={Multidimensional scaling by optimizing goodness of fit to a nonmetric hypothesis},
  author={Kruskal, Joseph B},
  journal={Psychometrika},
  volume={29},
  number={1},
  pages={1--27},
  year={1964},
  publisher={Springer}
}
@article{rousseeuw1987silhouettes,
  title={Silhouettes: a graphical aid to the interpretation and validation of cluster analysis},
  author={Rousseeuw, Peter J},
  journal={Journal of computational and applied mathematics},
  volume={20},
  pages={53--65},
  year={1987},
  publisher={Elsevier}
}
@article{calinski1974dendrite,
  title={A dendrite method for cluster analysis},
  author={Cali{\'n}ski, Tadeusz and Harabasz, Jerzy},
  journal={Communications in Statistics-theory and Methods},
  volume={3},
  number={1},
  pages={1--27},
  year={1974},
  publisher={Taylor \& Francis}
}

@article{Zhang2015VisualMap,
    title = {{Visual Correlation Analysis of Numerical and Categorical Data on the Correlation Map}},
    year = {2015},
    journal = {IEEE Transactions on Visualization and Computer Graphics},
    author = {Zhang, Zhiyuan and Mcdonnell, Kevin T and Zadok, Erez and Mueller, Klaus},
    number = {2},
    pages = {289--303},
    volume = {21}
}

@inproceedings{Inselberg1990,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Inselberg, Alfred and Dimsdale, Bernard},
booktitle = {1st conference on Visualization '90},
doi = {10.1109/VISUAL.1990.146402},
eprint = {arXiv:1011.1669v3},
isbn = {0-8186-2083-8},
issn = {1098-6596},
pages = {361--378},
pmid = {25246403},
title = {{Parallel Coordinates: a tool for visualizing muti-dimensional geometry}},
url = {http://dl.acm.org/citation.cfm?id=949588},
year = {1990}
}
@book{Pearl2000,
author = {Pearl, Judea},
isbn = {978-0521895606},
publisher = {Cambridge University Press},
title = {{Causality: Models, Reasoning, and Inference}},
year = {2000}
}
@article{Pearl2009,
archivePrefix = {arXiv},
arxivId = {arXiv:1112.1788v3},
author = {Pearl, Judea},
doi = {10.1214/09-SS057},
eprint = {arXiv:1112.1788v3},
isbn = {1935-7516},
issn = {1935-7516},
journal = {Statistics Surveys},
number = {0},
pages = {96--146},
pmid = {25246403},
title = {{Causal inference in statistics: An overview}},
volume = {3},
year = {2009}
}

@book{Spirtes2000,
address = {Cambridge, MA},
author = {Spirtes, Peter and Glymour, Clark and Scheines, Richard},
isbn = {978-0262194402},
keywords = {FCI,PC,SGS},
mendeley-groups = {Causal Inference Algorithms},
mendeley-tags = {FCI,PC,SGS},
publisher = {MIT Press},
title = {{Causation, Prediction, and Search}},
year = {2000}
}

@article{Pearl2001,
author = {Pearl, Judea and Russell, Stuart},
pages = {1--7},
title = {{Bayesian networks}},
year = {2001}
}

@article{Pearl2010AnInference,
    title = {{An Introduction to Causal Inference}},
    year = {2010},
    journal = {The International Journal of Biostatistics},
    author = {Pearl, Judea},
    number = {2},
    pages = {1--62},
    volume = {6},
    isbn = {0049124196},
    doi = {10.2202/1557-4679.1203},
    issn = {1557-4679},
    pmid = {20305706},
    arxivId = {0803973233},
    keywords = {Algorithms, Causality, Confounding Factors (Epidemiology), Humans, Models, Research Design, Statistical}
}
    
@article{Bongers2016StructuralReductions,
    title = {{Structural Causal Models: Cycles, Marginalizations, Exogenous Reparametrizations and Reductions}},
    year = {2016},
    journal = {arXiv},
    author = {Bongers, Stephan and Peters, Jonas and Sch{\"{o}}lkopf, Bernhard and Mooij, Joris M},
    month = {11},
    url = {http://arxiv.org/abs/1611.06221},
    arxivId = {1611.06221},
    keywords = {()}
}

@article{Pearl1995,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Pearl, Judea and Verma, Thomas S.},
doi = {10.1016/S0049-237X(06)80074-1},
eprint = {arXiv:1011.1669v3},
isbn = {1558601651},
issn = {0049237X},
journal = {Studies in Logic and the Foundations of Mathematics},
keywords = {IC},
mendeley-groups = {Causal Inference Algorithms},
mendeley-tags = {IC},
pages = {789--811},
pmid = {25246403},
title = {{A theory of inferred causation}},
volume = {134},
year = {1995}
}
@article{Colombo2014Order-independentLearning,
    title = {{Order-independent constraint-based causal structure learning}},
    year = {2014},
    journal = {Journal of Machine Learning Research},
    author = {Colombo, Diego and Maathuis, Marloes},
    doi = {papers3://publication/uuid/CC1A353F-4C95-4058-93CC-05855FD6E5E3}
}

@article{pellet2008using,
  title={Using Markov blankets for causal structure learning},
  author={Pellet, Jean-Philippe and Elisseeff, Andr{\'e}},
  journal={Journal of Machine Learning Research},
  volume={9},
  number={Jul},
  pages={1295--1342},
  year={2008}
}


@inproceedings{Dang2015ReactionFlow:Pathways,
    title = {{ReactionFlow: an interactive visualization tool for causality analysis in biological pathways}},
    year = {2015},
    booktitle = {Proceedings of the 5th Symposium on Biological Data Visualization: Part 2},
    author = {Dang, Tuan and Murray, Paul and Aurisano, Jillian and Forbes, Angus},
    number = {Suppl 6},
    volume = {9},
    url = {http://bmcproc.biomedcentral.com/articles/10.1186/1753-6561-9-S6-S6},
    doi = {10.1186/1753-6561-9-S6-S6},
    issn = {1753-6561}
}

@article{Elmqvist2004AnimatedGeometry,
    title = {{Animated visualization of causal relations through growing 2D geometry}},
    year = {2004},
    journal = {Information Visualization},
    author = {Elmqvist, Niklas and Tsigas, Philippas},
    number = {3},
    pages = {154--172},
    volume = {3},
    url = {http://dl.acm.org/citation.cfm?id=1039751.1039754},
    isbn = {1473-8716},
    doi = {10.1057/palgrave.ivs.9500074},
    issn = {1473-8716},
    keywords = {causal relations, interactive animation}
}

@article{Wang2016,
    author = {Wang, Jun and Mueller, Klaus},
    doi = {10.1109/TVCG.2015.2467931},
    isbn = {1077-2626},
    issn = {10772626},
    journal = {IEEE Transactions on Visualization and Computer Graphics},
    keywords = {Correlation,Inference algorithms,Layout,Linear regression,Optimization,Visualization},
    title = {{The Visual Causality Analyst: An Interactive Interface for Causal Reasoning}},
    year = {2016}
}

@inproceedings{wang2017visual,
  title={Visual causality analysis made practical},
  author={Wang, Jun and Mueller, Klaus},
  booktitle={Proc. IEEE VAST},
  pages={151--161},
  year={2017}
}

@article{Kadaba2007,
author = {Kadaba, Nivedita R. and Irani, Pourang P. and Leboe, Jason},
doi = {10.1109/TVCG.2007.70528},
file = {:D$\backslash$:/WorkSpace/Mendeley/Visualizing causal semantics using animations - IEEE Transactions on Visualization and Computer Graphics - 2007.pdf:pdf},
isbn = {1077-2626},
issn = {10772626},
journal = {IEEE Transactions on Visualization and Computer Graphics},
keywords = {Animated graphs,Causality,Graph semantics,Perception,Semantics,Visualization,Visualizing cause and effect},
number = {6},
pages = {1254--1261},
pmid = {17968072},
title = {{Visualizing causal semantics using animations}},
volume = {13},
year = {2007}
}

@article{Burnham2004,
abstract = {AICc justification},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Burnham, K. P. and Anderson, R.P.},
doi = {10.1177/0049124104268644},
eprint = {arXiv:1011.1669v3},
isbn = {00491241 (ISSN)},
issn = {0049-1241},
journal = {Sociological Methods {\&} Research},
number = {2},
pages = {261--304},
pmid = {21699709},
title = {{Multimodel Inference: Understanding AIC and BIC in Model Selection}},
volume = {33},
year = {2004}
}

@article{Siirtola1997,
doi = {10.1057/palgrave.ivs.9500086},
isbn = {1473-8716},
issn = {14738724},
journal = {Information Visualization},
keywords = {Multi-dimensional data visualization,barycenter heuristic,cluster analysis,the reorderable matrix,user interface},
number = {1},
pages = {32--48},
title = {{Constructing and reconstructing the reorderable matrix}},
volume = {4},
year = {1997}
}

@article{dressel2018accuracy,
  title={The accuracy, fairness, and limits of predicting recidivism},
  author={Dressel, Julia and Farid, Hany},
  journal={Science Advances},
  volume={4},
  number={1},
  pages={eaao5580},
  year={2018},
  publisher={American Association for the Advancement of Science}
}

@article{angwin2016machine,
  title={Machine bias},
  author={Angwin, Julia and Larson, Jeff and Mattu, Surya and Kirchner, Lauren},
  journal={ProPublica, May},
  volume={23},
  number={2016},
  pages={139--159},
  year={2016}
}

@book{hellman2008discrimination,
  title={When is discrimination wrong?},
  author={Hellman, Deborah},
  year={2008},
  publisher={Harvard University Press}
}

@book{eubanks2018automating,
  title={Automating inequality: How high-tech tools profile, police, and punish the poor},
  author={Eubanks, Virginia},
  year={2018},
  publisher={St. Martin's Press}
}

@article{chouldechova2017fair,
  title={Fair prediction with disparate impact: A study of bias in recidivism prediction instruments},
  author={Chouldechova, Alexandra},
  journal={Big data},
  volume={5},
  number={2},
  pages={153--163},
  year={2017},
  publisher={Mary Ann Liebert, Inc. 140 Huguenot Street, 3rd Floor New Rochelle, NY 10801 USA}
}

@inproceedings{kilbertus2017avoiding,
  title={Avoiding discrimination through causal reasoning},
  author={Kilbertus, Niki and Carulla, Mateo Rojas and Parascandolo, Giambattista and Hardt, Moritz and Janzing, Dominik and Sch{\"o}lkopf, Bernhard},
  booktitle={Advances in Neural Information Processing Systems},
  pages={656--666},
  year={2017}
}

@inproceedings{kusner2017counterfactual,
  title={Counterfactual fairness},
  author={Kusner, Matt J and Loftus, Joshua and Russell, Chris and Silva, Ricardo},
  booktitle={Advances in Neural Information Processing Systems}
}


@book{rousseeuw1990finding,
  title={Finding groups in data},
  author={Rousseeuw, Peter J and Kaufman, L},
  year={1990},
  publisher={Wiley Online Library Hoboken}
}

@article{kullback1951information,
  title={On information and sufficiency},
  author={Kullback, Solomon and Leibler, Richard A},
  journal={The annals of mathematical statistics},
  volume={22},
  number={1},
  pages={79--86},
  year={1951},
  publisher={JSTOR}
}

@Article{pcalg,
    title = {Causal Inference Using Graphical Models with the {R}
      Package {pcalg}},
    author = {Markus Kalisch and Martin M\"achler and Diego Colombo and
      Marloes H. Maathuis and Peter B\"uhlmann},
    journal = {Journal of Statistical Software},
    year = {2012},
    volume = {47},
    number = {11},
    pages = {1--26},
    url = {http://www.jstatsoft.org/v47/i11/},
  }

@article{cdt,
  title={Causal Discovery Toolbox: Uncover causal relationships in Python},
  author={Kalainathan, Diviyan and Goudet, Olivier},
  journal={arXiv preprint arXiv:1903.02278},
  year={2019}
}

@article{gower,
  title={A general coefficient of similarity and some of its properties},
  author={Gower, John C},
  journal={Biometrics},
  pages={857--871},
  year={1971},
  publisher={JSTOR}
}

@Article{MXM,
    title = {Feature Selection with the {R} Package {MXM}: Discovering
      Statistically Equivalent Feature Subsets},
    author = {Vincenzo Lagani and Giorgos Athineou and Alessio
      Farcomeni and Michail Tsagris and Ioannis Tsamardinos},
    journal = {Journal of Statistical Software},
    year = {2017},
    volume = {80},
    number = {7},
    doi = {10.18637/jss.v080.i07},
  }

@article{cytoscape,
  title={Cytoscape. js: a graph theory library for visualisation and analysis},
  author={Franz, Max and Lopes, Christian T and Huck, Gerardo and Dong, Yue and Sumer, Onur and Bader, Gary D},
  journal={Bioinformatics},
  volume={32},
  number={2},
  pages={309--311},
  year={2016},
  publisher={Oxford University Press}
}

@article{borkin2013makes,
  title={What makes a visualization memorable?},
  author={Borkin, Michelle A and Vo, Azalea A and Bylinskii, Zoya and Isola, Phillip and Sunkavalli, Shashank and Oliva, Aude and Pfister, Hanspeter},
  journal={IEEE Transactions on Visualization and Computer Graphics},
  volume={19},
  number={12},
  pages={2306--2315},
  year={2013},
  publisher={IEEE}
}

@article{salimi2019data,
  title={Data Management for Causal Algorithmic Fairness},
  author={Salimi, Babak and Howe, Bill and Suciu, Dan},
  journal={arXiv preprint arXiv:1908.07924},
  year={2019}
}

@article{glymour2019review,
  title={Review of causal discovery methods based on graphical models},
  author={Glymour, Clark and Zhang, Kun and Spirtes, Peter},
  journal={Frontiers in genetics},
  year={2019},
  publisher={Frontiers}
}

@inproceedings{silva,
  title={Silva: Interactively Assessing Machine Learning Fairness Using Causality},
  author={Yan, Jing Nathan and Gu, Ziwei and Lin, Hubert and Rzeszotarski, Jeffrey M},
  booktitle={ACM CHI Conference on Human Factors in Computing Systems},
  year={2020}
}
  
@article{DiscriLens,
  title={Visual Analysis of Discrimination in Machine Learning},
  author={Wang, Qianwen and Xu, Zhenhua and Chen, Zhutian and Wang, Yong and Liu, Shixia and Qu, Huamin},
  journal={arXiv},
  year={2020}
}

@article{tsagris2018constraint,
  title={Constraint-based causal discovery with mixed data},
  author={Tsagris, Michail and Borboudakis, Giorgos and Lagani, Vincenzo and Tsamardinos, Ioannis},
  journal={International journal of data science and analytics},
  year={2018}
}

@article{chickering2002optimal,
  title={Optimal structure identification with greedy search},
  author={Chickering, David Maxwell},
  journal={Journal of machine learning research},
  year={2002}
}

@inproceedings{ghai2021wordbias,
  title={WordBias: An Interactive Visual Tool for Discovering Intersectional Biases Encoded in Word Embeddings},
  author={Ghai, Bhavya and Hoque, Md Naimul and Mueller, Klaus},
  booktitle={ACM CHI, Extended Abstracts},
  year={2021}
}

@article{fges,
  title={A million variables and more: the Fast Greedy Equivalence Search algorithm for learning high-dimensional graphical causal models, with an application to functional magnetic resonance images},
  author={Ramsey, Joseph and Glymour, Madelyn and Sanchez-Romero, Ruben and Glymour, Clark},
  journal={International journal of data science and analytics},
  year={2017}
}


@article{xie2020visual,
  title={A visual analytics approach for exploratory causal analysis: Exploration, validation, and applications},
  author={Xie, Xiao and Du, Fan and Wu, Yingcai},
  journal={IEEE Transactions on Visualization and Computer Graphics},
  volume={27},
  number={2},
  pages={1448--1458},
  year={2020}
}

@misc{rajabi2021tabfairgan,
      title={TabFairGAN: Fair Tabular Data Generation with Generative Adversarial Networks}, 
      author={Amirarsalan Rajabi and Ozlem Ozmen Garibay},
      year={2021},
      eprint={2109.00666},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@article{hoque2021outcome,
  title={Outcome-explorer: A causality guided interactive visual interface for interpretable algorithmic decision making},
  author={Hoque, Md Naimul and Mueller, Klaus},
  journal={arXiv preprint arXiv:2101.00633},
  year={2021}
}

@article{wachter2021fairness,
  title={Why fairness cannot be automated: Bridging the gap between EU non-discrimination law and AI},
  author={Wachter, Sandra and Mittelstadt, Brent and Russell, Chris},
  journal={Computer Law \& Security Review},
  volume={41},
  pages={105567},
  year={2021},
  publisher={Elsevier}
}

@article{barocas2017fairness,
  title={Fairness in machine learning},
  author={Barocas, Solon and Hardt, Moritz and Narayanan, Arvind},
  journal={Nips tutorial},
  volume={1},
  pages={2017},
  year={2017}
}

@article{bickel1975sex,
  title={Sex bias in graduate admissions: Data from Berkeley},
  author={Bickel, Peter J and Hammel, Eugene A and O'Connell, J William},
  journal={Science},
  year={1975},
  publisher={American Association for the Advancement of Science}
}

@article{zhang2017anti,
  title={Anti-discrimination learning: a causal modeling-based framework},
  author={Zhang, Lu and Wu, Xintao},
  journal={International Journal of Data Science and Analytics},
  volume={4},
  number={1},
  pages={1--16},
  year={2017},
  publisher={Springer}
}

@inproceedings{zhang2017causal,
  title={A causal framework for discovering and removing direct and indirect discrimination},
  author={Zhang, Lu and Wu, Yongkai and Wu, Xintao},
  booktitle={Proceedings of the 26th International Joint Conference on Artificial Intelligence},
  year={2017}
}

@inproceedings{wu2018discrimination,
  title={On discrimination discovery and removal in ranked data using causal graph},
  author={Wu, Yongkai and Zhang, Lu and Wu, Xintao},
  booktitle={ACM SIGKDD Conference on Knowledge Discovery \& Data Mining},
  year={2018}
}

@inproceedings{chiappa2019path,
  title={Path-specific counterfactual fairness},
  author={Chiappa, Silvia},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  year={2019}
}

@techreport{friendly1994fourfold,
  title={A fourfold display for 2 by 2 by k tables},
  author={Friendly, Michael},
  year={1994},
  institution={Citeseer}
}

@article{sofrygin2017simcausal,
  title={Simcausal R package: conducting transparent and reproducible simulation studies of causal effect estimation with complex longitudinal data},
  author={Sofrygin, Oleg and van der Laan, Mark J and Neugebauer, Romain},
  journal={Journal of Statistical Software},
  year={2017},
  publisher={NIH Public Access}
}

@article{lee2019algorithmic,
  title={Algorithmic bias detection and mitigation: Best practices and policies to reduce consumer harms},
  author={Lee, Nicol Turner and Resnick, Paul and Barton, Genie},
  journal={Brookings Institute: Washington, DC, USA},
  year={2019}
}

@inproceedings{chiappa2018causal,
  title={A causal bayesian networks viewpoint on fairness},
  author={Chiappa, Silvia and Isaac, William S},
  booktitle={IFIP International Summer School on Privacy and Identity Management},
  pages={3--20},
  year={2018},
  organization={Springer}
}

@article{ghai2022cascaded,
  title={Cascaded Debiasing: Studying the Cumulative Effect of Multiple Fairness-Enhancing Interventions},
  author={Ghai, Bhavya and Mishra, Mihir and Mueller, Klaus},
  journal={arXiv preprint arXiv:2202.03734},
  year={2022}
}

@misc{feldman2021endtoend,
      title={End-To-End Bias Mitigation: Removing Gender Bias in Deep Learning}, 
      author={Tal Feldman and Ashley Peake},
      year={2021},
      eprint={2104.02532},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@book{pearl2018book,
  title={The book of Why: The New Science of Cause and Effect},
  author={Pearl, Judea and Mackenzie, Dana},
  year={2018},
  publisher={Basic books}
}

@article{zarebavani2019cupc,
  title={cuPC: CUDA-based parallel PC algorithm for causal structure learning on GPU},
  author={Zarebavani, Behrooz and Jafarinejad, Foad and Hashemi, Matin and Salehkaleybar, Saber},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  volume={31},
  number={3},
  pages={530--542},
  year={2019},
  publisher={IEEE}
}

@article{xie2021fairrankvis,
  title={FairRankVis: A Visual Analytics Framework for Exploring Algorithmic Fairness in Graph Mining Models},
  author={Xie, Tiankai and Ma, Yuxin and Kang, Jian and Tong, Hanghang and Maciejewski, Ross},
  journal={IEEE Transactions on Visualization and Computer Graphics},
  volume={28},
  number={1},
  pages={368--377},
  year={2021},
  publisher={IEEE}
}

% dramatvis.bib
% Created August 2021 by Niklas Elmqvist

@String{addrACM           = {New York, NY, USA}}
@String{addrIEEE          = {Piscataway, NJ, USA}}
@String{addrIEEECS        = {Los Alamitos, CA, USA}}
@String{jourCGF           = {Computer Graphics Forum}}
@String{jourCompGraphAppl = {{IEEE} Computer Graphics and Applications}}
@String{jourHCS           = {International Journal of Human-Computer Studies}}
@String{jourIEEEComp      = {{IEEE} Computer}}
@String{jourInfoVis       = {Information Visualization}}
@String{jourPersUbiqComp  = {Personal and Ubiquitous Computing}}
@String{jourPervComp      = {{IEEE} Pervasive Computing}}
@String{jourTVCG          = {{{IEEE} Transactions on Visualization and Computer Graphics}}}
@String{procCHI           = {Proceedings of the {ACM} Conference on Human Factors in Computing Systems}}
@String{procCHI-EA        = {Extended Abstracts of the ACM Conference on Human Factors in Computing Systems}}
@String{procCMV           = {Proceedings of the {IEEE} Conference on Coordinated and Multiple Views in Exploratory Visualization}}
@String{procCSCW          = {Proceedings of the {ACM} Conference on Computer-Supported Cooperative Work and Social Computing}}
@String{procISS           = {Proceedings of the {ACM} Conference on Interactive Surfaces and Spaces}}
@String{procITS           = {Proceedings of the {ACM} Conference on Interactive Tabletops and Surfaces}}
@String{procMobileHCI     = {Proceedings of the {ACM} Conference on Human-Computer Interaction with Mobile Devices and Services}}
@String{procNordiCHI      = {Proceedings of the Nordic Conference on Human-Computer Interaction}}
@String{procInfoVis    = {Proceedings of the {IEEE} Conference on Information Visualization}}
@String{procPacificVis    = {Proceedings of the {IEEE} Pacific Symposium on Visualization}}
@String{procUbiComp       = {Proceedings of the {ACM} Conference on Pervasive and Ubiquitous Computing}}
@String{procUIST          = {Proceedings of the {ACM} Symposium on User Interface Software and Technology}}
@String{procVAST          = {Proceedings of the {IEEE} Conference on Visual Analytics Science and Technology}}
@String{procAVI          = {Proceedings of the {ACM} Conference on Advanced Visual Interfaces}}
@String{proc3DUI          = {Proceedings of the {ACM} IEEE Symposium on 3D User Interfaces}}
@String{pubACM            = {{ACM}}}
@String{pubElsevier       = {Elsevier}}
@String{pubIEEE           = {{IEEE}}}
@String{pubSage           = {{SAGE} Publications}}
@String{pubSpringer       = {Springer Publishing}}
@String{pubSpringerIntern = {Springer International Publishing}}
@String{addrSpringer      = {New York, NY, USA}}
@String{jourACMTAP        = {{{ACM}} Transactions on Applied Perception}}
@String{procISMAR         = {Proceedings of the {IEEE} International Symposium on Mixed and Augmented Reality}}
@String{procISMARadjunct  = {{Adjunct Proceedings of the IEEE International Symposium on Mixed and Augmented Reality}}}
@String{procSIGGRAPH      = {Proceedings of the Annual Conference on Computer Graphics and Interactive Techniques}}
@String{pubACL = {Association for Computational Linguistics}}
@String{addrACL = {Florence, Italy}}

@article{DBLP:journals/tvcg/KimBISGP18,
  author    = {Nam Wook Kim and
               Benjamin Bach and
               Hyejin Im and
               Sasha Schriber and
               Markus H. Gross and
               Hanspeter Pfister},
  title     = {Visualizing Nonlinear Narratives with Story Curves},
  journal   = jourTVCG,
  volume    = {24},
  number    = {1},
  pages     = {595--604},
  year      = {2018},
  doi       = {10.1109/TVCG.2017.2744118},
}

@article{DBLP:journals/tvcg/TanahashiM12,
  author    = {Yuzuru Tanahashi and
               Kwan{-}Liu Ma},
  title     = {Design Considerations for Optimizing Storyline Visualizations},
  journal   = jourTVCG,
  volume    = {18},
  number    = {12},
  pages     = {2679--2688},
  year      = {2012},
  doi       = {10.1109/TVCG.2012.212},
}

@article{DBLP:journals/tvcg/LiuWWLL13,
  author    = {Shixia Liu and
               Yingcai Wu and
               Enxun Wei and
               Mengchen Liu and
               Yang Liu},
  title     = {{StoryFlow}: Tracking the Evolution of Stories},
  journal   = jourTVCG,
  volume    = {19},
  number    = {12},
  pages     = {2436--2445},
  year      = {2013},
  doi       = {10.1109/TVCG.2013.196},
}

@inproceedings{DBLP:conf/taai/HuangLS13,
  author    = {Chieh{-}Jen Huang and
               Cheng{-}Te Li and
               Man{-}Kwan Shan},
  title     = {{VizStory}: Visualization of Digital Narrative for Fairy Tales},
  booktitle = {Proceedings of the Conference on Technologies and Applications of Artificial Intelligence},
  pages     = {67--72},
  publisher = {{IEEE} Computer Society},
  address   = addrIEEE,
  year      = {2013},
  doi       = {10.1109/TAAI.2013.26},
}

@inproceedings{DBLP:conf/gd/GronemannJLM16,
  author    = {Martin Gronemann and
               Michael J{\"{u}}nger and
               Frauke Liers and
               Francesco Mambelli},
  title     = {Crossing Minimization in Storyline Visualization},
  booktitle = {Proceedings of the International Symposium on Graph Drawing and Network Visualization},
  series    = {Lecture Notes in Computer Science},
  volume    = {9801},
  pages     = {367--381},
  publisher = {Springer},
  year      = {2016},
  doi       = {10.1007/978-3-319-50106-2\_29},
}

@article{DBLP:journals/tvcg/CuiLTSSGQT11,
  author    = {Weiwei Cui and
               Shixia Liu and
               Li Tan and
               Conglei Shi and
               Yangqiu Song and
               Zekai Gao and
               Huamin Qu and
               Xin Tong},
  title     = {{TextFlow}: Towards Better Understanding of Evolving Topics in Text},
  journal   = jourTVCG,
  volume    = {17},
  number    = {12},
  pages     = {2412--2421},
  year      = {2011},
  doi       = {10.1109/TVCG.2011.239},
}

@inproceedings{DBLP:conf/iui/WatsonSSGMK19,
  author    = {Katie Watson and
               Samuel S. Sohn and
               Sasha Schriber and
               Markus Gross and
               Carlos Manuel Mu{\~{n}}iz and
               Mubbasir Kapadia},
  title     = {{StoryPrint}: an interactive visualization of stories},
  booktitle = {Proceedings of the ACM Conference on Intelligent User Interfaces},
  pages     = {303--311},
  publisher = pubACM,
  address   = addrACM,
  year      = {2019},
  doi       = {10.1145/3301275.3302302},
}

@article{DBLP:journals/cgf/CorrellWG11,
  author    = {Michael Correll and
               Michael Witmore and
               Michael Gleicher},
  title     = {Exploring Collections of Tagged Text for Literary Scholarship},
  journal   = {Computer Graphics Forum},
  volume    = {30},
  number    = {3},
  pages     = {731--740},
  year      = {2011},
  doi       = {10.1111/j.1467-8659.2011.01922.x},
}

@inproceedings{DBLP:conf/infovis/RohrerSE98,
  author    = {Randall M. Rohrer and
               John L. Sibert and
               David S. Ebert},
  title     = {The Shape of Shakespeare: Visualizing Text using Implicit Surfaces},
  booktitle = {Proceedings of the {IEEE} Symposium on Information Visualization},
  pages     = {121--129},
  publisher = pubIEEE,
  address   = addrIEEE,
  year      = {1998},
  doi       = {10.1109/INFVIS.1998.729568},
}

@inproceedings{DBLP:conf/dihu/ChaturvediGMAH12,
  author    = {Manish Chaturvedi and
               Gerald C. Gannod and
               Laura Mandell and
               Helen Armstrong and
               Eric Hodgson},
  editor    = {Jan Christoph Meister},
  title     = {Myopia: {A} Visualization Tool in Support of Close Reading},
  booktitle = {Proceedings of the Annual International Conference of the Alliance of Digital Humanities Organizations},
  pages     = {148--150},
  publisher = {Hamburg University Press},
  address   = {Hamburg, Germany},
  year      = {2012},
}

@article{DBLP:journals/cgf/Abdul-RahmanLCMMWJTC13,
  author    = {Alfie Abdul{-}Rahman and
               Julie Lein and
               Katherine Coles and
               Eamonn Maguire and
               Miriah D. Meyer and
               Martin Wynne and
               Chris R. Johnson and
               Anne E. Trefethen and
               Min Chen},
  title     = {Rule-based Visual Mappings - with a Case Study on Poetry Visualization},
  journal   = {Computer Graphics Forum},
  volume    = {32},
  number    = {3},
  pages     = {381--390},
  year      = {2013},
  doi       = {10.1111/cgf.12125},
}

@article{DBLP:journals/tvcg/McCurdyLCM16,
  author    = {Nina McCurdy and
               Julie Lein and
               Katherine Coles and
               Miriah D. Meyer},
  title     = {Poemage: Visualizing the Sonic Topology of a Poem},
  journal   = jourTVCG,
  volume    = {22},
  number    = {1},
  pages     = {439--448},
  year      = {2016},
  doi       = {10.1109/TVCG.2015.2467811},
}

@article{DBLP:journals/widm/AlencarOP12,
  author    = {Aretha Barbosa Alencar and
               Maria Cristina Ferreira de Oliveira and
               Fernando Vieira Paulovich},
  title     = {Seeing beyond reading: a survey on visual text analytics},
  journal   = {Wiley Interdisciplinary Reviews: Data Mining and Knowledge Discovery},
  volume    = {2},
  number    = {6},
  pages     = {476--492},
  year      = {2012},
  doi       = {10.1002/widm.1071},
}

@inproceedings{DBLP:conf/ieeevast/KeimO07,
  author    = {Daniel A. Keim and
               Daniela Oelke},
  title     = {Literature Fingerprinting: {A} New Method for Visual Literary Analysis},
  booktitle = {Proceedings of the {IEEE} Symposium on Visual Analytics Science and Technology},
  pages     = {115--122},
  publisher = pubIEEE,
  address   = addrIEEE,
  year      = {2007},
  doi       = {10.1109/VAST.2007.4389004},
}

@inproceedings{DBLP:conf/kes/SilicB10,
  author    = {Artur {\^S}ilic and
               Bojana Dalbelo Basic},
  editor    = {Rossitza Setchi and
               Ivan Jordanov and
               Robert J. Howlett and
               Lakhmi C. Jain},
  title     = {Visualization of Text Streams: {A} Survey},
  booktitle = {Proceedings of the International Conference on Knowledge-Based and Intelligent Information and Engineering Systems},
  series    = {Lecture Notes in Computer Science},
  volume    = {6277},
  pages     = {31--43},
  publisher = {Springer},
  year      = {2010},
  doi       = {10.1007/978-3-642-15390-7\_4},
}

@article{Qihong2014,
  author = {Gan, Qihong and Zhu, Min and Li, Mingzhao and Liang, Ting and Cao, Yu and Zhou, Baoyao},
  title = {Document visualization: an overview of current research},
  journal = {WIREs Computational Statistics },
  volume = {6},
  number = {1},
  pages = {19--36},
  doi = {https://doi.org/10.1002/wics.1285},
  year = {2014}
}


@inproceedings{DBLP:conf/ieeevast/StaskoGLS07,
  author    = {John T. Stasko and
               Carsten G{\"{o}}rg and
               Zhicheng Liu and
               Kanupriya Singhal},
  title     = {Jigsaw: Supporting Investigative Analysis through Interactive Visualization},
  booktitle = {Proceedings of the {IEEE} Symposium on Visual Analytics Science and Technology},
  pages     = {131--138},
  publisher = pubIEEE,
  address   = addrIEEE,
  year      = {2007},
  doi       = {10.1109/VAST.2007.4389006},
}

@book{KingOnWriting,
  author        = "Stephen King",
  title         = "On Writing: A Memoir of the Craft",
  year          = "2000",
  publisher     = "Charles Scribner's Sons",
}

@book{FictionForDummies,
  title         = "Writing Fiction for Dummies",
  author        = "Randy Ingermanson",
  publisher     = "For Dummies", 
  year          = "2009",
}

@inproceedings{DBLP:conf/infovis/WiseTPLPSC95,
  author    = {James A. Wise and
               James J. Thomas and
               Kelly Pennock and
               David Lantrip and
               Marc Pottier and
               Anne Schur and
               Vern Crow},
  title     = {Visualizing the non-visual: spatial analysis and interaction with
               information from text documents},
  booktitle = {Proceedings of the {IEEE} Symposium on Information Visualization},
  pages     = {51--58},
  publisher = pubIEEE,
  address   = addrIEEE,
  year      = {1995},
  doi       = {10.1109/INFVIS.1995.528686},
}

@article{Cui2011,
  author    = {Weiwei Cui and
               Shixia Liu and
               Li Tan and
               Conglei Shi and
               Yangqiu Song and
               Zekai Gao and
               Huamin Qu and
               Xin Tong},
  title     = {{TextFlow}: Towards Better Understanding of Evolving Topics in Text},
  journal   = jourTVCG,
  volume    = {17},
  number    = {12},
  pages     = {2412--2421},
  year      = {2011},
  doi       = {10.1109/TVCG.2011.239},
}

@article{rudinger2018gender,
  title={Gender bias in coreference resolution},
  author={Rudinger, Rachel and Naradowsky, Jason and Leonard, Brian and Van Durme, Benjamin},
  journal={arXiv preprint arXiv:1804.09301},
  year={2018}
}

@inproceedings{garimella2019women,
  title={Women’s syntactic resilience and men’s grammatical luck: Gender-Bias in Part-of-Speech Tagging and Dependency Parsing},
  author={Garimella, Aparna and Banea, Carmen and Hovy, Dirk and Mihalcea, Rada},
  booktitle={Proceedings of the Annual Meeting of the Association for Computational Linguistics},
  pages={3493--3498},
  year={2019},
  publisher = pubACL,
  address = addrACL,
}

@inproceedings{toshniwal2020learning,
  title={Learning to Ignore: Long Document Coreference with Bounded Memory Neural Networks},
  author={Toshniwal, Shubham and Wiseman, Sam and Ettinger, Allyson and Livescu, Karen and Gimpel, Kevin},
  booktitle={Proceedings of the Conference on Empirical Methods in Natural Language Processing},
  pages={8519--8526},
  year={2020},
  publisher = pubACL
}

@inproceedings{talebrush, 
    author = {Chung, John Joon Young and Kim, Wooseok and Yoo, Kang Min and Lee, Hwaran and Adar, Eytan and Chang, Minsuk}, 
    title = {{TaleBrush}: Sketching Stories with Generative Pretrained Language Models},
    year = {2022},
    booktitle =  procCHI,
    publisher = pubACM,
    address = addrACM,
    pages = {to appear},
}

@article{DBLP:journals/tvcg/GadJGEEHR15,
  author    = {Samah Gad and
               Waqas Javed and
               Sohaib Ghani and
               Niklas Elmqvist and
               E. Thomas Ewing and
               Keith N. Hampton and
               Naren Ramakrishnan},
  title     = {{ThemeDelta}: Dynamic Segmentations over Temporal Topic Models},
  journal   = jourTVCG,
  volume    = {21},
  number    = {5},
  pages     = {672--685},
  year      = {2015},
  doi       = {10.1109/TVCG.2014.2388208},
}

@article{flerx1976sex,
  title={Sex role stereotypes: Developmental aspects and early intervention},
  author={Flerx, Vicki C and Fidler, Dorothy S and Rogers, Ronald W},
  journal={Child Development},
  pages={998--1007},
  year={1976},
  publisher={JSTOR},
}

@article{kolbe1981sex,
  title={Sex-role stereotyping in preschool children's picture books},
  author={Kolbe, Richard and La Voie, Joseph C},
  journal={Social Psychology Quarterly},
  pages={369--374},
  year={1981},
  publisher={JSTOR}
}

@article{braun2006using,
  title={Using thematic analysis in psychology},
  author={Braun, Virginia and Clarke, Victoria},
  journal={Qualitative Research in Psychology},
  volume={3},
  number={2},
  pages={77--101},
  year={2006},
  publisher={Taylor \& Francis}
}

@article{peterson1990gender,
  title={Gender stereotypes in children's books: Their prevalence and influence on cognitive and affective development},
  author={Peterson, Sharyl Bender and Lach, Mary Alyce},
  journal={Gender and education},
  volume={2},
  number={2},
  pages={185--197},
  year={1990},
  publisher={Taylor \& Francis}
}
@techreport{adukia2021we,
  title={What we teach about race and gender: Representation in images and text of children’s books},
  author={Adukia, Anjali and Eble, Alex and Harrison, Emileigh and Runesha, Hakizumwami Birali and Szasz, Teodora},
  year={2021},
  institution={National Bureau of Economic Research}
}

@article{hamilton2006gender,
  title={Gender stereotyping and under-representation of female characters in 200 popular children’s picture books: A twenty-first century update},
  author={Hamilton, Mykol C. and Anderson, David and Broaddus, Michelle and Young, Kate},
  journal={Sex Roles},
  volume={55},
  number={11},
  pages={757--765},
  year={2006},
  publisher={Springer}
}

@article{layne2015zebra,
  title={``Zebra world'': The promotion of imperial stereotypes in a children’s book},
  author={Layne, Heidi and Alemanji, Amikeng A},
  journal={Power and Education},
  volume={7},
  number={2},
  pages={181--195},
  year={2015},
  publisher={SAGE Publications Sage UK: London, England}
}

@article{beckett2010away,
  title={`Away with the fairies?' Disability within primary-age children's literature},
  author={Beckett, Angharad and Ellison, Nick and Barrett, Sam and Shah, Sonali},
  journal={Disability \& Society},
  volume={25},
  number={3},
  pages={373--386},
  year={2010},
  publisher={Taylor \& Francis}
}
 
@misc{CLPE,
  title = {Reflecting Realities-Survey of Ethnic Representation within UK Children’s Literature},
  author = {The Centre for Literacy in Primary Education},
  year = 2020,
  url = {https://clpe.org.uk/research/clpe-reflecting-realities-survey-ethnic-representation-within-uk-childrens-literature},
  note = {Accessed: 08/30/2021}
}
@article{narahara1998gender,
  title={Gender Stereotypes in Children's Picture Books.},
  author={Narahara, May M},
  year={1998},
  publisher={ERIC}
}
@book{paynter2011gender,
  title={Gender stereotypes and representation of female characters in children's picture books},
  author={Paynter, Kelly Crisp},
  year={2011},
  publisher={Liberty University}
}
@article{tsao2008gender,
  title={Gender issues in young children's literature},
  author={Tsao, Ya-Lun},
  journal={Reading Improvement},
  volume={45},
  number={3},
  pages={108--115},
  year={2008},
  publisher={Project Innovation (Alabama)}
}

@misc{scrivener,
  author = {Literature and Latte},
  title = {Scrivener},
  year = {2021},
  note =  {Accessed: 2022-02-04},
  url = {https://www.literatureandlatte.com/scrivener/overview/},
}

@article{brown2020language,
  author    = {Tom B. Brown and
               Benjamin Mann and
               Nick Ryder and
               Melanie Subbiah and
               Jared Kaplan and
               Prafulla Dhariwal and
               Arvind Neelakantan and
               Pranav Shyam and
               Girish Sastry and
               Amanda Askell and
               Sandhini Agarwal and
               Ariel Herbert{-}Voss and
               Gretchen Krueger and
               Tom Henighan and
               Rewon Child and
               Aditya Ramesh and
               Daniel M. Ziegler and
               Jeffrey Wu and
               Clemens Winter and
               Christopher Hesse and
               Mark Chen and
               Eric Sigler and
               Mateusz Litwin and
               Scott Gray and
               Benjamin Chess and
               Jack Clark and
               Christopher Berner and
               Sam McCandlish and
               Alec Radford and
               Ilya Sutskever and
               Dario Amodei},
  title     = {Language Models are Few-Shot Learners},
  journal   = {CoRR},
  volume    = {abs/2005.14165},
  year      = {2020},
  numpages  = {75},
  url       = {https://arxiv.org/abs/2005.14165},
  eprinttype = {arXiv},
  eprint    = {2005.14165},
}

@inproceedings{clark2018creative,
  title={Creative writing with a machine in the loop: Case studies on slogans and stories},
  author={Clark, Elizabeth and Ross, Anne Spencer and Tan, Chenhao and Ji, Yangfeng and Smith, Noah A},
  booktitle={Proceedings of the ACM Conference on Intelligent User Interfaces},
  pages={329--340},
  year={2018},
  publisher = pubACM,
  address = addrACM
}

@article{coenen2021wordcraft,
  author    = {Andy Coenen and
               Luke Davis and
               Daphne Ippolito and
               Emily Reif and
               Ann Yuan},
  title     = {Wordcraft: a Human-{AI} Collaborative Editor for Story Writing},
  journal   = {CoRR},
  volume    = {abs/2107.07430},
  year      = {2021},
  url       = {https://arxiv.org/abs/2107.07430},
  eprinttype = {arXiv},
  eprint    = {2107.07430},
  numpages  = {7},
}

@article{lee2022coauthor,
  title={CoAuthor: Designing a Human-AI Collaborative Writing Dataset for Exploring Language Model Capabilities},
  author={Lee, Mina and Liang, Percy and Yang, Qian},
  journal={procCHI},
  year={2022}
}

@inproceedings{hui2018introassist,
  title={IntroAssist: A tool to support writing introductory help requests},
  author={Hui, Julie S and Gergle, Darren and Gerber, Elizabeth M},
  booktitle={Proceedings of the ACM Conference on Human Factors in Computing Systems},
  pages={1--13},
  year={2018},
  doi = {10.1145/3173574.3173596},
  publisher = pubACM,
  address = addrACM
}

@inproceedings{maiden2018making,
  title={Making the news: Digital creativity support for journalists},
  author={Maiden, Neil and Zachos, Konstantinos and Brown, Amanda and Brock, George and Nyre, Lars and Nyg{\aa}rd Tonheim, Aleksander and Apsotolou, Dimitris and Evans, Jeremy},
  booktitle=procCHI,
  pages={1--11},
  year={2018},
  publisher = pubACM,
  address = addrACM
}

@inproceedings{sterman2020interacting,
  title={Interacting with Literary Style through Computational Tools},
  author={Sterman, Sarah and Huang, Evey and Liu, Vivian and Paulos, Eric},
  booktitle=procCHI,
  pages={1--12},
  year={2020},
  publisher = pubACM,
  address = addrACM
}

@misc{granthika,
  author = {Granthika},
  title = {Granthika Writing Tool},
  year = 2021,
  url = {https://granthika.co},
  note =  {Accessed: 2022-02-04}
}

@misc{QuillJS,
  title = {QuillJS: a Rich Text Editor},
  author = {QuillJS},
  year = 2021,
  url = {https://quilljs.com},
  note = {Accessed: 2022-02-04}
}

@misc{delta,
  author = {QuillJS},
  title = {Delta},
  year = 2021,
  url = {https://github.com/quilljs/delta/},
  note = {Accessed: 2022-02-04}
}

@software{spacy,
  author = {Honnibal, Matthew and Montani, Ines and Van Landeghem, Sofie and Boyd, Adriane},
  title = {{spaCy: Industrial-strength Natural Language Processing in Python}},
  year = 2020,
  publisher = {Zenodo},
  doi = {10.5281/zenodo.1212303},
  url = {https://doi.org/10.5281/zenodo.1212303}
}

@misc{sleeping_beauty,
    author = {Arthur Quiller-Couch, Charles Perrault},
    title = {The Sleeping Beauty and other fairy tales},
    year = 2016,
    url = {https://www.gutenberg.org/files/51275/51275-h/51275-h.htm},
    note = {Accessed: 08/30/2021}
}

@misc{anna_kerreina,
    author = {Leo Tolstoy},
    title = {Anna Karenina},
    year = 1998,
    url = {https://www.gutenberg.org/files/1399/1399-0.txt},
    note = {Accessed: 08/30/2021}
}

@misc{neuralcoref,
  author = {Hugging Face}, 
  title = {NeuralCoref 4.0: Coreference Resolution in spaCy with Neural Networks},
  year = 2021,
  url = {https://github.com/huggingface/neuralcoref},
  note = {Accessed: 2022-02-04}
}
@misc{jurafskyspeech,
  title={Speech and Language Processing: An Introduction to Natural Language Processing, Computational Linguistics, and Speech Recognition},
  author={Jurafsky, Daniel and Martin, James H}
}

@article{mitri2020story,
  title={Story analysis using natural language processing and interactive dashboards},
  author={Mitri, Michel},
  journal={Journal of Computer Information Systems},
  pages={1--11},
  year={2020},
  publisher={Taylor \& Francis}
}

@article{hearst2019evaluation,
  title={An evaluation of semantically grouped word cloud designs},
  author={Hearst, Marti A. and Pedersen, Emily and Patil, Lekha and Lee, Elsie and Laskowski, Paul and Franconeri, Steven},
  journal=jourTVCG,
  volume={26},
  number={9},
  pages={2748--2761},
  year={2019},
  publisher={IEEE}
}

@article{bostock2011d3,
  title={D$^3$ data-driven documents},
  author={Bostock, Michael and Ogievetsky, Vadim and Heer, Jeffrey},
  journal=jourTVCG,
  volume={17},
  number={12},
  pages={2301--2309},
  year={2011},
  publisher={IEEE}
}

@article{viegas2009participatory,
  title={Participatory visualization with wordle},
  author={Viegas, Fernanda B and Wattenberg, Martin and Feinberg, Jonathan},
  journal=jourTVCG,
  volume={15},
  number={6},
  pages={1137--1144},
  year={2009},
  publisher={IEEE}
}

@inproceedings{pethe2020chapter,
  title={Chapter Captor: Text Segmentation in Novels},
  author={Pethe, Charuta and Kim, Allen and Skiena, Steven},
  booktitle={Proceedings of the Conference on Empirical Methods in Natural Language Processing},
  pages={8373--8383},
  year={2020}
}

@inproceedings{kim2020time,
  title={What Time Is It? Temporal Analysis of Novels},
  author={Kim, Allen and Pethe, Charuta and Skiena, Steven},
  booktitle={Proceedings of the Conference on Empirical Methods in Natural Language Processing},
  pages={9076--9086},
  year={2020},
  publisher = pubACL,
  address = addrACL
}

@article{reagan2016emotional,
  title={The emotional arcs of stories are dominated by six basic shapes},
  author={Reagan, Andrew J and Mitchell, Lewis and Kiley, Dilan and Danforth, Christopher M and Dodds, Peter Sheridan},
  journal={EPJ Data Science},
  volume={5},
  number={1},
  pages={1--12},
  year={2016},
  publisher={SpringerOpen}
}

@article{labatut2019extraction,
  title={Extraction and analysis of fictional character networks: A survey},
  author={Labatut, Vincent and Bost, Xavier},
  journal={ACM Computing Surveys},
  volume={52},
  number={5},
  pages={1--40},
  year={2019},
  publisher={ACM New York, NY, USA}
}

@article{dekker2019evaluating,
  title={Evaluating named entity recognition tools for extracting social networks from novels},
  author={Dekker, Niels and Kuhn, Tobias and van Erp, Marieke},
  journal={PeerJ Computer Science},
  volume={5},
  pages={e189},
  year={2019},
  publisher={PeerJ Inc.}
}

@article{zhao2018gender,
  title={Gender bias in coreference resolution: Evaluation and debiasing methods},
  author={Zhao, Jieyu and Wang, Tianlu and Yatskar, Mark and Ordonez, Vicente and Chang, Kai-Wei},
  journal={arXiv preprint arXiv:1804.06876},
  year={2018}
}

@inproceedings{fast2016shirtless,
  title={Shirtless and dangerous: Quantifying linguistic signals of gender bias in an online fiction writing community},
  author={Fast, Ethan and Vachovsky, Tina and Bernstein, Michael S.},
  booktitle={Proceedings of the International AAAI Conference on Web and Social Media},
  year={2016},
  pages = {112--120},
  publisher = pubACL,
  address = addrACL,
}

@inproceedings{madaan2018analyze,
  title={Analyze, detect and remove gender stereotyping from bollywood movies},
  author={Madaan, Nishtha and Mehta, Sameep and Agrawaal, Taneea and Malhotra, Vrinda and Aggarwal, Aditi and Gupta, Yatin and Saxena, Mayank},
  booktitle={Conference on fairness, accountability and transparency},
  pages={92--105},
  year={2018},
  organization={PMLR}
}

@article{emons2010he,
  title={“He Works Outside the Home; She Drinks Coffee and Does the Dishes” Gender Roles in Fiction Programs on Dutch Television},
  author={Emons, Pascale and Wester, Fred and Scheepers, Peer},
  journal={Journal of Broadcasting \& Electronic Media},
  volume={54},
  number={1},
  pages={40--53},
  year={2010},
  publisher={Taylor \& Francis}
}

@misc{gdfilms2008,
  author = {Geena Davis Institue on Gender in Media},
  title = {Gender Stereotypes: An Analysis of Popular Films and TV},
  year = 2008,
  url = {https://seejane.org/wp-content/uploads/GDIGM_Gender_Stereotypes.pdf}
}

@misc{gdblack2019,
  author = {Geena Davis Institue on Gender in Media},
  title = {Representation Of Black Women in Hollywood},
  year = 2019,
  url = {https://seejane.org/research-informs-empowers/representations-of-black-women-in-hollywood/}
}

@misc{uclareport2020,
author = {Hunt, Darnell  and Ramón, Ana-Christina },
title = {Hollywood Diversity Report 2020},
url = {https://socialsciences.ucla.edu/wp-content/uploads/2020/02/UCLA-Hollywood-Diversity-Report-2020-Film-2-6-2020.pdf},
year = {2020}
}

@misc{parity_children,
  author = {Geena Davis Institue on Gender in Media},
  title = {Historic Gender Parity in Children's Television},
  year = 2019,
  url = {https://seejane.org/research-informs-empowers/see-jane-2019/}
}
@misc{parity_films,
  author = {Geena Davis Institue on Gender in Media},
  title = {Historic Gender Parity in Family Films!},
  year = 2020,
  url = {https://seejane.org/2020-film-historic-gender-parity-in-family-films/}
}


@misc{gd_equity2021,
  author = {Geena Davis Institue on Gender in Media},
  title = {Behind the Scenes: the State of Inclusion and Equity In TV Writing},
  year = 2021,
  url = {https://seejane.org/research-informs-empowers/behind-the-scenes-the-state-of-inclusion-and-equity-in-tv-writing/}
}

@article{norberg2016naughty,
  title={Naughty boys and sexy girls: the representation of young individuals in a web-based corpus of English},
  author={Norberg, Cathrine},
  journal={Journal of English Linguistics},
  volume={44},
  number={4},
  pages={291--317},
  year={2016},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{pearce2008investigating,
  title={Investigating the collocational behaviour of MAN and WOMAN in the BNC using Sketch Engine},
  author={Pearce, Michael},
  journal={Corpora},
  volume={3},
  number={1},
  pages={1--29},
  year={2008},
  publisher={Edinburgh University Press 22 George Square, Edinburgh EH8 9LF UK}
}

@inproceedings{hoyle-etal-2019-unsupervised,
    title = "Unsupervised Discovery of Gendered Language through Latent-Variable Modeling",
    author = "Hoyle, Alexander Miserlis  and
      Wolf-Sonkin, Lawrence  and
      Wallach, Hanna  and
      Augenstein, Isabelle  and
      Cotterell, Ryan",
    booktitle = "Proceedings of the Annual Meeting of the Association for Computational Linguistics",
    month = jul,
    year = "2019",
    address = "Florence, Italy",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/P19-1167",
    doi = "10.18653/v1/P19-1167",
    pages = "1706--1716",
}

@inproceedings{joseph2017girls,
  title={Girls rule, boys drool: Extracting semantic and affective stereotypes from Twitter},
  author={Joseph, Kenneth and Wei, Wei and Carley, Kathleen M.},
  booktitle={Proceedings of the ACM Conference on Computer Supported Cooperative Work and Social Computing},
  pages={1362--1374},
  year={2017},
  publisher = pubACM,
  address = addrACM
}

@article{lucy2020content,
  title={Content analysis of textbooks via natural language processing: Findings on gender, race, and ethnicity in Texas US history textbooks},
  author={Lucy, Li and Demszky, Dorottya and Bromley, Patricia and Jurafsky, Dan},
  journal={AERA Open},
  volume={6},
  number={3},
  pages={2332858420940312},
  year={2020},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@inproceedings{ferrer2020discovering,
  title={Discovering and categorising language biases in Reddit},
  author={Ferrer, Xavier and van Nuenen, Tom and Such, Jose M and Criado, Natalia},
  journal={Proceedings of the International AAAI Conference on Web and Social Media},
  year={2021},
  pages={140--151},
  publisher = {{AAAI} Press},
  address = {Palo Alto, CA, USA},
}

@article{matamoros2017platformed,
  title={Platformed racism: The mediation and circulation of an Australian race-based controversy on Twitter, Facebook and YouTube},
  author={Matamoros-Fern{\'a}ndez, Ariadna},
  journal={Information, Communication \& Society},
  volume={20},
  number={6},
  pages={930--946},
  year={2017},
  publisher={Taylor \& Francis}
}

@article{hoque2020toward,
  title={Toward Interactively Balancing the Screen Time of Actors Based on Observable Phenotypic Traits in Live Telecast},
  author={Hoque, Md Naimul and Saquib, Nazmus and Billah, Syed Masum and Mueller, Klaus},
  journal={Proceedings of the ACM on Human-Computer Interaction},
  volume={4},
  number={CSCW2},
  pages={1--18},
  year={2020},
  publisher={ACM New York, NY, USA}
}

@article{scheuerman2019computers,
  title={How computers see gender: An evaluation of gender classification in commercial facial analysis services},
  author={Scheuerman, Morgan Klaus and Paul, Jacob M and Brubaker, Jed R},
  journal={Proceedings of the ACM on Human-Computer Interaction},
  volume={3},
  number={CSCW},
  pages={1--33},
  year={2019},
  publisher={ACM New York, NY, USA}
}

@article{angwin2016machine,
  title={Machine bias},
  author={Angwin, Julia and Larson, Jeff and Mattu, Surya and Kirchner, Lauren},
  journal={ProPublica, May},
  volume={23},
  pages={2016},
  year={2016}
}

@article{100years,
  title={Word embeddings quantify 100 years of gender and ethnic stereotypes},
  author={Garg, Nikhil and Schiebinger, Londa and Jurafsky, Dan and Zou, James},
  journal={Proceedings of the National Academy of Sciences},
  volume={115},
  number={16},
  pages={E3635--E3644},
  year={2018},
  publisher={National Acad Sciences}
}

@inproceedings{ghai2021wordbias,
  title={WordBias: An Interactive Visual Tool for Discovering Intersectional Biases Encoded in Word Embeddings},
  author={Ghai, Bhavya and Hoque, Md Naimul and Mueller, Klaus},
  booktitle={Extended Abstracts of the ACM Conference on Human Factors in Computing Systems},
  pages={1--7},
  year={2021},
  publisher = pubACM,
  address = addrACM,
}

@article{ross2019media,
  title={Media and stereotypes},
  author={Ross, Tara},
  journal={Journal: The Palgrave Handbook of Ethnicity},
  pages={1--17},
  year={2019}
}

@misc{ghai2022cascaded,
  author    = {Bhavya Ghai and
               Mihir Mishra and
               Klaus Mueller},
  title     = {Cascaded Debiasing : Studying the Cumulative Effect of Multiple Fairness-Enhancing Interventions},
  journal   = {CoRR},
  volume    = {abs/2202.03734},
  year      = {2022},
  numpages  = {12},
  url       = {https://arxiv.org/abs/2202.03734},
  eprinttype = {arXiv},
  eprint    = {2202.03734},
}

@inproceedings{mehrabi2020man,
  title={Man is to person as woman is to location: Measuring gender bias in named entity recognition},
  author={Mehrabi, Ninareh and Gowda, Thamme and Morstatter, Fred and Peng, Nanyun and Galstyan, Aram},
  booktitle={Proceedings of the ACM Conference on Hypertext and Social Media},
  pages={231--232},
  year={2020},
  publisher = pubACM,
  address = addrACM
}

@article{kraicer2019social,
  title={Social characters: the hierarchy of gender in contemporary English-language fiction},
  author={Kraicer, Eve and Piper, Andrew},
  journal={Journal of Cultural Analytics},
  volume={1},
  number={1},
  pages={11055},
  year={2019},
  publisher={Department of Languages, Literatures, and Cultures}
}

@article{mishra2020assessing,
  title={Assessing Demographic Bias in Named Entity Recognition},
  author={Mishra, Shubhanshu and He, Sijun and Belli, Luca},
  journal={arXiv preprint arXiv:2008.03415},
  year={2020}
}

@article{bamman2020litbank,
  title={LitBank: Born-Literary Natural Language Processing},
  author={Bamman, David},
  journal={Computational Humanities, Debates in Digital Humanities},
}

@inproceedings{rosiger2018towards,
  title={Towards coreference for literary text: Analyzing domain-specific phenomena},
  author={R{\"o}siger, Ina and Schulz, Sarah and Reiter, Nils},
  booktitle={Proceedings of the Second Joint SIGHUM Workshop on Computational Linguistics for Cultural Heritage, Social Sciences, Humanities and Literature},
  pages={129--138},
  year={2018}
}

@article{hart2006nasa,
  title={NASA-task load index (NASA-TLX); 20 years later},
  author={Hart, Sandra G},
  journal={Proceedings of the human factors and ergonomics society annual meeting},
  volume={50},
  number={9},
  pages={904--908},
  year={2006},
  organization={Sage Publications Sage CA: Los Angeles, CA}
}

@article{correll2007influence,
  title={The influence of stereotypes on decisions to shoot},
  author={Correll, Joshua and Park, Bernadette and Judd, Charles M. and Wittenbrink, Bernd},
  journal={European Journal of Social Psychology},
  volume={37},
  number={6},
  pages={1102--1117},
  year={2007},
  publisher={Wiley Online Library}
}

@article{entman1992blacks,
  title={Blacks in the news: Television, modern racism and cultural change},
  author={Entman, Robert M.},
  journal={Journalism Quarterly},
  volume={69},
  number={2},
  pages={341--361},
  year={1992},
}

@article{ramasubramanian2007activating,
  title={Activating and suppressing hostile and benevolent racism: Evidence for comparative media stereotyping},
  author={Ramasubramanian, Srividya and Oliver, Mary Beth},
  journal={Media psychology},
  volume={9},
  number={3},
  pages={623--646},
  year={2007},
  publisher={Taylor \& Francis}
}
@article{valentino1999crime,
  title={Crime news and the priming of racial attitudes during evaluations of the president},
  author={Valentino, Nicholas A},
  journal={Public Opinion Quarterly},
  pages={293--320},
  year={1999},
  publisher={JSTOR}
}

@article{benjamin2019race,
  title={Race after technology: Abolitionist tools for the new jim code},
  author={Benjamin, Ruha},
  journal={Social Forces},
  year={2019}
}

@incollection{dragicevic2016fair,
  title={Fair Statistical Communication in HCI},
  author={Dragicevic, Pierre},
  booktitle={Modern Statistical Methods for HCI},
  pages={291--330},
  year={2016},
  publisher=pubSpringer,
  address=addrSpringer,
}

@article{efron1992bootstrap,
  title={Bootstrap methods: another look at the jackknife},
  author={Efron, Bradley},
  journal={The Annals of Statistics},
  pages={1--26},
  volume = {7},
  number = {1},
  year={1979},
  publisher={Institute of Mathematical Statistics},
  url = {https://www.jstor.org/stable/2958830},
}

@book{cohen1988statistical,
  title={Statistical Power Analysis for the Social Sciences},
  author={Cohen, Jacob},
  year={1988},
  publisher={Erlbaum Associates},
  address = {Hillsdale, NJ, USA},
}

@inproceedings{karduni2020bois,
  title={{DuBois} wrapped bar chart: Visualizing categorical data with disproportionate values},
  author={Karduni, Alireza and Wesslen, Ryan and Cho, Isaac and Dou, Wenwen},
  booktitle=procCHI,
  pages={1--12},
  year={2020},
  publisher = pubACM,
  address = addrACM,
  doi={10.1145/3313831.3376365},
}

@inproceedings{fr_es,
  title={Examining Gender Bias in Languages with Grammatical Gender},
  author={Zhou, Pei and Shi, Weijia and Zhao, Jieyu and Huang, Kuan-Hao and Chen, Muhao and Cotterell, Ryan and Chang, Kai-Wei},
  booktitle={Proceedings of the Conference on Empirical Methods in Natural Language Processing and the International Joint Conference on Natural Language Processing},
  pages={5279--5287},
  year={2019},
  publisher = pubACL,
  address = addrACL
}

@inproceedings{hindi,
  title={Debiasing Gender biased Hindi Words with Word-embedding},
  author={Pujari, Arun K and Mittal, Ansh and Padhi, Anshuman and Jain, Anshul and Jadon, Mukesh and Kumar, Vikas},
  booktitle={Proceedings of the 2019 2nd International Conference on Algorithms, Computing and Artificial Intelligence},
  pages={450--456},
  year={2019}
}


@article{teso2018should,
  title={" Why Should I Trust Interactive Learners?" Explaining Interactive Queries of Classifiers to Users},
  author={Teso, Stefano and Kersting, Kristian},
  journal={arXiv preprint arXiv:1805.08578},
  year={2018}
}

@article{shivaswamy2015coactive,
  title={Coactive learning},
  author={Shivaswamy, Pannaga and Joachims, Thorsten},
  journal={Journal of Artificial Intelligence Research},
  volume={53},
  pages={1--40},
  year={2015}
}

@techreport{settles2009active,
  title={Active learning literature survey},
  author={Settles, Burr},
  year={2009},
  institution={University of Wisconsin-Madison Department of Computer Sciences}
}

@inproceedings{settles2011closing,
  title={Closing the loop: Fast, interactive semi-supervised annotation with queries on features and instances},
  author={Settles, Burr},
  booktitle={Proceedings of the conference on empirical methods in natural language processing},
  pages={1467--1478},
  year={2011},
  organization={Association for Computational Linguistics}
}

@inproceedings{druck2009active,
  title={Active learning by labeling features},
  author={Druck, Gregory and Settles, Burr and McCallum, Andrew},
  booktitle={Proceedings of the 2009 Conference on Empirical Methods in Natural Language Processing: Volume 1-Volume 1},
  pages={81--90},
  year={2009},
  organization={Association for Computational Linguistics}
}

@misc{olsson2009literature,
  title={A literature survey of active machine learning in the context of natural language processing},
  author={Olsson, Fredrik},
  year={2009},
  publisher={Swedish Institute of Computer Science}
}

@techreport{zhu2005semi,
  title={Semi-supervised learning literature survey},
  author={Zhu, Xiaojin Jerry},
  year={2005},
  institution={University of Wisconsin-Madison Department of Computer Sciences}
}

@article{cohn1994improving,
  title={Improving generalization with active learning},
  author={Cohn, David and Atlas, Les and Ladner, Richard},
  journal={Machine learning},
  volume={15},
  number={2},
  pages={201--221},
  year={1994},
  publisher={Springer}
}

@inproceedings{lewis1994sequential,
  title={A sequential algorithm for training text classifiers},
  author={Lewis, David D and Gale, William A},
  booktitle={SIGIR’94},
  pages={3--12},
  year={1994},
  organization={Springer}
}

@inproceedings{settles2008multiple,
  title={Multiple-instance active learning},
  author={Settles, Burr and Craven, Mark and Ray, Soumya},
  booktitle={Advances in neural information processing systems},
  pages={1289--1296},
  year={2008}
}

@article{raghavan2006active,
  title={Active learning with feedback on features and instances},
  author={Raghavan, Hema and Madani, Omid and Jones, Rosie},
  journal={Journal of Machine Learning Research},
  volume={7},
  number={Aug},
  pages={1655--1686},
  year={2006}
}

@inproceedings{lomasky2007active,
  title={Active class selection},
  author={Lomasky, Rachel and Brodley, Carla E and Aernecke, Matthew and Walt, David and Friedl, Mark},
  booktitle={European Conference on Machine Learning},
  pages={640--647},
  year={2007},
  organization={Springer}
}

@inproceedings{zheng2002active,
  title={On active learning for data acquisition},
  author={Zheng, Zhiqiang and Padmanabhan, Balaji},
  booktitle={2002 IEEE International Conference on Data Mining, 2002. Proceedings.},
  pages={562--569},
  year={2002},
  organization={IEEE}
}


@inproceedings{cakmak2012designing,
  title={Designing robot learners that ask good questions},
  author={Cakmak, Maya and Thomaz, Andrea L},
  booktitle={Proceedings of the seventh annual ACM/IEEE international conference on Human-Robot Interaction},
  pages={17--24},
  year={2012},
  organization={ACM}
}

@inproceedings{saponaro2011generation,
  title={Generation of meaningful robot expressions with active learning},
  author={Saponaro, Giovanni and Bernardino, Alexandre},
  booktitle={2011 6th ACM/IEEE International Conference on Human-Robot Interaction (HRI)},
  pages={243--244},
  year={2011},
  organization={IEEE}
}

@inproceedings{chao2010transparent,
  title={Transparent active learning for robots},
  author={Chao, Crystal and Cakmak, Maya and Thomaz, Andrea L},
  booktitle={2010 5th ACM/IEEE International Conference on Human-Robot Interaction (HRI)},
  pages={317--324},
  year={2010},
  organization={IEEE}
}

@inproceedings{gonzalez2014asking,
  title={Asking rank queries in pose learning},
  author={Gonzalez-Pacheco, Victor and Malfaz, Maria and Salichs, Miguel A},
  booktitle={Proceedings of the 2014 ACM/IEEE international conference on Human-robot interaction},
  pages={164--165},
  year={2014},
  organization={ACM}
}

@article{cakmak2010designing,
  title={Designing interactions for robot active learners},
  author={Cakmak, Maya and Chao, Crystal and Thomaz, Andrea L},
  journal={IEEE Transactions on Autonomous Mental Development},
  volume={2},
  number={2},
  pages={108--118},
  year={2010},
  publisher={IEEE}
}

@article{simard2017machine,
  title={Machine teaching: A new paradigm for building machine learning systems},
  author={Simard, Patrice Y and Amershi, Saleema and Chickering, David M and Pelton, Alicia Edelman and Ghorashi, Soroush and Meek, Christopher and Ramos, Gonzalo and Suh, Jina and Verwey, Johan and Wang, Mo and others},
  journal={arXiv preprint arXiv:1707.06742},
  year={2017}
}

@article{amershi2014power,
  title={Power to the people: The role of humans in interactive machine learning},
  author={Amershi, Saleema and Cakmak, Maya and Knox, William Bradley and Kulesza, Todd},
  journal={AI Magazine},
  volume={35},
  number={4},
  pages={105--120},
  year={2014}
}

@inproceedings{fails2003interactive,
  title={Interactive machine learning},
  author={Fails, Jerry Alan and Olsen Jr, Dan R},
  booktitle={Proceedings of the 8th international conference on Intelligent user interfaces},
  pages={39--45},
  year={2003},
  organization={ACM}
}

@inproceedings{kulesza2012tell,
  title={Tell me more?: the effects of mental model soundness on personalizing an intelligent agent},
  author={Kulesza, Todd and Stumpf, Simone and Burnett, Margaret and Kwan, Irwin},
  booktitle={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
  pages={1--10},
  year={2012},
  organization={ACM}
}

@inproceedings{rosenthal2010towards,
  title={Towards maximizing the accuracy of human-labeled sensor data},
  author={Rosenthal, Stephanie L and Dey, Anind K},
  booktitle={Proceedings of the 15th international conference on Intelligent user interfaces},
  pages={259--268},
  year={2010},
  organization={ACM}
}

@inproceedings{stumpf2007toward,
  title={Toward harnessing user feedback for machine learning},
  author={Stumpf, Simone and Rajaram, Vidya and Li, Lida and Burnett, Margaret and Dietterich, Thomas and Sullivan, Erin and Drummond, Russell and Herlocker, Jonathan},
  booktitle={Proceedings of the 12th international conference on Intelligent user interfaces},
  pages={82--91},
  year={2007},
  organization={ACM}
}

@article{gunning2017explainable,
  title={Explainable artificial intelligence (xai)},
  author={Gunning, David},
  journal={Defense Advanced Research Projects Agency (DARPA), nd Web},
  volume={2},
  year={2017}
}

@article{carvalho2019machine,
  title={Machine Learning Interpretability: A Survey on Methods and Metrics},
  author={Carvalho, Diogo V and Pereira, Eduardo M and Cardoso, Jaime S},
  journal={Electronics},
  volume={8},
  number={8},
  pages={832},
  year={2019},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{guidotti2019survey,
  title={A survey of methods for explaining black box models},
  author={Guidotti, Riccardo and Monreale, Anna and Ruggieri, Salvatore and Turini, Franco and Giannotti, Fosca and Pedreschi, Dino},
  journal={ACM computing surveys (CSUR)},
  volume={51},
  number={5},
  pages={93},
  year={2019},
  publisher={ACM}
}

@article{doshi2017towards,
  title={Towards a rigorous science of interpretable machine learning},
  author={Doshi-Velez, Finale and Kim, Been},
  journal={arXiv preprint arXiv:1702.08608},
  year={2017}
}

@inproceedings{ribeiro2016should,
  title={Why should i trust you?: Explaining the predictions of any classifier},
  author={Ribeiro, Marco Tulio and Singh, Sameer and Guestrin, Carlos},
  booktitle={Proceedings of the 22nd ACM SIGKDD international conference on knowledge discovery and data mining},
  pages={1135--1144},
  year={2016},
  organization={ACM}
}

@inproceedings{hohman2019gamut,
  title={Gamut: A design probe to understand how data scientists understand machine learning models},
  author={Hohman, Fred and Head, Andrew and Caruana, Rich and DeLine, Robert and Drucker, Steven M},
  booktitle={Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems},
  pages={579},
  year={2019},
  organization={ACM}
}

@inproceedings{kulesza2015principles,
  title={Principles of explanatory debugging to personalize interactive machine learning},
  author={Kulesza, Todd and Burnett, Margaret and Wong, Weng-Keen and Stumpf, Simone},
  booktitle={Proceedings of the 20th international conference on intelligent user interfaces},
  pages={126--137},
  year={2015},
  organization={ACM}
}

@inproceedings{brooks2015featureinsight,
  title={FeatureInsight: Visual support for error-driven feature ideation in text classification},
  author={Brooks, Michael and Amershi, Saleema and Lee, Bongshin and Drucker, Steven M and Kapoor, Ashish and Simard, Patrice},
  booktitle={2015 IEEE Conference on Visual Analytics Science and Technology (VAST)},
  pages={105--112},
  year={2015},
  organization={IEEE}
}

@inproceedings{krause2017workflow,
  title={A workflow for visual diagnostics of binary classifiers using instance-level explanations},
  author={Krause, Josua and Dasgupta, Aritra and Swartz, Jordan and Aphinyanaphongs, Yindalon and Bertini, Enrico},
  booktitle={2017 IEEE Conference on Visual Analytics Science and Technology (VAST)},
  pages={162--172},
  year={2017},
  organization={IEEE}
}

@inproceedings{guillory2011simultaneous,
  title={Simultaneous Learning and Covering with Adversarial Noise.},
  author={Guillory, Andrew and Bilmes, Jeff A},
  booktitle={ICML},
  volume={11},
  pages={369--376},
  year={2011}
}

@inproceedings{lundberg2017unified,
  title={A unified approach to interpreting model predictions},
  author={Lundberg, Scott M and Lee, Su-In},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4765--4774},
  year={2017}
}

@inproceedings{dodge2019explaining,
  title={Explaining models: an empirical study of how explanations impact fairness judgment},
  author={Dodge, Jonathan and Liao, Q Vera and Zhang, Yunfeng and Bellamy, Rachel KE and Dugan, Casey},
  booktitle={Proceedings of the 24th International Conference on Intelligent User Interfaces},
  pages={275--285},
  year={2019},
  organization={ACM}
}

@article{mcknight1998initial,
  title={Initial trust formation in new organizational relationships},
  author={McKnight, D Harrison and Cummings, Larry L and Chervany, Norman L},
  journal={Academy of Management review},
  volume={23},
  number={3},
  pages={473--490},
  year={1998},
  publisher={Academy of Management Briarcliff Manor, NY 10510}
}

@article{mcknight2002developing,
  title={Developing and validating trust measures for e-commerce: An integrative typology},
  author={McKnight, D Harrison and Choudhury, Vivek and Kacmar, Charles},
  journal={Information systems research},
  volume={13},
  number={3},
  pages={334--359},
  year={2002},
  publisher={INFORMS}
}

@inproceedings{korber2018theoretical,
  title={Theoretical considerations and development of a questionnaire to measure trust in automation},
  author={K{\"o}rber, Moritz},
  booktitle={Congress of the International Ergonomics Association},
  pages={13--30},
  year={2018},
  organization={Springer}
}

@article{lewis1995computer,
  title={Computer usability satisfaction questionnaires: Psychometric evaluation and instructions for use},
  author={Lewis, JR},
  journal={International Journal of Human-Computer Interaction},
  volume={7},
  number={1},
  pages={57--78},
  year={1995}
}

@article{o2018practical,
  title={A practical approach to measuring user engagement with the refined user engagement scale (UES) and new UES short form},
  author={O’Brien, Heather L and Cairns, Paul and Hall, Mark},
  journal={International Journal of Human-Computer Studies},
  volume={112},
  pages={28--39},
  year={2018},
  publisher={Elsevier}
}

@incollection{hart1988development,
  title={Development of NASA-TLX (Task Load Index): Results of empirical and theoretical research},
  author={Hart, Sandra G and Staveland, Lowell E},
  booktitle={Advances in psychology},
  volume={52},
  pages={139--183},
  year={1988},
  publisher={Elsevier}
}

@article{malle2011attribution,
  title={Attribution theories: How people make sense of behavior},
  author={Malle, Bertram F},
  journal={Theories in social psychology},
  volume={23},
  pages={72--95},
  year={2011}
}

@inproceedings{cai2019effects,
  title={The effects of example-based explanations in a machine learning interface},
  author={Cai, Carrie J and Jongejan, Jonas and Holbrook, Jess},
  booktitle={Proceedings of the 24th International Conference on Intelligent User Interfaces},
  pages={258--262},
  year={2019},
  organization={ACM}
}

@inproceedings{altschuler2019stopping,
  title={Stopping active learning based on predicted change of f measure for text classification},
  author={Altschuler, Michael and Bloodgood, Michael},
  booktitle={2019 IEEE 13th International Conference on Semantic Computing (ICSC)},
  pages={47--54},
  year={2019},
  organization={IEEE}
}

@misc{adultIncome ,
author = "Kohavi, Ronny  and Becker, Barry",
year = "1996",
title = "Adult Income dataset ({UCI} Machine Learning Repository)",
url = "https://archive.ics.uci.edu/ml/datasets/Adult",
institution = "University of California, Irvine, School of Information and Computer Sciences" }

@misc{inflation,
title = "US Inflation Calculator",
year = {2019 (accessed July, 2019)},
howpublished = "\url{https://www.usinflationcalculator.com/}"}
}

@article{yang2018benchmark,
  title={A benchmark and comparison of active learning for logistic regression},
  author={Yang, Yazhou and Loog, Marco},
  journal={Pattern Recognition},
  volume={83},
  pages={401--415},
  year={2018},
  publisher={Elsevier}
}

@article{ren2016squares,
  title={Squares: Supporting interactive performance analysis for multiclass classifiers},
  author={Ren, Donghao and Amershi, Saleema and Lee, Bongshin and Suh, Jina and Williams, Jason D},
  journal={IEEE transactions on visualization and computer graphics},
  volume={23},
  number={1},
  pages={61--70},
  year={2016},
  publisher={IEEE}
}

@article{krause2014infuse,
  title={INFUSE: interactive feature selection for predictive modeling of high dimensional data},
  author={Krause, Josua and Perer, Adam and Bertini, Enrico},
  journal={IEEE transactions on visualization and computer graphics},
  volume={20},
  number={12},
  pages={1614--1623},
  year={2014},
  publisher={IEEE}
}


@article{arya2019one,
  title={One Explanation Does Not Fit All: A Toolkit and Taxonomy of AI Explainability Techniques},
  author={Arya, Vijay and Bellamy, Rachel KE and Chen, Pin-Yu and Dhurandhar, Amit and Hind, Michael and Hoffman, Samuel C and Houde, Stephanie and Liao, Q Vera and Luss, Ronny and Mojsilovi{\'c}, Aleksandra and others},
  journal={arXiv preprint arXiv:1909.03012},
  year={2019}
}

@inproceedings{kulesza2013too,
  title={Too much, too little, or just right? Ways explanations impact end users' mental models},
  author={Kulesza, Todd and Stumpf, Simone and Burnett, Margaret and Yang, Sherry and Kwan, Irwin and Wong, Weng-Keen},
  booktitle={2013 IEEE Symposium on Visual Languages and Human Centric Computing},
  pages={3--10},
  year={2013},
  organization={IEEE}
}

@book{cramer2004sage,
  title={The Sage dictionary of statistics: a practical resource for students in the social sciences},
  author={Cramer, Duncan and Howitt, Dennis Laurence},
  year={2004},
  publisher={Sage}
}

@inproceedings{qbc,
  title={Query by committee},
  author={Seung, H Sebastian and Opper, Manfred and Sompolinsky, Haim},
  booktitle={Proceedings of the fifth annual workshop on Computational learning theory},
  pages={287--294},
  year={1992},
  organization={ACM}
}

@inproceedings{unc,
  title={A sequential algorithm for training text classifiers},
  author={Lewis, David D and Gale, William A},
  booktitle={SIGIR’94},
  pages={3--12},
  year={1994},
  organization={Springer}
}

@inproceedings{dasgupta2008hierarchical,
  title={Hierarchical sampling for active learning},
  author={Dasgupta, Sanjoy and Hsu, Daniel},
  booktitle={Proceedings of the 25th international conference on Machine learning},
  pages={208--215},
  year={2008},
  organization={ACM}
}

@inproceedings{quire,
  title={Active learning by querying informative and representative examples},
  author={Huang, Sheng-Jun and Jin, Rong and Zhou, Zhi-Hua},
  booktitle={Advances in neural information processing systems},
  pages={892--900},
  year={2010}
}

@article{qbc2,
  title={Selective sampling using the query by committee algorithm},
  author={Freund, Yoav and Seung, H Sebastian and Shamir, Eli and Tishby, Naftali},
  journal={Machine learning},
  volume={28},
  number={2-3},
  pages={133--168},
  year={1997},
  publisher={Springer}
}

@inproceedings{entropy,
  title={An analysis of active learning strategies for sequence labeling tasks},
  author={Settles, Burr and Craven, Mark},
  booktitle={Proceedings of the conference on empirical methods in natural language processing},
  pages={1070--1079},
  year={2008},
  organization={Association for Computational Linguistics}
}

@inproceedings{confidence,
  title={Reducing labeling effort for structured prediction tasks},
  author={Culotta, Aron and McCallum, Andrew},
  booktitle={AAAI},
  volume={5},
  pages={746--751},
  year={2005}
}

@inproceedings{margin,
  title={Margin based active learning},
  author={Balcan, Maria-Florina and Broder, Andrei and Zhang, Tong},
  booktitle={International Conference on Computational Learning Theory},
  pages={35--50},
  year={2007},
  organization={Springer}
}

@inproceedings{batchSize,
  title={Impact of batch size on stopping active learning for text classification},
  author={Beatty, Garrett and Kochis, Ethan and Bloodgood, Michael},
  booktitle={2018 IEEE 12th International Conference on Semantic Computing (ICSC)},
  pages={306--307},
  year={2018},
  organization={IEEE}
}

@article{song2018active,
  title={Active learning with confidence-based answers for crowdsourcing labeling tasks},
  author={Song, Jinhua and Wang, Hao and Gao, Yang and An, Bo},
  journal={Knowledge-Based Systems},
  volume={159},
  pages={244--258},
  year={2018},
  publisher={Elsevier}
}

@article{poursabzi2018manipulating,
  title={Manipulating and measuring model interpretability},
  author={Poursabzi-Sangdeh, Forough and Goldstein, Daniel G and Hofman, Jake M and Vaughan, Jennifer Wortman and Wallach, Hanna},
  journal={arXiv preprint arXiv:1802.07810},
  year={2018}
}

@inproceedings{cheng2019explaining,
  title={Explaining Decision-Making Algorithms through UI: Strategies to Help Non-Expert Stakeholders},
  author={Cheng, Hao-Fei and Wang, Ruotong and Zhang, Zheng and O'Connell, Fiona and Gray, Terrance and Harper, F Maxwell and Zhu, Haiyi},
  booktitle={Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems},
  pages={559},
  year={2019},
  organization={ACM}
}

@article{thomaz2008teachable,
  title={Teachable robots: Understanding human teaching behavior to build more effective robot learners},
  author={Thomaz, Andrea L and Breazeal, Cynthia},
  journal={Artificial Intelligence},
  volume={172},
  number={6-7},
  pages={716--737},
  year={2008},
  publisher={Elsevier}
}

@inproceedings{knox2012reinforcement,
  title={Reinforcement learning from human reward: Discounting in episodic tasks},
  author={Knox, W Bradley and Stone, Peter},
  booktitle={2012 IEEE RO-MAN: The 21st IEEE International Symposium on Robot and Human Interactive Communication},
  pages={878--885},
  year={2012},
  organization={IEEE}
}

@inproceedings{springer2019progressive,
  title={Progressive disclosure: empirically motivated approaches to designing effective transparency},
  author={Springer, Aaron and Whittaker, Steve},
  booktitle={Proceedings of the 24th International Conference on Intelligent User Interfaces},
  pages={107--120},
  year={2019},
  organization={ACM}
}

@article{lee2017human,
  title={The human touch: How non-expert users perceive, interpret, and fix topic models},
  author={Lee, Tak Yeon and Smith, Alison and Seppi, Kevin and Elmqvist, Niklas and Boyd-Graber, Jordan and Findlater, Leah},
  journal={International Journal of Human-Computer Studies},
  volume={105},
  pages={28--42},
  year={2017},
  publisher={Elsevier}
}

@inproceedings{lai2019human,
  title={On Human Predictions with Explanations and Predictions of Machine Learning Models: A Case Study on Deception Detection},
  author={Lai, Vivian and Tan, Chenhao},
  booktitle={Proceedings of the Conference on Fairness, Accountability, and Transparency},
  pages={29--38},
  year={2019},
  organization={ACM}
}

@inproceedings{chou2014democratizing,
  title={Democratizing data science},
  author={Chou, Sophie and Li, William and Sridharan, Ramesh},
  booktitle={Proceedings of the KDD 2014 20th ACM SIGKDD International Conference on Knowledge Discovery and Data Mining, New York, NY, USA},
  pages={24--27},
  year={2014},
  organization={Citeseer}
}



@inproceedings{fogarty2008cueflik,
  title={CueFlik: interactive concept learning in image search},
  author={Fogarty, James and Tan, Desney and Kapoor, Ashish and Winder, Simon},
  booktitle={Proceedings of the sigchi conference on human factors in computing systems},
  pages={29--38},
  year={2008}
}


@article{wellman2004theory,
  title={Theory of mind for learning and teaching: The nature and role of explanation},
  author={Wellman, Henry M and Lagattuta, Kristin H},
  journal={Cognitive development},
  volume={19},
  number={4},
  pages={479--497},
  year={2004},
  publisher={Elsevier}
}

 @article{meyer1997consensually,
  title={Consensually driven explanation in science teaching},
  author={Meyer, Karen and Woodruff, Earl},
  journal={Science Education},
  volume={81},
  number={2},
  pages={173--192},
  year={1997},
  publisher={Wiley Online Library}
}

@inproceedings{lim2009and,
  title={Why and why not explanations improve the intelligibility of context-aware intelligent systems},
  author={Lim, Brian Y and Dey, Anind K and Avrahami, Daniel},
  booktitle={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
  pages={2119--2128},
  year={2009}
}

@inproceedings{pu2006trust,
  title={Trust building with explanation interfaces},
  author={Pu, Pearl and Chen, Li},
  booktitle={Proceedings of the 11th international conference on Intelligent user interfaces},
  pages={93--100},
  year={2006}
}

@inproceedings{kocielnik2019will,
  title={Will you accept an imperfect ai? exploring designs for adjusting end-user expectations of ai systems},
  author={Kocielnik, Rafal and Amershi, Saleema and Bennett, Paul N},
  booktitle={Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems},
  pages={1--14},
  year={2019}
}

@inproceedings{stumpf2016explanations,
  title={Explanations considered harmful? user interactions with machine learning systems},
  author={Stumpf, Simone and Bussone, Adrian and O’sullivan, Dympna},
  booktitle={Proceedings of the ACM SIGCHI Conference on Human Factors in Computing Systems (CHI)},
  year={2016}
}


@inproceedings{buccinca2020proxy,
  title={Proxy tasks and subjective measures can be misleading in evaluating explainable AI systems},
  author={Bu{\c{c}}inca, Zana and Lin, Phoebe and Gajos, Krzysztof Z and Glassman, Elena L},
  booktitle={Proceedings of the 25th International Conference on Intelligent User Interfaces},
  pages={454--464},
  year={2020}
}

@article{smithno,
  title={No Explainability without Accountability: An Empirical Study of Explanations and Feedback in Interactive ML},
  author={Smith-Renner, Alison and Fan, Ron and Birchfield, Melissa and Wu, Tongshuang and Boyd-Graber, Jordan and Weld, Dan and Findlater, Leah}
}


@article{wu2019local,
  title={Local Decision Pitfalls in Interactive Machine Learning: An Investigation into Feature Selection in Sentiment Analysis},
  author={Wu, Tongshuang and Weld, Daniel S and Heer, Jeffrey},
  journal={ACM Transactions on Computer-Human Interaction (TOCHI)},
  volume={26},
  number={4},
  pages={1--27},
  year={2019},
  publisher={ACM New York, NY, USA}
}

@inproceedings{ahn2007open,
  title={Open user profiles for adaptive news systems: help or harm?},
  author={Ahn, Jae-wook and Brusilovsky, Peter and Grady, Jonathan and He, Daqing and Syn, Sue Yeon},
  booktitle={Proceedings of the 16th international conference on World Wide Web},
  pages={11--20},
  year={2007}
}

@article{stumpf2009interacting,
  title={Interacting meaningfully with machine learning systems: Three experiments},
  author={Stumpf, Simone and Rajaram, Vidya and Li, Lida and Wong, Weng-Keen and Burnett, Margaret and Dietterich, Thomas and Sullivan, Erin and Herlocker, Jonathan},
  journal={International Journal of Human-Computer Studies},
  volume={67},
  number={8},
  pages={639--662},
  year={2009},
  publisher={Elsevier}
}

@inproceedings{wagstaff2001constrained,
  title={Constrained k-means clustering with background knowledge},
  author={Wagstaff, Kiri and Cardie, Claire and Rogers, Seth and Schr{\"o}dl, Stefan and others},
  booktitle={Icml},
  volume={1},
  pages={577--584},
  year={2001}
}

@article{altendorf2012learning,
  title={Learning from sparse data by exploiting monotonicity constraints},
  author={Altendorf, Eric E and Restificar, Angelo C and Dietterich, Thomas G},
  journal={arXiv preprint arXiv:1207.1364},
  year={2012}
}

@inproceedings{kapoor2010interactive,
  title={Interactive optimization for steering machine classification},
  author={Kapoor, Ashish and Lee, Bongshin and Tan, Desney and Horvitz, Eric},
  booktitle={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
  pages={1343--1352},
  year={2010}
}

@inproceedings{vig2011navigating,
  title={Navigating the tag genome},
  author={Vig, Jesse and Sen, Shilad and Riedl, John},
  booktitle={Proceedings of the 16th international conference on Intelligent user interfaces},
  pages={93--102},
  year={2011}
}

@article{kulesza2011oriented,
  title={Why-oriented end-user debugging of naive Bayes text classification},
  author={Kulesza, Todd and Stumpf, Simone and Wong, Weng-Keen and Burnett, Margaret M and Perona, Stephen and Ko, Andrew and Oberst, Ian},
  journal={ACM Transactions on Interactive Intelligent Systems (TiiS)},
  volume={1},
  number={1},
  pages={1--31},
  year={2011},
  publisher={ACM New York, NY, USA}
}

@inproceedings{amershi2015modeltracker,
  title={Modeltracker: Redesigning performance analysis tools for machine learning},
  author={Amershi, Saleema and Chickering, Max and Drucker, Steven M and Lee, Bongshin and Simard, Patrice and Suh, Jina},
  booktitle={Proceedings of the 33rd Annual ACM Conference on Human Factors in Computing Systems},
  pages={337--346},
  year={2015}
}

@inproceedings{krause2016interacting,
  title={Interacting with predictions: Visual inspection of black-box machine learning models},
  author={Krause, Josua and Perer, Adam and Ng, Kenney},
  booktitle={Proceedings of the 2016 CHI Conference on Human Factors in Computing Systems},
  pages={5686--5697},
  year={2016}
}


}

@article{choo2013utopian,
  title={Utopian: User-driven topic modeling based on interactive nonnegative matrix factorization},
  author={Choo, Jaegul and Lee, Changhyun and Reddy, Chandan K and Park, Haesun},
  journal={IEEE transactions on visualization and computer graphics},
  volume={19},
  number={12},
  pages={1992--2001},
  year={2013},
  publisher={IEEE}
}

@inproceedings{smith2018closing,
  title={Closing the loop: User-centered design and evaluation of a human-in-the-loop topic modeling system},
  author={Smith, Alison and Kumar, Varun and Boyd-Graber, Jordan and Seppi, Kevin and Findlater, Leah},
  booktitle={23rd International Conference on Intelligent User Interfaces},
  pages={293--304},
  year={2018}
}

@inproceedings{talbot2009ensemblematrix,
  title={EnsembleMatrix: interactive visualization to support machine learning with multiple classifiers},
  author={Talbot, Justin and Lee, Bongshin and Kapoor, Ashish and Tan, Desney S},
  booktitle={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
  pages={1283--1292},
  year={2009}
}

@article{wexler2019if,
  title={The What-If Tool: Interactive probing of machine learning models},
  author={Wexler, James and Pushkarna, Mahima and Bolukbasi, Tolga and Wattenberg, Martin and Vi{\'e}gas, Fernanda and Wilson, Jimbo},
  journal={IEEE transactions on visualization and computer graphics},
  volume={26},
  number={1},
  pages={56--65},
  year={2019},
  publisher={IEEE}
}

@inproceedings{donmez2008proactive,
  title={Proactive learning: cost-sensitive active learning with multiple imperfect oracles},
  author={Donmez, Pinar and Carbonell, Jaime G},
  booktitle={Proceedings of the 17th ACM conference on Information and knowledge management},
  pages={619--628},
  year={2008}
}



@inproceedings{cheng2015measuring,
  title={Measuring crowdsourcing effort with error-time curves},
  author={Cheng, Justin and Teevan, Jaime and Bernstein, Michael S},
  booktitle={Proceedings of the 33rd Annual ACM Conference on Human Factors in Computing Systems},
  pages={1365--1374},
  year={2015}
}



@inproceedings{zhang2020effect,
title={Effect of Confidence and Explanation on Accuracy and Trust Calibration in AI-Assisted Decision Making},
    author={Zhang, Yunfeng and Liao, Q Vera and Bellamy, Rachel KE},
  booktitle={Proceedings of the Conference on Fairness, Accountability, and Transparency},
  year={2020},
  organization={ACM}
}



@inproceedings{liao2020questioning,
  title={Questioning the AI: Informing Design Practices for Explainable AI User Experiences},
  author={Liao, Q Vera and Gruen, Daniel and Miller, Sarah},
  booktitle={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
  year={2020},
  organization={ACM}
}


@article{tomsett2018interpretable,
  title={Interpretable to whom? A role-based model for analyzing interpretable machine learning systems},
  author={Tomsett, Richard and Braines, Dave and Harborne, Dan and Preece, Alun and Chakraborty, Supriyo},
  journal={arXiv preprint arXiv:1806.07552},
  year={2018}
}

@inproceedings{gurumoorthy2019efficient,
  title={Efficient Data Representation by Selecting Prototypes with Importance Weights},
  author={Gurumoorthy, Karthik S and Dhurandhar, Amit and Cecchi, Guillermo and Aggarwal, Charu},
  booktitle={2019 IEEE International Conference on Data Mining (ICDM)},
  pages={260--269},
  year={2019},
  organization={IEEE}
}

@article{narayanan2018humans,
  title={How do humans understand explanations from machine learning systems? an evaluation of the human-interpretability of explanation},
  author={Narayanan, Menaka and Chen, Emily and He, Jeffrey and Kim, Been and Gershman, Sam and Doshi-Velez, Finale},
  journal={arXiv preprint arXiv:1802.00682},
  year={2018}
}

@article{zhang2018manifold,
  title={Manifold: A model-agnostic framework for interpretation and diagnosis of machine learning models},
  author={Zhang, Jiawei and Wang, Yang and Molino, Piero and Li, Lezhi and Ebert, David S},
  journal={IEEE transactions on visualization and computer graphics},
  volume={25},
  number={1},
  pages={364--373},
  year={2018},
  publisher={IEEE}
}

@article{cacioppo1982need,
  title={The need for cognition.},
  author={Cacioppo, John T and Petty, Richard E},
  journal={Journal of personality and social psychology},
  volume={42},
  number={1},
  pages={116},
  year={1982},
  publisher={American Psychological Association}
}

@inproceedings{sokol2020explainability,
  title={Explainability fact sheets: a framework for systematic assessment of explainable approaches},
  author={Sokol, Kacper and Flach, Peter},
  booktitle={Proceedings of the 2020 Conference on Fairness, Accountability, and Transparency},
  pages={56--67},
  year={2020}
}

@article{cacioppo1983effects,
  title={Effects of need for cognition on message evaluation, recall, and persuasion.},
  author={Cacioppo, John T and Petty, Richard E and Morris, Katherine J},
  journal={Journal of personality and social psychology},
  volume={45},
  number={4},
  pages={805},
  year={1983},
  publisher={American Psychological Association}
}

@article{haugtvedt1992personality,
  title={Personality and persuasion: Need for cognition moderates the persistence and resistance of attitude changes.},
  author={Haugtvedt, Curtis P and Petty, Richard E},
  journal={Journal of Personality and Social psychology},
  volume={63},
  number={2},
  pages={308},
  year={1992},
  publisher={American Psychological Association}
}

@incollection{lombrozo2012explanation,
  title={Explanation and Abductive Inference},
  author={Lombrozo, Tania},
  booktitle={The Oxford Handbook of Thinking and Reasoning},
  year={2012},
  publisher={Oxford University Press}
}



@article{mohseni2018multidisciplinary,
  title={A Multidisciplinary Survey and Framework for Design and Evaluation of Explainable AI Systems},
  author={Mohseni, Sina and Zarei, Niloofar and Ragan, Eric D},
  journal={arXiv},
  pages={arXiv--1811},
  year={2018}
}



@article{arrieta2019explainable,
  title={Explainable Artificial Intelligence (XAI): Concepts, Taxonomies, Opportunities and Challenges toward Responsible AI},
  author={Arrieta, Alejandro Barredo and D{\'\i}az-Rodr{\'\i}guez, Natalia and Del Ser, Javier and Bennetot, Adrien and Tabik, Siham and Barbado, Alberto and Garc{\'\i}a, Salvador and Gil-L{\'o}pez, Sergio and Molina, Daniel and Benjamins, Richard and others},
  journal={Information Fusion},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{lim2019these,
  title={Why these Explanations? Selecting Intelligibility Types for Explanation Goals.},
  author={Lim, Brian Y and Yang, Qian and Abdul, Ashraf M and Wang, Danding},
  booktitle={IUI Workshops},
  year={2019}
}

@article{lipton2018mythos,
  title={The mythos of model interpretability},
  author={Lipton, Zachary C},
  journal={Queue},
  volume={16},
  number={3},
  pages={31--57},
  year={2018},
  publisher={ACM New York, NY, USA}
}

@inproceedings{wang2019designing,
  title={Designing theory-driven user-centric explainable AI},
  author={Wang, Danding and Yang, Qian and Abdul, Ashraf and Lim, Brian Y},
  booktitle={Proceedings of the 2019 CHI conference on human factors in computing systems},
  pages={1--15},
  year={2019}
}


@article{chakraborti2020emerging,
  title={The Emerging Landscape of Explainable AI Planning and Decision Making},
  author={Chakraborti, Tathagata and Sreedharan, Sarath and Kambhampati, Subbarao},
  journal={arXiv preprint arXiv:2002.11697},
  year={2020}
}


@article{rosenfeld2019explainability,
  title={Explainability in human--agent systems},
  author={Rosenfeld, Avi and Richardson, Ariella},
  journal={Autonomous Agents and Multi-Agent Systems},
  volume={33},
  number={6},
  pages={673--705},
  year={2019},
  publisher={Springer}
}

@inproceedings{lim2010toolkit,
  title={Toolkit to support intelligibility in context-aware applications},
  author={Lim, Brian Y and Dey, Anind K},
  booktitle={Proceedings of the 12th ACM international conference on Ubiquitous computing},
  pages={13--22},
  year={2010}
}


@article{gurumoorthy2017protodash,
  title={Protodash: Fast interpretable prototype selection},
  author={Gurumoorthy, Karthik S and Dhurandhar, Amit and Cecchi, Guillermo},
  journal={arXiv preprint arXiv:1707.01212},
  year={2017}
}
@article{bien2011prototype,
  title={Prototype selection for interpretable classification},
  author={Bien, Jacob and Tibshirani, Robert and others},
  journal={The Annals of Applied Statistics},
  volume={5},
  number={4},
  pages={2403--2424},
  year={2011},
  publisher={Institute of Mathematical Statistics}
}

@inproceedings{ribeiro2018anchors,
  title={Anchors: High-precision model-agnostic explanations},
  author={Ribeiro, Marco Tulio and Singh, Sameer and Guestrin, Carlos},
  booktitle={Thirty-Second AAAI Conference on Artificial Intelligence},
  year={2018}
}

@inproceedings{hanafi2017seer,
  title={Seer: Auto-generating information extraction rules from user-specified examples},
  author={Hanafi, Maeda F and Abouzied, Azza and Chiticariu, Laura and Li, Yunyao},
  booktitle={Proceedings of the 2017 CHI Conference on Human Factors in Computing Systems},
  pages={6672--6682},
  year={2017}
}

@inproceedings{zaidan2007using,
  title={Using “annotator rationales” to improve machine learning for text categorization},
  author={Zaidan, Omar and Eisner, Jason and Piatko, Christine},
  booktitle={Human language technologies 2007: The conference of the North American chapter of the association for computational linguistics; proceedings of the main conference},
  pages={260--267},
  year={2007}
}
  


@article{ghai2020explainable,
  title={Explainable Active Learning (XAL): An Empirical Study of How Local Explanations Impact Annotator Experience},
  author={Ghai, Bhavya and Liao, Q Vera and Zhang, Yunfeng and Bellamy, Rachel and Mueller, Klaus},
  journal={arXiv preprint arXiv:2001.09219},
  year={2020}
}

@techreport{settles2009active,
  title={Active learning literature survey},
  author={Settles, Burr},
  year={2009},
  institution={University of Wisconsin-Madison Department of Computer Sciences}
}

@article{liu2019incorporating,
  title={Incorporating priors with feature attribution on text classification},
  author={Liu, Frederick and Avci, Besim},
  journal={arXiv preprint arXiv:1906.08286},
  year={2019}
}

@inproceedings{al_bagging,
  title={Query learning strategies using boosting and bagging},
  author={Mamitsuka, Naoki Abe Hiroshi and others},
  booktitle={Machine learning: proceedings of the fifteenth international conference (ICML’98)},
  volume={1},
  year={1998},
  organization={Morgan Kaufmann Pub}
}

@unpublished{adultUCI,
title= {Adult Census Income dataset},
author = {UCI Machine Learning Repository},
URL= {https://archive.ics.uci.edu/ml/datasets/adult},
year = {1998}
}

@inproceedings{raghavan2007interactive,
  title={An interactive algorithm for asking and incorporating feature feedback into support vector machines},
  author={Raghavan, Hema and Allan, James},
  booktitle={Proceedings of the 30th annual international ACM SIGIR conference on Research and development in information retrieval},
  pages={79--86},
  year={2007}
}
@inproceedings{ribeiro2016should,
  title={" Why should i trust you?" Explaining the predictions of any classifier},
  author={Ribeiro, Marco Tulio and Singh, Sameer and Guestrin, Carlos},
  booktitle={Proceedings of the 22nd ACM SIGKDD international conference on knowledge discovery and data mining},
  pages={1135--1144},
  year={2016}
}

@article{crowdsourcing,
  author  = {Jennifer Wortman Vaughan},
  title   = {Making Better Use of the Crowd: How Crowdsourcing Can Advance Machine Learning Research},
  journal = {Journal of Machine Learning Research},
  year    = {2018},
  volume  = {18},
  number  = {193},
  pages   = {1-46},
  url     = {http://jmlr.org/papers/v18/17-234.html}
}

@inproceedings{gadiraju,
  title={Understanding and mitigating worker biases in the crowdsourced collection of subjective judgments},
  author={Hube, Christoph and Fetahu, Besnik and Gadiraju, Ujwal},
  booktitle={Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems},
  pages={407},
  year={2019},
  organization={ACM}
}

@incollection{gender_survey,
  title={The ambivalent sexism inventory: Differentiating hostile and benevolent sexism},
  author={Glick, Peter and Fiske, Susan T},
  booktitle={Social Cognition},
  pages={116--160},
  year={2018},
  publisher={Routledge}
}

@inproceedings{kusner2017counterfactual,
  title={Counterfactual fairness},
  author={Kusner, Matt J and Loftus, Joshua and Russell, Chris and Silva, Ricardo},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4066--4076},
  year={2017}
}

@article{zhao2017men,
  title={Men also like shopping: Reducing gender bias amplification using corpus-level constraints},
  author={Zhao, Jieyu and Wang, Tianlu and Yatskar, Mark and Ordonez, Vicente and Chang, Kai-Wei},
  journal={arXiv preprint arXiv:1707.09457},
  year={2017}
}

@inproceedings{wikipedia,
  title={It's a man's Wikipedia? Assessing gender inequality in an online encyclopedia},
  author={Wagner, Claudia and Garcia, David and Jadidi, Mohsen and Strohmaier, Markus},
  booktitle={Ninth international AAAI conference on web and social media},
  year={2015}
}

@inproceedings{varshneyNIPS2017,
  title={Optimized pre-processing for discrimination prevention},
  author={Calmon, Flavio and Wei, Dennis and Vinzamuri, Bhanukiran and Ramamurthy, Karthikeyan Natesan and Varshney, Kush R},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3992--4001},
  year={2017}
}

@inproceedings{garg2019counterfactual,
  title={Counterfactual fairness in text classification through robustness},
  author={Garg, Sahaj and Perot, Vincent and Limtiaco, Nicole and Taly, Ankur and Chi, Ed H and Beutel, Alex},
  booktitle={Proceedings of the 2019 AAAI/ACM Conference on AI, Ethics, and Society},
  pages={219--226},
  year={2019}
}

@book{o2016weapons,
  title={Weapons of math destruction: How big data increases inequality and threatens democracy},
  author={O'neil, Cathy},
  year={2016},
  publisher={Broadway Books}
}

@article{bellamy2018ai,
  title={AI Fairness 360: An extensible toolkit for detecting, understanding, and mitigating unwanted algorithmic bias},
  author={Bellamy, Rachel KE and Dey, Kuntal and Hind, Michael and Hoffman, Samuel C and Houde, Stephanie and Kannan, Kalapriya and Lohia, Pranay and Martino, Jacquelyn and Mehta, Sameep and Mojsilovic, Aleksandra and others},
  journal={arXiv preprint arXiv:1810.01943},
  year={2018}
}

@inproceedings{microtalk,
  title={Microtalk: Using argumentation to improve crowdsourcing accuracy},
  author={Drapeau, Ryan and Chilton, Lydia B and Bragg, Jonathan and Weld, Daniel S},
  booktitle={Fourth AAAI Conference on Human Computation and Crowdsourcing},
  year={2016}
}

@inproceedings{reputation,
  title={Reputation-based worker filtering in crowdsourcing},
  author={Jagabathula, Srikanth and Subramanian, Lakshminarayanan and Venkataraman, Ashwin},
  booktitle={Advances in Neural Information Processing Systems},
  pages={2492--2500},
  year={2014}
}

@article{qualityControl,
  title={Quality control in crowdsourcing: A survey of quality attributes, assessment techniques, and assurance actions},
  author={Daniel, Florian and Kucherbaev, Pavel and Cappiello, Cinzia and Benatallah, Boualem and Allahbakhsh, Mohammad},
  journal={ACM Computing Surveys (CSUR)},
  volume={51},
  number={1},
  pages={1--40},
  year={2018},
  publisher={ACM New York, NY, USA}
}

@article{iat,
  title={Measuring individual differences in implicit cognition: the implicit association test.},
  author={Greenwald, Anthony G and McGhee, Debbie E and Schwartz, Jordan LK},
  journal={Journal of personality and social psychology},
  volume={74},
  number={6},
  pages={1464},
  year={1998},
  publisher={American Psychological Association}
}

@article{iat_counter,
  title={A meta-analysis of procedures to change implicit measures.},
  author={Forscher, Patrick S and Lai, Calvin K and Axt, Jordan R and Ebersole, Charles R and Herman, Michelle and Devine, Patricia G and Nosek, Brian A},
  journal={Journal of personality and social psychology},
  volume={117},
  number={3},
  pages={522},
  year={2019},
  publisher={American Psychological Association}
  }


@article{sdb_race,
  title={The interdependence of determinants for the strength and direction of social disirability bias in racial attitude surveys},
  author={Stock{\'e}, Volker},
  year={2004}
}

@article{sdb_samesex,
  title={Social desirability bias in polling on same-sex marriage ballot measures},
  author={Powell, Richard J},
  journal={American Politics Research},
  volume={41},
  number={6},
  pages={1052--1070},
  year={2013},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{sdb,
  title={Social-desirability bias and the validity of self-reported values},
  author={Fisher, Robert J and Katz, James E},
  journal={Psychology \& marketing},
  volume={17},
  number={2},
  pages={105--120},
  year={2000},
  publisher={Wiley Online Library}
}

@inproceedings{jigsaw,
  title={Measuring and mitigating unintended bias in text classification},
  author={Dixon, Lucas and Li, John and Sorensen, Jeffrey and Thain, Nithum and Vasserman, Lucy},
  booktitle={Proceedings of the 2018 AAAI/ACM Conference on AI, Ethics, and Society},
  pages={67--73},
  year={2018}
}
